Convex Online Video Frame Subset Selection using Multiple Criteria for Data Efficient Autonomous Driving

Training vision-based Urban Autonomous driving models is a challenging problem, which is highly researched in recent times. Training such models is a data-intensive task requiring the storage and processing of vast volumes of (possibly redundant) driving video data. In this paper, we study the problem of developing data-efficient autonomous driving systems. In this context, we study the problem of multi-criteria online video frame subset selection. We study convex optimization-based solutions and show that they are unable to provide solutions with high weightage to the loss of selected video frames. We design a novel convex optimization-based multi-criteria online subset selection algorithm that uses a thresholded concave function of selection variables. We also propose and study a submodular optimization-based algorithm. Extensive experiments using the driving simulator CARLA show that we are able to drop 80% of the frames while succeeding to complete 100% of the episodes w.r.t. the model trained on 100% data, in the most difficult task of taking turns. This results in a training time of less than 30% compared to training on the whole dataset. We also perform detailed experiments on prediction performances of various affordances used by the Conditional Affordance Learning (CAL) model and show that our subset selection improves performance on the crucial affordance "Relative Angle" during turns.

==> experiment1.tex <==
% \tr{
% - Comparison of approximate online subset selection methods:\\
% -- synthetic data: our method, PRL 2020, sub-modular. Can we compare against other methods?\\
% -- Video data: our method, PRL 2020, sub-modular.\\
% -- Sequential application \\
% -- comparison of PRL with variation in $\rho$
% - Data efficient autonomous driving:\\
% -- 
% }


In this section, we show a comparison of approximate online subset selection methods over synthetic data and our collected driving data from the CARLA simulator \cite{dosovitskiy2017carla}. Next, we compare the performances of various subset selection methods in the autonomous driving application from two aspects: episode completion and affordance prediction.

\subsection{Experimental Setup}

\textbf{Dataset}: We use the open-source driving simulator CARLA\cite{dosovitskiy2017carla} for generating our driving dataset. CARLA simulates an urban driving scenario where there are several other non-player agents like other vehicles, pedestrians, traffic lights and speed signs aiding the player agent vehicle.
In order to collect the training data, the agent vehicle was navigated using the Conditional Affordance Learning controller \cite{sauer2018conditional} based on the ground truth affordances like red light, hazard stop etc. which have been described later in this section. The affordances have been determined and categorised following \cite{sauer2018conditional}. We generated the driving data comprising of 262 episodes and a total of approximately 100,000 frames. We performed the experiments on our generated dataset and compared the subsets obtained using different selection methods.

% where the agent vehicle is driven by the game AI.
For each episode run, we collect: (1) images from camera attached to the agent vehicle, and (2) the corresponding six affordances (Discrete: Red Light, Hazard Stop, Speed Sign ; Continuous: Relative Angle, Centerline Distance, Vehicle Distance) \cite{sauer2018conditional}. Affordances are signals useful for navigation in the environment. We used approximately $85\%$ of the collected dataset as the training set, and the remaining as the test set.
 
 We ensured the similar distribution of affordances in both the training and test set. Figure \ref{fig:distrib} illustrates the distribution of four affordances per class label, in training and test set. Red light and Hazard Stop have two classes - \textit{True}, \textit{False}, Speed sign has four classes - \textit{None} , \textit{30kmph}, \textit{60kmph}, \textit{90kmph}, while in case of Relative angle which is the orientation angle of the agent vehicle, we have grouped the values into buckets corresponding to \textit{Left turn}, \textit{Straight} and \textit{Right turn}. We can divide the entire range of Relative Angle affordance across 20 buckets ranging from -1.0 to +1.0. Note that buckets corresponding to (-1.0 to -0.1), (-0.1 to 0.1) and (0.1 to 1.0) approximately indicate the left turn, straight road and right turn respectively.
 
 \begin{figure}[h!]
    %\centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_red.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:red}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_rel.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:relang}
    \caption{}
    \end{subfigure}
    % \captionsetup{justification=centering}
    % \caption{\textbf{Distribution of affordances: (\textit{Left}) : Red Light and (\textit{Right}) : Relative Angle in training and test set}}
    % \label{fig:distrib}
    
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_speed.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:spd}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_haz.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:haz}
    \caption{}
    \end{subfigure}
    %\captionsetup{justification=centering}
    \caption{\textbf{Distribution of affordances: (a) : Red Light (b) : Relative Angle (c) : Speed Sign (d) : Hazard Stop in training and test set}} 
    \label{fig:distrib}
    % \begin{subfigure}{0.48\columnwidth}
    % \centering
    % \includegraphics[width=\textwidth,height=2.5cm]{figures/speedsign.eps}
    % %\caption{Red light Affordance Distribution}
    % \label{fig:turn}
    % \end{subfigure}
    
    
\end{figure}

\subsection{Comparison of approximate online subset selection methods}

% We compare the performance of the online subset selection methods empirically in terms of their objective function values. 
% We show in Figure \ref{fig:convsub} the objective function values for the proposed method, \citep{das2020multi} method and the submodular approach \citep{buchbinder2014submodular}. For the synthesized data, we generated 10 random samples of dimension $100 \times 100$. Since the submodular approach is a randomized algorithm, we made 100 runs for each sample and show a box plot of the submodular method's objective function values. 

In this section, we compare the optimal subsets reported by the baseline method \cite{das2020multi}, submodular method, proposed convex optimization based method in terms of final objective function values. 
Figure \ref{fig:convsub} shows the objective function values for the three approaches, for 10 randomly synthesized problem instances ($d$ matrix of dimension $100\times 100$ and $l$ vector of dimension $100$ in equation \ref{eq:}). For the submodular method, we report a box plot of results over 100 runs of the algorithm to capture the randomness. While all three methods, find approximate solutions, the proposed convex method consistently finds lower values of objective function, followed by \cite{das2020multi}, and submodular optimization.


For the real data (CARLA data for our further experiments), we report the same for each episode in our collected data. Here, we are aiming at minimizing the objective function and we can clearly observe that function values attained by our proposed method lies below that of both the other approximate methods, thus proving our method to be an efficient approach. 
% We also reported in Table \ref{tab:measure} the mean \% difference between the objective function values of convex and submodular approach, and the mean time taken to optimise the synthesized data samples.
\vspace{-2.7mm}
\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/conv_prl_subm_syn_rename.pdf}a
    %\caption{Red light Affordance Distribution}
    \label{fig:synbox}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
     \centering
     \includegraphics[width=\textwidth,height=2.5cm]{figures/conv_prl_subm_real_rename.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:realbox}
    \caption{}
     \end{subfigure}
     \caption{\textbf{Objective function values for proposed method , \citep{das2020multi} method and Submodular method for (a) Synthetic data (b) CARLA driving data samples}}
     \label{fig:convsub}
 \end{figure}  

% \begin{table}[h!]
% \caption{\textbf{Captured mean \% difference in objective function values between Convex and Submodular approach and mean time taken to optimize on 100 x 100 synthesized data}}
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}\% Difference\\ between Convex\\ and Submodular\end{tabular} & \begin{tabular}[c]{@{}l@{}}Time taken\\ for Convex\\ (seconds)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Time taken\\ for Submodular\\ (seconds)\end{tabular} \\ \hline
% 4.67                                                                                    & 2.5                                                                         & 1.0                                                                             \\ \hline
% \end{tabular}
% \label{tab:measure}
% \end{table}
%\vspace{-4mm}
We show in Figure \ref{fig:inctime} the effect of using online subset selection mechanism. We observe the change in objective function values across increasing time-steps. The objective function values show a gradual decline with increasing time-steps which clearly affirms the efficiency of online subset selection.

We show in Figure \ref{fig:rhoPRL} the change in objective function value with variation in $\rho$. As we mentioned in Section \ref{sec:subset} that pointwise metric has a very limited impact on Equation \ref{eqn:oldsiftloss} \cite{das2020multi}, we can observe the same in the figure below. We can observe that the gap in objective function values decreases with increase in $\rho$ which marks higher weightage on pairwise metric. However, when the pointwise metric is given the entire weightage ($\rho = 0 $), only 1 representative gets selected from the existing or incoming set, whichever yields the highest value, irrespective of the compression ratio. Thus, this brings out empirically one of the drawbacks of \cite{das2020multi} explained in Section \ref{sec:subset}.

\vspace{-2.7mm}
\begin{figure}[h!]
    \centering
    %\caption{\textbf{Objective function values for proposed function , PRL function and submodular function for (a) Synthetic data (b) CARLA driving data samples}}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/seq_time.pdf}
    % \caption{\textbf{Objective function values for our proposed function on incoming set of CARLA driving data in sequence of time}}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:inctime}
    %\caption{}
    \end{subfigure}
    \hspace{1mm}
    \begin{subfigure}{0.45\columnwidth}
     \centering
     \includegraphics[width=\textwidth,height=2.5cm]{figures/rho_var_MCL.pdf}
    %  \caption{\textbf{Objective function values for our proposed function and PRL function on Synthetic data sample with variation of $\rho$}}
    %\caption{Relative Angle Affordance Distribution}
    \caption{}
    \label{fig:rhoPRL}
    %\caption{}
     \end{subfigure}
     \caption{(a)\textbf{Objective function values for proposed method on CARLA driving data in sequence of time} (b) \textbf{Objective function values for proposed method and \citep{das2020multi} on synthetic data sample with variation of $\rho$.}}
     \label{fig:incrho}
 \end{figure}

% \begin{figure}[h!]
%     \centering
%     \caption{\textbf{Objective function values for our proposed function on incoming set of CARLA driving data in sequence of time}}
%     \includegraphics[width=0.5\columnwidth,height=2.5cm]{figures/seq_time.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:inctime}
% \end{figure}

Next, we discuss the application of the subset selection methods on autonomous driving.

% \begin{figure}[h!]
%     \centering
%     \caption{\textbf{Objective function values for our proposed function and PRL function on Synthetic data sample with variation of $\rho$}}
%     \includegraphics[width=0.5\columnwidth,height=2.5cm]{figures/rho_var_PRL.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:rhoPRL}
% \end{figure}


\subsection{Subset selection on Autonomous Driving}

We use Conditional Affordance Learning model \cite{sauer2018conditional} (CAL) as the driving model to be trained on the dataset we collected using the CARLA \cite{dosovitskiy2017carla} simulator. We train the driving model on NVIDIA Tesla P100 for 50 epochs using Adam Optimizer with learning rate varying between $10^{-3}$ to $10^{-4}$.

We report results with the following methods of selection for two compression ratios 100:20 and 100:7:

\textbf{Whole Set (WS)}: This comprises of the dataset with no reduction.

\textbf{Uniform Skip (US)}: The data is sampled uniformly from the whole dataset, based on the compression ratio.

\textbf{Only SIFT (OS)}: Following Equation \ref{eqn:eq1}, this subset is obtained by selecting images based only on SIFT dissimilarity.

\textbf{Only Loss (OL)}: This subset is obtained by selecting images with highest losses.

\textbf{Multi-Criteria Loss (MCL)}\cite{das2020multi} : The subset is formed by using the multiple-criteria-based subset selection method (Equation \ref{eqn:oldsiftloss}), based on the compression ratio. We used the pairwise criteria (SIFT dissimilarity) and pointwise criteria (loss) as the components of this method.

\textbf{Submodular Bucketwise Multi-task Loss (SBML)}\cite{buchbinder2014submodular} : The subset is obtained by adapting the submodular approach proposed in \cite{buchbinder2014submodular}, in our framework with pairwise (SIFT dissimilarity) and pointwise metric (bucket-wise Relative Angle affordance aided with other multi task losses). 

\textbf{Convex Total Loss (CTL)}: This subset is obtained by adopting our proposed subset selection method (Equation \ref{eqn:newsiftloss}) using SIFT and total loss, based on the compression ratio.

\textbf{Convex Bucketwise Multi-task Loss (CBML)}: This subset is formed by adopting our proposed subset selection method (Equation \ref{eqn:newsiftloss}) using SIFT and bucket-wise Relative Angle affordance aided with other multi task losses, based on the compression ratio.

% \begin{table*}[]
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion}}
% \label{tab:epsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{c|}{Straight}                                                                                                                                               & \multicolumn{3}{c|}{One-Turn}                                                                                                                                             & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set episode completion count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{10}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{10}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SLO/\\ SLN\end{tabular} & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   & \begin{tabular}[c]{@{}l@{}}SIFT/\\ SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   \\ \hline
% 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   \\ \hline
% 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 1                                                       & 88.88                                                   & SLN                                                   & 10                                                      & 0                                                       & SLO                                                   & 1                                                       & 88.88                                                   \\ \hline
% %                                                                              & \multicolumn{12}{c|}{Whole Set test poses completion count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
% %                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{7}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    \\ \hline
% % 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}      & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% % 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 2                                                       & 71.42                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% % 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \scriptsize
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for relative angle affordance prediction}}
% \label{tab:relsumm}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{9}{c|}{Relative Angle buckets}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-10} 
%                                                                              & \multicolumn{3}{c|}{Left-Turn}                                                                                                                                                & \multicolumn{3}{c|}{Straight-Road}                                                                                                                                             & \multicolumn{3}{c|}{Right-Turn}                                                                                                                                               \\ \cline{2-10} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & SIFT                                                  & 0.02                                                        & 11.76                                                   & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.01                                                        & 33.33                                                   & SLN                                                  & 0.01                                                        & 12.5                                                   \\ \hline
% 100:7                                                                        & SIFT                                                  & 0.03                                                        & 16.67                                                   & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.01                                                        & 50.0                                                    & SLN                                                  & 0.01                                                        & 25.0                                                   \\ \hline
% 100:3                                                                        & SLN                                                   & 0.06                                                        & 28.57                                                   & SLO                                                    & 0.02                                                        & 60.0                                                    & SLN                                                   & 0.02                                                        & 25.0                                                    \\ \hline
% \end{tabular}
% \end{table*}
% We use Conditional Affordance Learning model \cite{sauer2018conditional} (CAL) as the driving model to be trained on the dataset we collected using the CARLA \cite{dosovitskiy2017carla} simulator. We train the driving model on NVIDIA Tesla P100 for 50 epochs using Adam Optimizer with learning rate varying between $10^{-3}$ to $10^{-4}$.

 
 \textbf{Subset selection and Training Times}:
%  \tr{write in 2 - 3 sentences how our methods are saving time as well as storage space refering to table \ref{tab:time}}
Table \ref{tab:time} shows the amount of total time taken for training and subset selection for each compression ratio. Compression ratio of 100:20 takes about 1/3rd the total time taken to train the whole set (WS). In terms of storage space, the whole set acquires about 14.5GB of data, which after compression reduces to 2.9GB for compression ratio of 100:20. This follows for the other compression ratio too and hence saves both time and space, essential in the current IoT setting with massively huge data.

 
%  \begin{table}[h]
% \captionsetup{justification=centering}
% \caption{\textbf{Time complexity of proposed methods}}
% \footnotesize
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Compression ratio    & WS  & 100:20 & 100:7 & 100:3 \\ \hline
% Training Time (hours)  & 30 & 8   & 3 & 1.5   \\ \hline
% Subset selection Time (hours) & 0  & 2   & 1.5 & 1   \\ \hline
% Total Time     & 30 & 10   & 4.5 & 2.5   \\ \hline
% \end{tabular}
% \label{tab:time}
% \end{table}

% \begin{table}[h]
% \captionsetup{justification=centering}
% \caption{\textbf{Time complexity of proposed method}}
% \footnotesize
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Compression ratio    & WS  & 100:20 & 100:7\\ \hline
% Training Time (hours)  & 42 & 11   & 7\\ \hline
% Subset selection Time (hours) & 0  & 3   & 1.5\\  \hline
% Total Time     & 42 & 14   & 8.5\\ \hline
% \end{tabular}
% \label{tab:time}
% \end{table}

\begin{table}[]
\caption{\textbf{Time complexity of selection methods}}
\footnotesize
\begin{tabular}{|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}                         & WS                 & \multirow{2}{*}{}                                         & 100:20 & 100:7 \\ \cline{1-2} \cline{4-5} 
\begin{tabular}[c]{@{}l@{}}Training Time\\ (hours)\end{tabular}                     & 42                 &                                                           & 11     & 7     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Subset Selection\\ (hours)\end{tabular}} & \multirow{3}{*}{0} & MCL                                                       & 2      & 1     \\ \cline{3-5} 
                                                                                    &                    & SBML                                                      & 5      & 2.5   \\ \cline{3-5} 
                                                                                    &                    & \begin{tabular}[c]{@{}l@{}}Proposed\\ Method\end{tabular} & 1.5    & 0.75  \\ \hline
\end{tabular}
\label{tab:time}
\end{table}


% \begin{table}[h!]
% \captionsetup{justification=centering}
% \caption{\textbf{Prediction accuracy of speed sign on test set using CAL model trained on whole dataset}}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Affordance & None  & 30kmph & 60kmph & 90kmph\\ \hline
% Speed Sign & 98.99 & 0.0   & 100.0 & 0.0\\ \hline
% \end{tabular}
% \label{speedacc}
% \end{table}

% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions}}
% \label{tab:ep}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 3                                                          & 8        & 2                                                          & 9        & 3                                                          & 9        & 3                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &        &                                                           &         &                                                           &        &                                                           &         &                                                           \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{9}                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{8}                                                          \\ \hline
% \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 2                                                          & 8        & 2                                                          & 9        & 3                                                          & 7        & 3                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 9        & 4                                                          & 9        & 4                                                          & 8        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         &                                                           \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{6}                                                          & 10       & \textbf{6}                                                          & 10       & \textbf{8}                                                          & 10       & \textbf{8}                                                          \\ \hline
% \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 1                                                          & 8        & 0                                                          & 9        & 2                                                          & 8        & 2                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 8        & 0                                                          & 8        & 0                                                          & 8        & 1                                                          & 9        & 0                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         & 0                                                          \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{5}                                                          & 10       & \textbf{5}                                                          & 10       & \textbf{6}                                                          & 9       & \textbf{6}                                                          \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.28                                                                     & 0.02                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.23                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLN                                            & 0.10                                                                     & 0.01                                                                         & 0.04                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.07                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                         \\ \cline{2-8} 
%                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff}
% \end{table*}

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 97.39                                                                     & 97.41                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 96.72                                                                     &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 96.11                                                                     & 96.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 93.49                                                                     & 91.96                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 92.63                                                                     & 91.94                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 89.55                                                                     & 87.23                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                       &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 97.12                                                                     & 97.04                                                                      &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.06                                                                     & 93.09                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 94.16                                                                     & 93.54                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 94.42                                                                      & 93.72                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 99.44                                                                     & 99.72                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.14                                                                     & 99.47                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.11                                                                     & 99.56                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.33                                                                     & 99.66                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.42                                                                     & 97.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.31                                                                     & 98.99                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                       &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.45                                                                     & 98.76                                                                      &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 98.57                                                                     & 97.67                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.29                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.12                                                                      & 98.23                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:hazaff}
% \end{table}
% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|p{12mm}|p{8mm}|l|p{15.5mm}|l|p{15.5mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & MAE           & \%Improvement         & MAE            & \%Improvement           \\ \cline{3-6} 
%                                                                              &                                                        & \multicolumn{2}{l|}{Vehicle Distance} & \multicolumn{2}{l|}{Centerline Distance} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.03          &                       & 0.05           &                         \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.05           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                    &            &                    \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.04          &                   & 0.06           &                    \\ \hline
% \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.06           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.09          &                 & 0.08           &                      \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                  &            &                      \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.07          &                   & 0.06           &                     \\ \hline
% \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.07          &                       & 0.09           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.11          &                  & 0.08           &                     \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                  &            &                      \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.06          &                  & 0.06           &                     \\ \hline
% \end{tabular}
% \end{table}

\textbf{Metrics reported}: We have reported metrics for the two subtasks: episode completion and affordance accuracies. An episode corresponds to a source-destination pair which is provided to the agent vehicle prior to running the simulator. The episode completion is measured in terms of the number of successfully completed episodes. The accuracies of discrete affordances are measured in terms of the standard metrics - Micro and Macro Accuracy, while the continuous affordances are measured in terms of Mean Absolute Error (MAE). 

\textbf{Affordance Selection}: We have reported results for five affordances - \textit{Red light}, \textit{Hazard Stop}, \textit{Relative Angle}, \textit{Centerline Distance} and \textit{Vehicle Distance}. Considering the setup of our dataset collection, from Figure \ref{fig:distrib}, we can observe that the two affordances \textit{Speed Sign} and \textit{Hazard Stop} suffer from class imbalance.

In case of Speed Sign, only 1.5\% of the entire data belongs to other classes of speed signs (0.7\% 30kmph, 0.4\% 60kmph and 0.3\% 90kmph), and are hence predicted incorrectly by the driving model trained on the whole dataset. The predicted accuracies of each class from the test set are as follows: 98.99\% for \textit{None}, 0.0\% for \textit{30kmph}, 100.0\% for \textit{60kmph} and 0.0\% for \textit{90kmph}. Owing to this reason, we refrain from reporting accuracies on this affordance. Alongside, prediction accuracy of this affordance does not have an impact on episode completion.


% Table \ref{speedacc} shows the predicted accuracies of each class from the test set which comprises of 0.4\% 30kmph , 0.2\% 60kmph, 0.04\% as 90kmph and the remaining as \textit{None}. 

\textbf{Multi-task criteria}: Autonomous vehicles need a high level of understanding of the environment it needs to interact with. There are multiple criteria/tasks to be considered while reaching a destination or in other words, completing an episode. Conditional Affordance Learning \citep{sauer2018conditional} has considered six of such tasks or affordances in its driving model. The affordance \textit{Relative Angle} is the orientation of the car with respect to the road and decides the steer value of the agent vehicle. Hence, this affordance becomes critical in episode completion. However, we notice a large skew in the distribution of affordances in Figure \ref{fig:distrib}b which essentially portrays the importance of selection of instances from the minority buckets (turn buckets) for the end-task of driving. There is also no established end-to-end connection between the selection of affordances and a successful episode. Therefore, this comes out as a challenge in selecting affordances for a chosen subset which will be significant in episode completion.

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{left}) 100:20 , (\textit{middle}) 100:7, (\textit{right}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure*}

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
    
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_20.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_20.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redllight_15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turn_15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_3.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_3.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7, (\textit{bottom}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure}

% In case of Hazard Stop, only 0.5 \% of data has presence of hazard stops, while test set has none. Overall, all the methods are able to predict the majority class (i.e no hazard stop) leading to an accuracy close to 100\%. In order to avoid the trivial case, we exclude this affordance from our results.



% \tr{Speed sign: Only about 1\% (0.5\% 30kmph, 0.1\% 60kmph and 0.3\% 90kmph) of the data belongs to other speed signs which are all predicted wrongly by the CAL model even with full dataset. Prediction accuracy of this affordance also does not affect episode completion. (give classwise accuracy and number of data points.) \\
% Hazard stop: The data has extreme skew only 0.6\% of the training data has hazard stop as true and there are no test instances with this.\\}
% \subsection{Comparison of data gradation methods with Whole Set}

% In this section, we provide a summary of results enlisting the best method from the two sets of experiments that we perform while comparing selection methods with whole set - episode completion and affordance prediction. 

% We consider four tasks under episode completion which had been originally defined in \cite{dosovitskiy2017carla}:
% \begin{enumerate}
%     \item Straight : The episode comprises of points which is a straight road.
%     \item One-Turn : The episode comprises of points which include a left or right turn in its path.
%     \item Straight Dynamic : It is similar to Straight task in the presence of other vehicles and pedestrians.
%     \item One-Turn Dynamic : It is similar to One-Turn task in the presence of other vehicles and pedestrians.
% \end{enumerate}

% In table \ref{tab:epsumm}, we show the best performing method for each task under episode completion along with the number of successfully completed episodes and its difference with that of the whole set. We can observe that the method SLN completes the most number of episodes (out of a total of 10 episodes) among all other gradation methods. It fails for only 33\% episodes in the difficult task of taking turns. The detailed results on episode completion is explained in the next subsection.




% \begin{table*}[]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in training conditions}}
% \label{tab:trainepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{l|}{Straight}                                                                                                                                               & \multicolumn{3}{l|}{One-Turn}                                                                                                                                             & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set Episode Completion Count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{9}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{9}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SLO/\\ SLN\end{tabular} & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   & \begin{tabular}[c]{@{}l@{}}SIFT/\\ SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   \\ \hline
% 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   \\ \hline
% 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 1                                                       & 88.88                                                   & SLN                                                   & 10                                                      & 0                                                       & SLO                                                   & 1                                                       & 88.88                                                   \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in testing conditions}\tr{Combine this with the training table}}
% \label{tab:testepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{l|}{Straight}                                                                                                                                             & \multicolumn{3}{l|}{One-Turn}                                                                                                                                             & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set Episode Completion Count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   & \begin{tabular}[c]{@{}l@{}}SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% 100:7                                                                        & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 2                                                       & 71.42                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% 100:3                                                                        & SLN                                                   & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLN\end{tabular}    & 1                                                       & 85.71                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   \\ \hline
% \end{tabular}
% \end{table*}

% In table \ref{tab:relsumm}, we show the best method for each compression ratio under the respective relative angle buckets along with its difference with that of whole set.  We explicitly focus on the relative angle affordance since it is a key factor in episode completion. We can observe that SLN turns out as the best performing method for the turn buckets while Uniform Skip turns out the best for Straight road. This can be attributed to the observation we made where SLN turned out as the best method in episode completion task. We have given a detailed analysis on the affordance predictions in the next subsections.




% \begin{table*}[]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in training conditions}}
% \label{tab:trainepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{9}{|c|}{Episode Completion Tasks}                                                                                                                                                                                                                                                                                                                                  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{2}{c|}{Straight}                                                        & \multicolumn{2}{c|}{One-Turn}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Straight \\ Dynamic\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}} \\ \cline{2-9} 
%                                                                              & Best Method                                                             & Difference & Best Method             & Difference & Best Method                                & Difference                          & Best Method                             & Difference                            \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SIFT+Loss-O/\\ SIFT+Loss-N\end{tabular} & 0          & SIFT+Loss-N             & 3          & SIFT/SIFT+Loss-N                           & 0                                   & SIFT+Loss-N                             & 3                                     \\ \hline
% 100:7                                                                        & SIFT+Loss-N                                                             & 0          & SIFT+Loss-N             & 6          & SIFT+Loss-N                                & 0                                   & SIFT+Loss-N                             & 6                                     \\ \hline
% 100:3                                                                        & SIFT+Loss-N                                                             & 0          & SIFT+Loss-O/SIFT+Loss-N & 8          & SIFT+Loss-N                                & 0                                   & SIFT+Loss-O                             & 8                                     \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in testing conditions}}
% \label{tab:testepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{9}{|c|}{Episode Completion Tasks}                                                                                                                                                                                                                                                                                                                             \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{2}{c|}{Straight}                                                   & \multicolumn{2}{c|}{One-Turn}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Straight \\ Dynamic\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}} \\ \cline{2-9} 
%                                                                              & Best Method                                                        & Difference & Best Method             & Difference & Best Method                             & Difference                             & Best Method                             & Difference                            \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT+Loss-O/\\ SIFT+Loss-N\end{tabular} & 0          & SIFT+Loss-N             & 4          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 4                                     \\ \hline
% 100:7                                                                        & SIFT+Loss-N                                                        & 0          & SIFT+Loss-N             & 5          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 5                                     \\ \hline
% 100:3                                                                        & SIFT+Loss-N                                                        & 0          & SIFT+Loss-O/SIFT+Loss-N & 6          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 6                                     \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \label{tab:relsumm}
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for relative angle affordance prediction}}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{6}{c|}{Relative Angle buckets}                                                                                                                                                                                                                                                                                                                     \\ \cline{2-7} 
%                                                                              & \multicolumn{2}{c|}{Left-Turn}                                                                                      & \multicolumn{2}{c|}{Straight-Road}                                                                                  & \multicolumn{2}{c|}{Right-Turn}                                                                                     \\ \cline{2-7} 
%                                                                              & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} \\ \hline
% 100:20                                                                       & SIFT                             & 0.02                                                                             & Uniform Skip                     & 0.01                                                                             & SIFT+Loss-N                      & 0.01                                                                             \\ \hline
% 100:7                                                                        & SIFT                             & 0.03                                                                             & Uniform Skip                     & 0.01                                                                             & SIFT+Loss-N                      & 0.01                                                                             \\ \hline
% 100:3                                                                        & SIFT+Loss-N                      & 0.06                                                                             & SIFT+Loss-O                      & 0.02                                                                             & SIFT+Loss-N                      & 0.02                                                                             \\ \hline
% \end{tabular}
% \end{table*}
% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:20 compression ratio}}
% \label{tab:ep5}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 3                                                          & 8        & 3                                                          & 9        & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
%                                                                              & Only SIFT                                                   & 10       & 7                                                          & 10       & 7                                                          & 10       & 7                                                          & 9        & 6                                                          \\ \cline{2-10} 
%                                                                             & Only Loss                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & PRL                                                    & 9        &  8                                                         & 9        & 8                                                          & 7       &  7                                                         & 7        & 7                                                          \\ \cline{2-10} 
%                                                     & SubM                                                    & 9        &  7                                                         & 9        & 7                                                          & 9       &  7                                                         & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & STL                                                    & 10       & 8                                                         & 10       & 7                                                          & 10       & 9                                                          & 10       & 9 
%                                 \\ \cline{2-10} 
%                                                                              & SML                                                    & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       &\textbf{10}                                \\        \hline
% % \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 2                                                          & 8        & 2                                                          & 9        & 3                                                          & 7        & 3                                                          \\ \cline{2-10} 
% %                                                                              & SIFT                                                   & 9        & 4                                                          & 9        & 4                                                          & 8        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
% %                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         &                                                           \\ \cline{2-10} 
% %                                                                              & SLN                                                    & 10       & \textbf{6}                                                          & 10       & \textbf{6}                                                          & 10       & \textbf{8}                                                          & 10       & \textbf{8}                                                          \\ \hline
% % \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 1                                                          & 8        & 0                                                          & 9        & 2                                                          & 8        & 2                                                          \\ \cline{2-10} 
% %                                                                              & SIFT                                                   & 8        & 0                                                          & 8        & 0                                                          & 8        & 1                                                          & 9        & 0                                                          \\ \cline{2-10} 
% %                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         & 0                                                          \\ \cline{2-10} 
% %                                                                              & SLN                                                    & 10       & \textbf{5}                                                          & 10       & \textbf{5}                                                          & 10       & \textbf{6}                                                          & 9       & \textbf{6}                                                          \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:7 compression ratio}}
% \label{tab:ep15}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:7}                                                      & \begin{tabular}[c]{@{}l@{}}Only SIFT\end{tabular} & 9        & 5                                                          & 9        & 5                                                           & 9        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
%                                                                             & Only Loss                                                   & 10        & 6                                                          & 10       & 6                                                          &    9    & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & PRL                                                    & 9        & 5                                                            & 9        & 5                                                          & 7        &  4                                                         & 7        & 4                                                          \\ \cline{2-10}
%                                                                              & SubM                                                    & 9        & 3                                                            & 9        & 3                                                          & 9        & 2                                                          & 9        & 2                                                          \\ \cline{2-10}
%                                                                              & STL                                                    & 10       & 7                                                          & 10        & 7                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}  
%                                 \\ \cline{2-10} 
%                                                                              & SML                                                    & 10       & \textbf{8}                                                           & 10       & \textbf{8}                                                          & 10       &\textbf{9}                                                           & 10       & \textbf{9}                                 \\        \hline
% \end{tabular}
% \end{table*}

\begin{table*}[]
%\footnotesize
\scriptsize
\centering
\captionsetup{justification=centering}
\caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:20 and 100:7 compression ratio}}
\label{tab:ep5_15}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
                                                                             &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
                                                                             & WS    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
\multirow{4}{*}{100:20}                                                      & US & 9        & 3                                                          & 8        & 3                                                          & 9        & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
                                                                             & OS                                                   & 10       & 7                                                          & 10       & 7                                                          & 10       & 7                                                          & 9        & 6                                                          \\ \cline{2-10} 
                                                                            & OL                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
                                                                             & MCL                                                    & 9        &  8                                                         & 9        & 8                                                          & 7       &  7                                                         & 7        & 7                                                          \\ \cline{2-10} 
                                                    & SBML                                                    & 9        &  7                                                         & 9        & 7                                                          & 9       &  7                                                         & 9        & 7                                                          \\ \cline{2-10} 
                                                                             & CTL                                                    & 10       & 8                                                         & 10       & 7                                                          & 10       & 9                                                          & 10       & 9 
                                \\ \cline{2-10} 
                                                                             & CBML                                                    & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       &\textbf{10}                                \\        \hline
                                                        \hline
\multirow{4}{*}{100:7}                                                      & \begin{tabular}[c]{@{}l@{}}MCL\end{tabular} & 9        & 5                                                            & 9        & 5                                                          & 7        &  4                                                         & 7        & 4                                                          \\ \cline{2-10}
                                                                             & SBML                                                    & 9        & 3                                                            & 9        & 3                                                          & 9        & 2                                                          & 9        & 2                                                          \\ \cline{2-10}
                                                                             & CTL                                                    & 10       & 7                                                          & 10        & 7                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}  
                                \\ \cline{2-10} 
                                                                             & CBML                                                    & 10       & \textbf{8}                                                           & 10       & \textbf{8}                                                          & 10       &\textbf{9}                                                           & 10       & \textbf{9}                                 \\        \hline                                                    
\end{tabular}
\end{table*}



\subsection{Comparison of Methods: Episode Completion}



In this section, we will study the performance of different subset selection techniques on the basis of episode completion which is the main intended objective.

We consider four tasks under episode completion which had been originally defined in \cite{dosovitskiy2017carla}:
\begin{enumerate}
    \item Straight : The episode comprises of pairs of points which are straight roads.
    \item One-Turn : The episode comprises of pairs of points which include left or right turn in their paths.
    \item Straight Dynamic : Similar to \textit{Straight} task, it occurs in the presence of other vehicles and pedestrians.
    \item One-Turn Dynamic : Similar to \textit{One-Turn} task in the presence of other vehicles and pedestrians.
\end{enumerate}

We show in Table \ref{tab:ep5_15} the performance of driving model trained on subsets, obtained by different subset selection techniques, by simulating it with the CARLA \citep{dosovitskiy2017carla} simulator.


We report number of successfully completed episodes (out of a total of 10 episodes) for each subtask in training and test conditions. We observe that the tasks - \textit{Straight} and \textit{Straight Dynamic} are fairly easy to accomplish for all subset selection methods. The challenge arises in the other two tasks where we see a large number of unsuccessful episodes.

The completion of episodes in turns, largely depends on the affordance \textit{Relative Angle} which as we mentioned before, provides the steering angle of the agent vehicle. We observe that Uniform Skip (US) is unable to complete majority of the turns in training or test conditions. This is due to the inherent nature of selection of US method, which does not take the important frame sequences into consideration.

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/relangle_episode.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/relloss_episode.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{A temporal plot of an episode with (a) the relative angle affordance value (b) its corresponding relative angle loss values in the respective frames.}}
%     \label{fig:lossrel}
% \end{figure}
%\vspace{-1mm}
\begin{figure*}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/deviation_dist_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/deviation_episode_MCL_whole.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \caption{}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/deviation_episode_error_MCL_whole.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_MCL.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{Anecdotal example of a sample episode showing (a) the region of failure by MCL (b) the corresponding errors and (c) fraction of selected instances from those regions. CBML selects more fraction of instances from regions important for episode completion.}}
    \label{fig:deviate}
\end{figure*}
% One of the 

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
    
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_20.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_20.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redllight_15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turn_15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_3.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_3.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7, (\textit{bottom}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure}

On the other hand, OS, OL, MCL, SBML complete some of the turn episodes, with CBML completing the highest of all methods (100\% both in training and test conditions) followed by CTL. This is due to the consideration of pointwise metric - bucketwise relative angle aided with remaining multi task losses in Equation \ref{eqn:newsiftloss} along with pairwise metric SIFT dissimilarity, which leads to the selection of important frames. We also report the episode completion numbers for 100:7 compression ratio in Table \ref{tab:ep5_15}, for two baselines - MCL and SBML and the proposed method. We can observe that CTL and CBML continue to perform better compared to the other baselines with CBML completing 80\% and 90\% episodes in training and test conditions even after dropping 93\% of the frames.

% As mentioned under Multi-task criteria, we observe that Relative Angle affordance turns out to be vital in the task of episode completion. We can divide the entire range of Relative Angle affordance value across 20 buckets ranging from -1.0 to +1.0. Note that buckets corresponding to (-1.0 to -0.1) and (0.1 to 1.0) approximately indicate the left and right turns. 

% In Figure \ref{fig:lossrel}, we show an entire sequence of frames of an episode with its corresponding \textit{Relative Angle} affordance value and its respective loss value.  As seen from the figure, which is one of the left turn episodes, we can notice the higher relative angle loss values at the turn. This essentially shows us the need for selection of such frames in order to have successful episodes. So, using the above intuition, we fine-tune the weights corresponding to the bucket-wise relative angle loss values and feed in our subset selection framework SML.


% One of the possible reasons of success can be attributed to Figure \ref{fig:bucketprop5} where we see that SML has a higher fraction of selected instances for most of the buckets than all other methods which essentially portrays its effectiveness. Only Loss also selects fairly large fraction of instances for some of the buckets. However, it only concentrates on the frames which incur a high loss value. The completion of an episode relies on various other factors like perceptual difference and having only frames with high end-task losses in the compressed sequence does not lead to an effective result.


We show an anecdotal example of a failed episode from MCL \citep{das2020multi} method in Figure \ref{fig:deviate} and try to analyse the reason behind it. In Figure \ref{fig:deviate}a, we show a plot of an episode with distance covered vs Relative Angle affordance. The cumulative distance is chosen as an axis of reference in order to make the comparison spatially similar for all the methods. Overall, the agent vehicle in the simulator is resilient to errors. However, we can observe the gradual deviation of MCL \citep{das2020multi} method and its accumulated errors which lead to an incomplete episode. We can also relate the region of failures to the corresponding relative angle errors in Figure \ref{fig:deviate}b where we observe that overall, MCL \citep{das2020multi} is having a higher error compared to proposed method CBML and model trained on the whole set. This occurs because we fine-tune the weights corresponding to the bucket-wise relative angle loss values and feed in our subset selection framework CBML along with pairwise metric. We also show the fraction of selected instances by both the selection methods, in Figure \ref{fig:deviate}c from the same region, and we can observe that CBML selects more fraction of instances in the area right before the turn and during the turn, which eventually help in its completion.

We discuss the next subtask - affordance prediction in the following subsection.

\begin{figure}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_left_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_left_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_straight_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_straight_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_right_15.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_right_plot_15.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{(a) Fraction of selected instances and (b) Mean Absolute Error (MAE) for Relative Angle affordance for all subset selection methods. Selection of more fraction of instances in turn buckets lead to lower MAE in CBML for 100:20 compression ratio.}}
    \label{fig:fracmae_100_20}
\end{figure}

\begin{figure}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_left_100_7_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_left_100_7_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_straight_100_7_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_straight_100_7_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_right_100_7_15.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_right_100_7_plot_15.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{(a) Fraction of selected instances and (b) Mean Absolute Error (MAE) for Relative Angle affordance for two baselines (MCL and SBML) and the proposed methods. Selection of more fraction of instances in turns lead to lower MAE in CBML for 100:7 compression ratio.}}
    \label{fig:fracmae_100_7}
\end{figure}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_left.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_straight.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_right.pdf}
    
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for subset selection methods for 100:20 compression ratio}}
%     \label{fig:fracall}
% \end{figure*}


% We show in Figure \ref{fig:deviate} three instances of the points of deviation where three of the baselines - Only SIFT, Only Loss and PRL fail in completing their respective episodes. The buckets correspond to the areas in the town where the models trained using Only SIFT, Only Loss and PRL had deviated leading to incomplete episode. We can clearly observe that the error corresponding to SML and STL are considerably lower which make them reach the end goal.

% We show in Figure \ref{fig:deviate} three instances of the points of deviation where three of the baselines - Only SIFT, Only Loss and PRL fail in completing their respective episodes. We have run the simulator using the ground truth affordances and the individual trained model's predicted affordances. We kept a track of the predicted relative angle along with the covered cumulative distance. Note that the change in relative angle values (y-axis) arise when turns appear. We can observe in both the plots, that the agent vehicle started deviating more using the Only Loss and PRL method right before turns, leading to intersection with the sidewalk thus failing to complete the episode.  The points immediately before the turn are important for consideration since those mark the intersecting points or junctions. We can see in both the plots that our gradation method - STL and SML appear to predict values closer to the ground truth during the intersection points while Only Loss (left) and PRL (right) methods  begin deviating at the intersections leading to failures. The loss values in these buckets (-0.1 to 0.1) are not considerably higher due to presence of large number of training samples in these buckets since the relative angle values for the straight roads also fall in them. Hence, Only Loss selects lesser number of instances from these buckets leading to failure.  On the other side, PRL takes SIFT and Loss into consideration, but due to its drawback as described in section, it also fails in completing all the turns. Both SML and STL take pairwise and pointwise metric into consideration during selection of frames and result in more successful episodes. SML performs better than STL due to the inclusion of SIFT and weighted losses which help in selection of more important frames. 
% A wrong prediction in relative angle at certain points may take the vehicle to waypoints from which recovering back without manual intervention would not be possible.
% STL even though predicts closer to ground truth values than SML at the junctions, yet it is not able to complete all the episodes since the turns after the intersection is vital too and we can observe in the plots that STL predicts better at those.
% It can also be seen that the number of successfully completed episodes with STL is considerably less than SML but reasonably better than the other methods. The consideration of both pairwise and pointwise metric (total loss) lead to its better selection of frames, however the weighted multi-task loss has led to an added benefit.
% Note that 100:7 and 100:3 is very high in comparison to the 63000 frames dataset we collected. The original model \cite{sauer2018conditional} was trained on 10x amount of data we have used in our experiments. We expect that the successful completion rate will increase with increasing dataset size.

% We have also performed experiments on the subset selection method using only relative angle loss as the pointwise metric, to which it did not yield good results. One potential future work can be to use different components of the six affordance losses and weighing them according to its importance in episode completion. 

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 97.39                                                                     & 97.41                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 96.72                                                                     & 97.03                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & Only SIFT                                                   & 96.11                                                                     & 96.07                                                                     &                                                          &                                                          \\ \cline{2-6}
%                         & Only Loss                                                   & 92.31                                                                     & 91.08                                                                     &                                                          &                                                          \\ \cline{2-6}
%                         & PRL                                            &  91.63                                                                    & 89.73                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & STL                                            & 96.38                                                                     & 96.05                                                                     &                                                          &
%                       \\ \cline{2-6} 
%                         & SML                                            & 93.98                                                                     & 92.83                                                                     &                                                          &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 92.63                                                                     & 91.94                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 89.55                                                                     & 87.23                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 94.72                                                                      & 94.54                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 97.12                                                                     & 97.04                                                                      &                                                          &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.06                                                                     & 93.09                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 94.16                                                                     & 93.54                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 90.12                                                                     & 94.41                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 94.42                                                                      & 93.72                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \label{tab:redlaff}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Method                                              & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                             & WS                                                  & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                     & US                                                  & 96.72                                                    & 97.03                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 96.11                                                    & 96.07                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 92.31                                                    & 91.08                                                    \\ \cline{2-4} 
%                                                             & PRL                                                 & 91.63                                                    & 89.73                                                    \\ \cline{2-4} 
%                                                             & STL                                                 & 96.38                                                    & 96.05                                                    \\ \cline{2-4} 
%                                                             & SML                                                 & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \label{tab:hazaff}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Method                                              & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                             & WS                                                  & 99.44                                                    & 99.72                                                    \\ \hline
% \multirow{6}{*}{100:20}                                     & US                                                  & 99.14                                                    & 99.47                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     \\ \cline{2-4} 
%                                                             & PRL                                                 & 99.43                                                    & 98.39                                                    \\ \cline{2-4} 
%                                                             & STL                                                 & 99.31                                                    & 99.61                                                    \\ \cline{2-4} 
%                                                             & SML                                                 & 99.45                                                    & 99.71                                                    \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
% \label{tab:redrhazaff}
% \begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                                              & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
%                                                                              & PRL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
%                         & SubM                                                 & 99.25                                                    &                                                     & 94.33                                                    &                                                     \\ \cline{2-6}                                                     & STL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
%                                                                              & SML                                                 & 99.45                                                    & \begin{tabular}[c]{@{}l@{}}99.71\\ (1.32\%)\end{tabular}                                           & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{table}




% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 99.44                                                                     & 99.72                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.14                                                                     & 99.47                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & Only SIFT                                                   & 99.11                                                                     & 99.56                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & Only Loss                                                   & 99.41                                                                     & 99.6                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & PRL                                            & 99.43                                                                     & 98.39                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLT                                            & 99.23                                                                     & 99.61                                                                     &                                                          &
%                         \\ \cline{2-6} 
%                         & SLM                                            & \textbf{99.45}                                                                     & \textbf{99.71}                                                                     &                                                          &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.42                                                                     & 97.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 99.31                                                                     & 98.99                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 99.39                                                                      & 98.37                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 99.45                                                                     & 98.76                                                                      &                                                          &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 98.57                                                                     & 97.67                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 99.29                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 99.39                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 99.12                                                                      & 98.23                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:hazaff}
% \end{table}
% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|p{12mm}|p{8mm}|l|p{15.5mm}|l|p{15.5mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & MAE           & \%Improvement         & MAE            & \%Improvement           \\ \cline{3-6} 
%                                                                              &                                                        & \multicolumn{2}{l|}{Vehicle Distance} & \multicolumn{2}{l|}{Centerline Distance} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.03          &                       & 0.05           &                         \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.05           &                         \\ \cline{2-6} 
%                                                                              & Only SIFT                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6}
%                                                                              & Only Loss                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6}
%                                                                              & PRL                                                    & 0.05          &                   & 0.06           &                    \\ \cline{2-6} 
%                                                                              & SLT                                                    & 0.05          & 44.44                  & 0.05           & 37.5
%                                           \\ \cline{2-6} 
%                                                                              & SLM                                                    & \textbf{0.04}          &    55.55               & 0.05           & 37.5                                  
%                                                                              \\ \hline
% % \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.06           &                         \\ \cline{2-6} 
% %                                                                              & SIFT                                                   & 0.09          &                 & 0.08           &                      \\ \cline{2-6} 
% %                                                                              & SLO                                                    & 0.09          & 0.09                 &            &                      \\ \cline{2-6} 
% %                                                                              & SLN                                                    & 0.07          &                   & 0.06           &                     \\ \hline
% % \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.07          &                       & 0.09           &                         \\ \cline{2-6} 
% %                                                                              & SIFT                                                   & 0.11          &                  & 0.08           &                     \\ \cline{2-6} 
% %                                                                              & SLO                                                    & 0.09          & 0.09                 &            &                      \\ \cline{2-6} 
% %                                                                              & SLN                                                    & 0.06          &                  & 0.06           &                     \\ \hline
% \end{tabular}
% \end{table}




%\tr{TBD}

% \begin{table}[]
% \begin{tabular}{|l|p{2mm}|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ratio\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\\ (Macro)\end{tabular}}                   & \multicolumn{4}{c|}{MAE}                                                                                                                                                                                \\ \cline{3-8} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}CAL\\ RL\end{tabular}        & \begin{tabular}[c]{@{}l@{}}TS\\ RL\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ CD\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ CD\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                       &                                                                              & \begin{tabular}[c]{@{}l@{}}95.86\\ (95.16)\end{tabular} & \begin{tabular}[c]{@{}l@{}}95.86\\ (95.16)\end{tabular}                                               &\begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05 \end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                                 & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                                \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:20}}                                 &
% \begin{tabular}[c]{@{}l@{}}95.32\\ (94.7)\end{tabular} & \begin{tabular}[c]{@{}l@{}}95.54\\ (94.82)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.06\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}91.36\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                &                                                  &                                                &                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}89.18\\ (87.25)\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}}90.52 \\(88.26)\end{tabular}                                                & 0.07                                                 & 0.06                                                & 0.09                                                 & 0.10                                                \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:7}}                                 & \begin{tabular}[c]{@{}l@{}}91.94 \\ (91.08)\end{tabular} & \begin{tabular}[c]{@{}l@{}}94.58\\ (95.02)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.10\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8}
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}90.28\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 

% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}89.7\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.08                                                 &                                                 & 0.11                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}85.76\\ (83.67)\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.07                                                 &                                                 & 0.11                                                &                                                 \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:3}}                                 & \begin{tabular}[c]{@{}l@{}} 91.72\\ (91.27)\end{tabular} & \begin{tabular}[c]{@{}l@{}}93.58\\ (92.60)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}} 0.06\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}} 0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8}
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}90.04\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.10\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}87.68\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.08                                                 &                                                 & 0.12                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                &                                                  &                                                 &                                                 &                                                 \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques in terms of affordance accuracies}
% \label{afftable}
% \end{table}

% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.15                                                      & 0.02                                                          & 0.08                                                       & 0.09                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                              & 0.08                                                           & 0.07                                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 95.32                                                    & 94.7                                                     & 0.39                                                      & 0.03                                                          & 0.09                                                       & 0.09                                                          & 95.54                                                    & 94.82                                                    & 0.28                                                          & 0.03                                                              & 0.07                                                           & 0.09                                                          \\ \hline
% SIFT                                                                               & 91.36                                                    & 88.12                                                         & 0.17                                                      & 0.06                                                          & 0.09                                                       & 0.09                                                          & 91.9                                                         & 90.75                                                         & 0.16                                                          & 0.05                                                              & 0.14                                                           & 0.09                                                              \\ \hline
% SIFT+Loss-O                                                                        & 88.34                                                         & 86.96                                                         & 0.19                                                      & 0.07                                                          & 0.08                                                       & 0.09                                                              & 89.94                                                         & 87.79                                                         & 0.17                                                          & 0.04                                                              & 0.08                                                           & 0.08                                                              \\ \hline
% SIFT+Loss-N                                                                        & 89.18                                                    & 88.25                                                    & 0.18                                                      & 0.05                                                          & 0.07                                                       & 0.09                                                          & 90.52                                                    & 89.26                                                    & 0.16                                                          & 0.05                                                              & 0.08                                                           & 0.08                                                          \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:20}
% \label{afftable1}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.19                                                      & 0.03                                                          & 0.08                                                       & 0.08                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                              & 0.08                                                           & 0.07                                                               \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 91.94                                                    & 91.08                                                     & 0.38                                                      & 0.04                                                          & 0.11                                                       & 0.11                                                          & 94.58                                                    & 95.02                                                    & 0.27                                                          & 0.04                                                              & 0.09                                                           & 0.10                                                          \\ \hline
% SIFT                                                                               & 90.28                                                    & 90.1                                                         & 0.18                                                     & 0.06                                                          & 0.14                                                       & 0.11                                                          & 90.1                                                         & 88.58                                                         & 0.17                                                           & 0.05                                                              & 0.16                                                           & 0.09                                                              \\ \hline
% SIFT+Loss-O                                                                        & 89.7                                                         & 89.8                                                         & 0.19                                                      & 0.05                                                          & 0.13                                                       &  0.11                                                             & 91.76                                                         & 91.4                                                         & 0.21                                                          & 0.05                                                              & 0.11                                                           & 0.11                                                              \\ \hline
% SIFT+Loss-N                                                                        & 87.04                                                    &                                                     & 0.21                                                      & 0.10                                                          & 0.06                                                       & 0.12                                                          & 91.32                                                    &                                                     & 0.19                                                          & 0.08                                                              & 0.06                                                           & 0.14                                                          \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:7}
% \label{afftable2}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.19                                                      & 0.03                                                          & 0.08                                                       & 0.08                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                               & 0.08                                                           & 0.07                                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 91.26                                                    & 90.36                                                      & 0.44                                                      & 0.6                                                          & 0.15                                                       & 0.11                                                          & 93.58                                                    & 92.60                                                    & 0.32                                                          & 0.05                                                              & 0.09                                                           & 0.11                                                          \\ \hline
% SIFT                                                                               & 90.04                                                    & 90.34                                                         & 0.32                                                     & 0.06                                                          & 0.15                                                       & 0.11                                                          & 91.87                                                         & 89.02                                                         & 0.28                                                          & 0.05                                                              & 0.14                                                           &  0.09                                                             \\ \hline
% SIFT+Loss-O                                                                        & 87.68                                                         & 88.54                                                         & 0.26                                                      & 0.05                                                          & 0.16                                                       & 0.11                                                              & 91.36                                                         & 90.78                                                         & 0.23                                                          & 0.07                                                              & 0.11                                                           & 0.13                                                              \\ \hline
% SIFT+Loss-N                                                                        & 86.08                                                    & 85.54                                                    & 0.22                                                      & 0.08                                                          & 0.06                                                       & 0.13                                                          &                                                     &                                                     &                                                           &                                                               &                                                            &                                                           \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:3}
% \label{afftable3}
% \end{table*}




% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ratio\end{tabular}} & \multirow{2}{*}{Tasks}                                     & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Train\\ Poses\end{tabular}}                               & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Poses\end{tabular}}                                \\ \cline{4-7} 
%                                                                           &                                                                              &                                                            & \begin{tabular}[c]{@{}l@{}}CAL\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ Model\end{tabular} \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}}      & \multirow{4}{*}{}                                                            & Straight                                                   & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 9                                                    &                                                    & 7                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 8                                                    &                                                    & 7                                                    &                                                    \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:20}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 0                                                    & 0                                                   & 1                                                    & 0                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &  8                                                   & 9                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 0                                                    & 0                                                   & 1                                                    & 0                                                   \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 2                                                    &                                                    & 1                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    &                                                    & 9                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 2                                                    &                                                    & 1                                                    &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &  10                                                   & 9                                                   & 10                                                    & 9                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 9                                                   & 9                                                    & 8                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   & 10                                                    & 10                                                   & 10                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 6                                                    &                                                    & 3                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    & 10                                                   & 10                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 6                                                    &                                                    & 3                                                    &                                                    \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:7}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 10                                                   & 7                                                     & 10                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\
                                    
%                                 \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:3}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 9                                                   & 8                                                    & 9                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
                                                                          
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\
%                                     \hline
% \end{tabular}
% \label{eptable}
% \end{table}





% \begin{table*}[h!]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training conditions}}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Episodes}                             \\ \cline{3-6} 
%                                                                              &                          & Straight & One-Turn & Straight Dynamic & One-Turn Dynamic \\ \hline
%                                                                              & Whole Set                & 10       & 9        & 10               & 9                \\ \hline
% \multirow{4}{*}{100:20}                                                      & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 10       & 2        & 10               & 2                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 10       & 3        & 8                & 2                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 6        & 10               & 6                \\ \hline
% \multirow{4}{*}{100:7}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 9        & 2        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 2        & 9                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 3        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:3}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8         & 1        & 8                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 8                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10         & 1         & 10                 & 0                 \\ \hline
% \end{tabular}
% \label{tab:eptabletrain}
% \end{table*}


% \begin{table*}[h!]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in test conditions}}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Episodes}                             \\ \cline{3-6} 
%                                                                              &                          & Straight & One-Turn & Straight Dynamic & One-Turn Dynamic \\ \hline
%                                                                              & Whole Set                & 10       & 7        & 10               & 7                \\ \hline
% \multirow{4}{*}{100:20}                                                      & Uniform Skip             & 9        & 1        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT                     & 10       & 1        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 10       & 2        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 3        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:7}                                                       & Uniform Skip             & 9        & 0        & 7                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8        & 1        & 8                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 9                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 2        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:3}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8         & 1        & 7                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 8                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10         & 1         & 10                 & 1                 \\ \hline
% \end{tabular}
% \label{tab:eptabletest}
% \end{table*}


\begin{table*}
\noindent\scriptsize
\begin{minipage}[b]{0.4\linewidth}
    \centering
\caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
\label{tab:redrhazaff}
\begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
                                                                             &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
                                                                             & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
\multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
                                                                             & OS & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
                                                                             & OL & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
                                                                             & MCL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
                        & SBML                                                 & 99.25                                                    & 99.60                                                    & 94.33                                                    & 93.91                                                    \\ \cline{2-6}                                                     & CTL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
                                                                             & CBML                                                 & 99.45                                                    & 99.71                                            & 93.98                                                    & 92.83                                                    \\ \hline
\end{tabular}
\end{minipage}
\hspace{2cm}
\begin{minipage}[b]{0.4\linewidth}
\caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
\label{tab:vehcen}
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
                                                                             &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
\multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
                                                                             & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
                                                                             & OS & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
                                                                             & OL & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
                                                                             & MCL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                                                    & SBML                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
                                                                            & CTL                                                 & 0.05
                                                                 &0.05                                 \\ \cline{2-4} 
                                                                             & CBML                                                 & 0.04
                                                                 &0.05                                 \\ \hline
\end{tabular}
\end{minipage}
\end{table*}


\subsection{Comparison of Methods: Affordance Accuracies}

% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
% \label{tab:redrhazaff}
% \begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                                              & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
%                                                                              & PRL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
%                         & SubM                                                 & 99.25                                                    & 99.60                                                    & 94.33                                                    & 93.91                                                    \\ \cline{2-6}                                                     & STL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
%                                                                              & SML                                                 & 99.45                                                    & \begin{tabular}[c]{@{}l@{}}99.71\\ (1.32\%)\end{tabular}                                           & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & PRL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
%                                                     & SubM                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
%                                                                             & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.05\\ (44.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \cline{2-4} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.04\\ (55.55\%)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}
% \begin{table}
% \scriptsize
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.06                                                     & 0.01                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.20                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.20                                                     & 0.04                                                     & 0.25                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.17                                                     & 0.02                                                     & 0.16                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.12                                                     & 0.02                                                     & 0.18                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.18                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.11                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.10\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \scriptsize
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:7}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (70.0\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{table}
% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.23                                                     & 0.03                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.16                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.15                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.11                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.10                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.10\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.34                                                     & 0.03                                                     & 0.17                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.18                                                     & 0.02                                                     & 0.12                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}


% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.04                                                     & 0.01                                                     & 0.07                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.21                                                     & 0.02                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.18                                                     & 0.03                                                     & 0.14                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.12                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & MCL                                                 & 0.12                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SBML                                                 & 0.08                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & CTL                                                 & 0.08 & 0.01 & 0.09                                                    \\ \cline{2-5} 
%                                                                              & CBML                                                 & \0.08 & 0.01 & 0.08 \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
                                                                       
%                                                                              & MCL                                                 & 0.30                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SBML                                                 & 0.32                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & CTL                                                 & 0.10 & 0.03                                                     & 0.09 \\ \cline{2-5} 
%                                                                              & CBML                                                 & 0.11 & 0.01 & 0.08  \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}


% \begin{table}[]
% \centering
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & PRL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
%                                                     & SubM                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
%                                                                             & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.05\\ (44.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \cline{2-4} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.04\\ (55.55\%)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \hline
% \end{tabular}
% \end{table}
% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip5_US_SLN_SIFT_1.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip15_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip30_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE for relative angle}}
%     \label{fig:bucketmae}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_15p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:7 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turns_30p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_road_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:3 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
%     %\footnotesize
%     \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance}}
%     \begin{tabular}{|c|p{0.2mm}|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.32                                                                         & 94.7                                                                          & 95.54                                                                         & 94.82                                                                         & 0.22                                                                          & 0.12                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 91.94                                                                         & 91.08                                                                         & 94.58                                                                         & 95.02                                                                         & \textbf{3.08}                                                                          & \textbf{3.94}                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 91.26                                                                         & 90.36                                                                         & 93.58                                                                         & 92.60                                                                         & 2.32                                                                          & 2.24                                                                          \\ \hline
% \multirow{3}{*}{SLO}                                          & 100:20                                                                                            & 88.34                                                                         & 86.96                                                                         & 89.94                                                                         & 87.79                                                                         & 1.6                                                                           & 0.83                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 89.7                                                                          & 89.8                                                                          & 91.76                                                                         & 91.4                                                                          & 2.06                                                                          & 1.6                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 87.68                                                                         & 88.54                                                                         & 91.36                                                                         & 90.78                                                                         & \textbf{3.68}                                                                          & \textbf{2.24}                                                                          \\ \hline
% \multirow{3}{*}{SLN}                                          & 100:20                                                                                            & 89.18                                                                         & 88.25                                                                         & 90.52                                                                         & 89.26                                                                         & 1.34                                                                           & \textbf{1.01}                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 88.04                                                                          & 88.5                                                                          & 91.32                                                                         & 89.17                                                                          & \textbf{5.28}                                                                          & 0.67                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 86.4                                                                         & 86.22                                                                         & 88.0                                                                         & 86.71                                                                         & 1.6                                                                          & 0.49                                                                          \\ \hline
                                    
% \end{tabular}
% \label{tab:redl}
% \end{minipage}
% \hspace{4cm}
% \begin{minipage}[b]{0.4\linewidth}
%     %\footnotesize
%     \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
%     \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & 16.67                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & \textbf{22.22}                                 \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.08                     & 0.06                           & \textbf{25.0}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.10                     & 0.09                           & 10.0                                 \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & \textbf{16.67}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.05                     & 0.05                           & 0.0                                 \\ \hline
% \end{tabular}
% %\caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
% \label{tab:veh}
% \end{minipage}
% \end{table*}


% \begin{table*}[]
% \footnotesize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance}}
% \centering
% \begin{tabular}{|c|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.32                                                                         & 94.7                                                                          & 95.54                                                                         & 94.82                                                                         & 0.22                                                                          & 0.12                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 91.94                                                                         & 91.08                                                                         & 94.58                                                                         & 95.02                                                                         & \textbf{3.08}                                                                          & \textbf{3.94}                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 91.26                                                                         & 90.36                                                                         & 93.58                                                                         & 92.60                                                                         & 2.32                                                                          & 2.24                                                                          \\ \hline
% \multirow{3}{*}{SLO}                                          & 100:20                                                                                            & 88.34                                                                         & 86.96                                                                         & 89.94                                                                         & 87.79                                                                         & 1.6                                                                           & 0.83                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 89.7                                                                          & 89.8                                                                          & 91.76                                                                         & 91.4                                                                          & 2.06                                                                          & 1.6                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 87.68                                                                         & 88.54                                                                         & 91.36                                                                         & 90.78                                                                         & \textbf{3.68}                                                                          & \textbf{2.24}                                                                          \\ \hline
% \multirow{3}{*}{SLN}                                          & 100:20                                                                                            & 89.18                                                                         & 88.25                                                                         & 90.52                                                                         & 89.26                                                                         & 1.34                                                                           & \textbf{1.01}                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 88.04                                                                          & 88.5                                                                          & 91.32                                                                         & 89.17                                                                          & \textbf{5.28}                                                                          & 0.67                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 86.4                                                                         & 86.22                                                                         & 88.0                                                                         & 86.71                                                                         & 1.6                                                                          & 0.49                                                                          \\ \hline
                                    
% \end{tabular}
% \label{tab:redl}
% \end{table*}


% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Relative Angle affordance}}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{3}{c|}{CAL}                                                                                                                                                         & \multicolumn{3}{c|}{Timestamp}                                                                                                                                                   & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{3-11} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.39                                                    & 0.03                                                        & 0.09                                                     & 0.28                                                    & 0.03                                                        & 0.07                                                     & 28.21                                                    & 0.0                                                         & 22.22                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.38                                                    & 0.04                                                        & 0.11                                                     & 0.27                                                    & 0.04                                                        & 0.09                                                     & \textbf{28.94}                                                    & 0.0                                                         & 18.18                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.44                                                    & 0.06                                                        & 0.15                                                     & 0.32                                                    & 0.05                                                        & 0.09                                                     & 27.27                                                    & \textbf{16.66}                                                         & \textbf{40.0}                                                      \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                                                            & 0.19                                                    & 0.07                                                        & 0.08                                                     & 0.17                                                    & 0.04                                                        & 0.08                                                     & 10.52                                                     & \textbf{3.0}                                                         & 15.38                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.19                                                    & 0.05                                                        & 0.13                                                     & 0.20                                                    & 0.05                                                        & 0.11                                                     & -5.0                                                    & 0.0                                                         & 15.38                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.16                                                     & 0.23                                                    & 0.05                                                        & 0.11                                                     & \textbf{11.53}                                                     & 0.0                                                        & \textbf{31.25}                                                      \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                                                            & 0.18                                                    & 0.05                                                        & 0.07                                                     & 0.16                                                    & 0.05                                                        & 0.07                                                     & 11.11                                                     & 0.0                                                         & 0.0                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.21                                                    & 0.07                                                        & 0.06                                                     & 0.20                                                    & 0.07                                                        & 0.05                                                     & 4.76                                                    & 0.0                                                         & 16.66                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.16                                                     &    0.22                                                 & 0.05                                                        & 0.05                                                     & \textbf{15.38}                                                     & 0.0                                                        & \textbf{68.75}                                                      \\ \hline
% \end{tabular}
% \label{tab:relative}
% \end{table*}

% \begin{table}[]
% \footnotesize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & 16.67                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & \textbf{22.22}                                 \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.08                     & 0.06                           & \textbf{25.0}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.10                     & 0.09                           & 10.0                                 \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & \textbf{16.67}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.05                     & 0.05                           & 0.0                                 \\ \hline
% \end{tabular}
% \label{tab:veh}
% \end{table}

% \begin{table}[]
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \begin{tabular}{|p{7mm}|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods                                                & MAE  & \%Improvement & MAE            & \% Improvement          \\ \hline
% \multicolumn{4}{|c|}{Vehicle Distance}                                                                                                      & \multicolumn{2}{c|}{Centerline Distance} \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &               & 0.09           &                         \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.05 &               & 0.09           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.06 & 16.67         & 0.09           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.05 & 0.0           & 0.08           & 11.11                   \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.04 & 20.0          & 0.07           & 22.22                   \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &               & 0.11           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.07 & -14.28        & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.08 & -25.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.06 & 0.0           & 0.11           & 0.0                     \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               & 0.11           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.10 & -10.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.10 & -10.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.05 & 44.44         & 0.12           & -8.3                    \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% %\captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods                                                & MAE  & \%Improvement \\ \hline
% \multicolumn{4}{|c|}{Vehicle Distance}                                                                                                      \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &               \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.05 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.06 & 16.67         \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.05 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.04 & 20.0          \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.07 & -14.28        \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.08 & -25.0         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.06 & 0.0           \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.10 & -10.0         \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.10 & -10.0         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.05 & 44.44         \\ \hline
% \multicolumn{4}{|c|}{Centerline Distance}                                                                                                   \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.09 &               \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.09 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.08 & 11.11         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.07 & 22.22         \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.11 & 0.0           \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.12 & -8.3          \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% %\captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \centering
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  & \% Improvement \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &                \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                                   & 0.05 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.06 & 16.67               \\ \cline{2-4} 
%                                                             & SLO  & 0.05 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.04 & \textbf{20.0}               \\ \hline
% \multirow{4}{*}{100:7}                                      &\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.07 & -14.28               \\ \cline{2-4} 
%                                                             & SLO  & 0.08 & -25.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.06 & 0.0               \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.10 & -10.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.10 & -10.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.05     & \textbf{44.44}               \\ \hline
% \end{tabular}
% \label{tab:vehaff}
% \end{table}

% \begin{table}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Centerline Distance} \tr{combine this with vehicle distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \centering
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  & \% Improvement \\ \hline
%                                                             & Whole Set    & 0.09 &                \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.09 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.08 & 11.11               \\ \cline{2-4} 
%                                                             & SLN  & 0.07 & \textbf{22.22}               \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.11 & 0.0               \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.12     & -8.3               \\ \hline
% \end{tabular}
% \label{tab:centaff}
% \end{table}

In this section, we will study the performance of different subset selection methods on the basis of their performance in affordance predictions.

We show in tables \ref{tab:redrhazaff}, \ref{tab:vehcen} the performance of Conditional Affordance Learning (CAL) \citep{sauer2018conditional} driving model for four affordances, on subsets obtained by different subset selection techniques for 100:20 compression ratio. 
% We report the best improvement of our proposed methods (STL,SML) for each affordance over the baselines (Uniform Skip (US), Only SIFT, Only Loss, PRL, SubM).
We notice in Table \ref{tab:redrhazaff} that all the methods are able to classify the affordances reasonably well. This is due to weighted cross-entropy losses used for the large number of imbalanced classes as seen initially in Figure \ref{fig:distrib}. From Table \ref{tab:vehcen}, we can see that CTL and CBML outpeform all other methods in predicting vehicle distance affordance. In case of centerline distance, all the methods work similarly with OS and OL performing the worst.

% We notice in table \ref{tab:redlaff} that the \textit{Red Light} accuracies are more for Uniform Skip than all other subset selection methods. Figure \ref{fig:distribhist} (\textit{left)} is a clear indication of the above statement, where we see that the distribution of Uniform Skip for Red Light is higher than all the other gradation methods. It is evident that Uniform Skip method, due to its inherent nature of selection, selects more number of \textit{Red Light True} instances. For example, if the agent vehicle is stuck in traffic, the Uniform Skip method will tend to choose frames uniformly leading to higher selection of true red light instances. However, in case of SLN, since the SIFT dissimilarity and multi-task loss values dominate the selection procedure, it selects the appropriate instances based on them. Since it tries to keep the compression ratio intact while trying to avoid repetitive instances, it tends to drop more frames with \textit{Red Light true} instances leading to a lower accuracy. However, this affordance is not directly related to the episode completion objective.

% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.28                                                                     & 0.02                                                                         & 0.10                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & Only SIFT                                                   & 0.23                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & Only Loss                                                   & 0.16                                                                     & 0.02                                                                         & 0.10                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & PRL                                            & 0.15                                                                     & 0.02                                                                         & 0.10                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLT                                            & 0.11                                                                     & 0.02                                                                         & 0.10                                                                      & 60.71                                                        & 33.33                                                            & 0.0
%                         \\ \cline{2-8} 
%                         & SLM                                            & 0.10                                                                     & 0.02                                                                         & 0.09                                                                      & 64.28                                                        & 33.33                                                            & 10.0
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.46                                                                     & 0.03                                                                         & 0.20                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.51                                                                     & 0.03                                                                         & 0.18                                                                      &                                                         &                                                             &                                                         \\ \cline{2-8} 
% %                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff}
% \end{table*}


% \begin{table}[]
% \centering
% \scriptsize

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.23                                                     & 0.03                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.16                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.15                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.11                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.10                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.10\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \centering
% \scriptsize
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.34                                                     & 0.03                                                     & 0.17                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.18                                                     & 0.02                                                     & 0.12                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{table}



% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     \centering
%     \includegraphics[height=3cm]{figures/preds_allmeth_100_20.png}
%     \caption{\textbf{Bucket-wise MAE of relative angle for 100:20 compression ratio}}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
% \end{figure}

% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Only SIFT\end{tabular} & 0.34                                                                     & 0.03                                                                         & 0.17                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & Only Loss                                                   & 0.18                                                                     & 0.02                                                                         & 0.12                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & PRL                                                   & 0.38                                                                     & 0.03                                                                         & 0.18                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & SLT                                            & 0.12                                                                     & 0.03                                                                         & 0.10                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLM                                            & 0.12                                                                     & 0.02                                                                         &    0.09                                                                   &                                                         &                                                             &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.46                                                                     & 0.03                                                                         & 0.20                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.51                                                                     & 0.03                                                                         & 0.18                                                                      &                                                         &                                                             &                                                         \\ \cline{2-8} 
% %                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff_100_7}
% \end{table*}
 
In case of \textit{Relative Angle} affordance, we have grouped the values into three different buckets meant for Left Turn, Straight Road, Right Turn. We observe in Figures \ref{fig:fracmae_100_20} and \ref{fig:fracmae_100_7} that our proposed method achieves the lowest MAE for turns in comparison to other subset selection methods for both the compression ratio. This is a result of selection of instances using both the pairwise and weighted multi-task pointwise metric as we discussed in Section \ref{sec:subset}. We can also observe in Figures \ref{fig:fracmae_100_20}a and \ref{fig:fracmae_100_7}a that CBML selects more fraction of instances for both Left and Right turns while relaxes comparatively in the Straight Road buckets. SBML also has close fraction of instances to our method for left turn in Figure \ref{fig:fracmae_100_20}a, however it drops down in the fraction of right turns.

Figures \ref{fig:fracmae_100_20}b and \ref{fig:fracmae_100_7}b  portray the effective nature of our subset selection methods (CTL, CBML) over the other baselines in terms of Mean Absolute Error. We observe that the MAE for straight road buckets for all selection methods are very low in range. This is essentially due to the skewness in Relative Angle affordance which we observed initially in Figure \ref{fig:distrib}. On the other hand, both CTL and CBML outperform all other methods in the turn buckets which have in usual, lesser number of datapoints. The difference in MAE becomes more evident with increase in compression ratio. It is indicative of the fact that our proposed method gives more importance to the frames which are non-redundant (during turns especially) and also having higher losses, thus leading to the lower MAE values in extreme buckets. Thus, we can clearly see that our proposed methods CTL and CBML are performing better quantitatively in terms of affordance predictions and qualitatively in terms of deployment of the trained model in simulator and measuring the episode completion rate.


% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{AISTATS2021PaperPack/figures/mae_bucket_100_20.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{AISTATS2021PaperPack/figures/mae_bucket_100_7.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE of relative angle for 100:20 and 100:7 compression ratio}}
%     \label{fig:maebuck}
% \end{figure}


% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/leftbucket_allmeth.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/straightbucket_allmeth.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/rightbucket_allmeth.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}








% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlysift_sim_fail.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlyloss_sim_fail.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prl_sim_fail.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Buckets in simulator episodes leading to failures for \textit{Only SIFT}(left), \textit{Only Loss}(middle) and \textit{PRL}(right) }}
%     \label{fig:deviate}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/sift_sml_stl_13_27.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlyloss_sml_stl_48_41.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prl_sml_stl_87_95.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Buckets in simulator episodes leading to failures for \textit{Only SIFT}(left), \textit{Only Loss}(middle) and \textit{PRL}(right) }}
%     \label{fig:deviate}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip5_US_SLN_SIFT_1.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip15_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip30_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE for relative angle}}
%     \label{fig:bucketmae}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_15p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:7 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turns_30p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_road_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:3 compression ratio}}
%     \label{fig:bucketprop30}
% \end{figure*}
% The same can be observed in table \ref{tab:relaff} where the Straight-Road MAE for all gradation methods have a narrow margin. This happens due to the more number of straight road instances than the turns in our dataset, as depicted in Figure \ref{fig:distrib} (\textit{Right}). However, SLN maintains an overall lower MAE across the buckets, thus proving its selection method efficient.
 
% We also show a similar plot for distribution of predicted affordances in Figure \ref{fig:distribhistpred} where we observe that the predictions also follow similar pattern as the distribution of ground truth affordances in Figure \ref{fig:distribhist}.


% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 96.26                                                    & 95.43                                                    \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 95.54                                                    & 94.82                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 91.9                                                     & 90.75                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 89.94                                                    & 87.79                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 90.52                                                    & 89.26                                                    \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 94.58                                                    & 95.02                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 90.1                                                     & 88.58                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 91.76                                                    & 91.4                                                     \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 91.32                                                    & 89.17                                                    \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 93.58                                                    & 92.60                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 91.87                                                    & 89.02                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 91.36                                                    & 90.78                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &                                                          &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Red Light affordance}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 0.15                                                    & 0.02                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.28                                                    & 0.03                                                        & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.16                                                    & 0.05                                                        & 0.14                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.17                                                    & 0.04                                                        & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.16                                                    & 0.05                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.27                                                    & 0.04                                                        & 0.09                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.17                                                    & 0.05                                                        & 0.16                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.21                                                    & 0.05                                                        & 0.11                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.19                                                    & 0.08                                                        & 0.06                                                     \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.32                                                    & 0.05                                                        & 0.09                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.28                                                    & 0.05                                                        & 0.14                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.23                                                    & 0.06                                                        & 0.11                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &                                                         &                                                             &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}
% \label{tab:relaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  \\ \hline
% \-\-                                                        & Whole Set    & 0.02 \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.04 \\ \cline{2-3} 
%                                                             & SIFT         & 0.04 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.04 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.05 \\ \cline{2-3} 
%                                                             & SIFT         & 0.07 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.06 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.07 \\ \cline{2-3} 
%                                                             & SIFT         & 0.09 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.09 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  &      \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Vehicle Distance affordance}
% \label{tab:vehaff}
% \end{table}




% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 95.86                                                    & 95.16                                                    \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 95.32 (-6.32)                                                   & 94.7 (-6.45)                                                   \\ \cline{2-4} 
%                                                             & SIFT         & 91.36 (-2.18)                                                    & 88.12 (0.13)                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 88.34 (0.84)                                                   & 86.96 (1.29)                                                   \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 89.18                                                   & 88.25                                                    \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 91.94 (-3.93)                                                   & 91.08 (-2.58)                                                   \\ \cline{2-4} 
%                                                             & SIFT         & 90.28 (-2.24)                                                    & 90.1 (-1.6)                                                   \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 89.7 (-1.66)                                                   & 89.8 (-1.3)                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &    88.04                                                 & 88.5                                                    \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 91.26                                                    & 90.36                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 90.04                                                    & 90.34                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 87.68                                                    & 88.54                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &                                                          &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Red Light affordance}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 0.15                                                    & 0.02                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.39 (0.21)                                                   & 0.03 (-0.02)                                                       & 0.09 (0.02)                                                    \\ \cline{2-5} 
%                                                             & SIFT         & 0.17 (-0.01)                                                   & 0.06 (-0.01)                                                       & 0.09 (0.01)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.19 (0.01)                                                   & 0.07                                                       & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.18                                                    & 0.05                                                        & 0.07                                                     \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.38 (0.18)                                                   & 0.04 (-0.03)                                                       & 0.11 (0.05)                                                    \\ \cline{2-5} 
%                                                             & SIFT         & 0.18 (-0.02)                                                   & 0.06 (-0.01)                                                       & 0.14 (0.08)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.19 (0.01)                                                   & 0.05 (-0.02)                                                       & 0.13 (0.07)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &    0.20                                                 & 0.07                                                        & 0.06                                                     \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.44                                                    & 0.06                                                        & 0.15                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.32                                                    & 0.06                                                        & 0.15                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.26                                                    & 0.05                                                        & 0.16                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &                                                         &                                                             &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}
% \label{tab:relaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  \\ \hline
% \-\-                                                        & Whole Set    & 0.02 \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.05 (0.01) \\ \cline{2-3} 
%                                                             & SIFT         & 0.06 (0.02) \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.05 (0.01) \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.06 (0.0) \\ \cline{2-3} 
%                                                             & SIFT         & 0.07 (0.01)\\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.08 (0.02) \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.06 \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.09 \\ \cline{2-3} 
%                                                             & SIFT         & 0.10 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.10 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  &      \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Vehicle Distance affordance}
% \label{tab:vehaff}
% \end{table}


% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 95.54                                                                         & 94.82                                                                         & 0.28                                                                         & 0.03                                                                             & 0.07                                                                          & 0.04                                  \\ \hline
% SIFT                                                   & 91.9                                                                          & 90.75                                                                         & 0.16                                                                         & 0.05                                                                             & 0.14                                                                          & 0.04                                      \\ \hline
% SIFT+Loss-O                                            & 89.94                                                                         & 87.79                                                                         & 0.17                                                                         & 0.04                                                                             & 0.08                                                                          & 0.04                                      \\ \hline
% SIFT+Loss-N                                            & 90.52                                                                         & 89.26                                                                         & 0.16                                                                         & 0.05                                                                             & 0.08                                                                          & 0.04                                      \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:20}
% \label{tab:grade_20}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.58                                                                         & 95.02                                                                         & 0.27                                                                         & 0.04                                                                             & 0.09                                                                          & 0.05                                  \\ \hline
% SIFT                                                   & 90.1                                                                          & 88.58                                                                         & 0.17                                                                         & 0.05                                                                             & 0.16                                                                          & 0.07                                      \\ \hline
% SIFT+Loss-O                                            & 91.76                                                                         & 91.4                                                                         & 0.21                                                                         & 0.05                                                                             & 0.11                                                                          & 0.06                                      \\ \hline
% SIFT+Loss-N                                            & 91.32                                                                         & 89.17                                                                         & 0.19                                                                         & 0.08                                                                             & 0.06                                                                          & 0.04                                      \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:7}
% \label{tab_grade_7}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 93.58                                                                         & 92.60                                                                         & 0.32                                                                         & 0.05                                                                             & 0.09                                                                          & 0.07                                   \\ \hline
% SIFT                                                   & 91.87                                                                          & 89.02                                                                         & 0.28                                                                         & 0.05                                                                             & 0.14                                                                          & 0.09                                      \\ \hline
% SIFT+Loss-O                                            & 91.36                                                                         & 90.78                                                                         & 0.23                                                                         & 0.07                                                                             & 0.11                                                                          & 0.09                                       \\ \hline
% SIFT+Loss-N                                            &                                                                          &                                                                          &                                                                          &                                                                              &                                                                           &                                       \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:3}
% \label{tab:grade_3}
% \end{table*}

% Considering the first type of observation for each compression ratio (or table), we notice that the Timestamp model shows an improved performance for each affordance in comparison. This is because the CAL model takes continuous frames into consideration, while in the Timestamp model, we have integrated the normalised timestamp difference between the subsequent frames. This leads to the better performance in Timestamp model, for all the data gradation methods where both uniformly and non-uniformly skipped frames are present.

% Following the second type of observation for each data gradation method under the same model (CAL or Timestamp), we notice that the \textit{Red Light} accuracies are more for Uniform Skip than all other subset selection methods. The reason becomes evident from Figure \ref{fig:distribhist} (\textit{top left)} where we see that the Uniform Skip method, due to its inherent nature of selection, selects more number of \textit{Red Light True} instances compared to the other methods. In case of \textit{Relative Angle} affordance, we have grouped the corresponding values into three different bins meant for Left Turn, Straight Road, Right Turn. We can observe from Figure \ref{fig:distribhist} (\textit{top right}) that SIFT+Loss-N (SLN) selects more number of instances belonging to the turn category. This is a result of selection of instances using the pointwise metric as we discussed in Section \ref{improved}. Even SIFT and SIFT+Loss-O perform close to SIFT+Loss-N in the selection method due to their selection mechanisms. The similar distribution in the values of Uniform Skip and Whole Set is trivial.

% We observe that even though the Uniform Skip method has similar distribution to that of WS, it is not what should ideally be for a decreased set of instances. This is because the reduced subset unless has enough instances of turns, the driving model would not be able to predict its next waypoint. SIFT and Sift+Loss-O have more instances of left turn instances than Uniform Skip. However, SIFT+Loss-N has a significantly higher number of instances for both the turns. Taking this into consideration, we observe from each table, that under each model (CAL or Timestamp), the gradation methods SIFT, SIFT+Loss-O and SIFT+Loss-N perform significantly better under turns than the Uniform Skip model.

% We show a bucketwise plot of relative angle for different compression ratios in Figure \ref{fig:bucketmae}, which portrays the effective nature of the gradation methods over Uniform Skip. The buckets corresponding to (-0.1 - 0.1) refer to the straight road instances, and the buckets to its left are meant for left turns while to its right, for right turns. We observe that the MAE for straight road buckets for all gradation methods are very low and close to one another. This happens due to the more number of straight road instances than the turns, as depicted in Figure \ref{fig:distrib} (\textit{Right}). Owing to the selection of large number of straight road instances in Uniform Skip selection, the MAE for straight road is lesser compared to the other selection methods. However, predicting its next waypoint on straight road is an easier task compared to turns, which we will observe in the next subsection.

% Lastly, with increasing degree of compression ratio, the performance of the gradation methods shifts away from that of the Whole Set, which is trivial. However, we observe that the difference between the performance of CAL and Timestamp model for each gradation method, becomes more vivid with increasing compression ratio. 



% We observe that the accuracies of the discrete affordance (Red Light) of the models trained using subsets are different by a comparatively wider margin, whereas that of the continuous affordances (Relative Angle and Centerline Distance) differ by a narrow margin. Uniform skip even though performs the best among all subsets in terms of red light affordance accuracy, it fails in selecting images necessary to be present during the turns.
% We show in Figure \ref{fig:distribhist} the distribution of two of the affordances (\textit{Red Light} and \textit{Relative Angle}) in all the selection methods for the compression ratio 100:20. We observe that distribution of both the affordances for Uniform Skip (US) is similar to that of the Whole Set (WS), which is trivial. However, the distribution differs for the other selection methods. In case of red light, SLN (Sift+Loss-N) selects comparatively more number of \textit{Red Light True} instances than the other two methods, namely SIFT and SLO (Sift + Loss-O), but lesser than that of US (Uniform Skip). This leads to the decrease in Red Light accuracy for the selection methods. The reason behind the decrease in selection of \textit{Red Light True} instances is that since the frames captured while in traffic are redundant, the selection methods try to skip the frames. \\
% The figure to the right showing the distribution of affordances for relative angle, we observe that even though the US method has similar distribution to that of WS, it is not what should ideally be for a decreased set of instances. This is because the reduced subset unless has enough instances of turns, the training model would not be able to predict its next waypoint. SIFT and SLO have more instances of left turn instances than US. However, SLN has a significantly higher number of instances for both the turns. The average MAE for SLN is slightly higher than that of US or SIFT. This is because the more number of test instances are concentrated towards the \textit{Straight} task, which has lesser number of selected frames due to redundancy. We show a bucketwise plot of relative angle which portrays the effective nature of SLN.
%\textcolor{red}{More explanation}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth,height=3.5cm]{figures/redlight.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:distribhist}
% \end{figure}



% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_pred5.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_pred5.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_pred15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_pred15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%      \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_30.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relative_30.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of predicted affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7 , (\textit{bottom}) 100:3 compression ratio: WS : Whole Set; US : Uniform Skip; SLO : SIFT+Loss-O; SLN : SIFT+Loss-N}}
%     \label{fig:distribhistpred}
% \end{figure}
% \begin{figure}[h!]
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redl.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:relhist}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turns.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:turnhist}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/haz.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:relhist}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/speed.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:turnhist}
%     \end{subfigure}
%     \captionsetup{justification=centering}
%     \caption{Comparison of distribution of affordances among the selection methods for 100:20 compression ratio: WS : Whole Set; US : Uniform Skip; SLO : SIFT+Loss-O; SLN : SIFT+Loss-N}
%     \label{fig:distribhist}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth,height=4cm]{figures/test_turns_skip5.png}
%     \caption{Bucket-wise MAE for relative angle}
%     \label{fig:turnskip5}
% \end{figure}









% \begin{table*}[]
% %\centering
% \begin{tabular}{|l|p{7mm}|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{3}{*}{Ratio}  & \multirow{3}{*}{Poses} & \multicolumn{8}{c|}{Tasks}                                                                                                                                                                                                                                                    \\ \cline{4-11} 
%                                                                           &                         &                        & \multicolumn{2}{l|}{Straight} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}One\\ Turn\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}One\\ Turn\\Dynamic\end{tabular}} \\ \cline{4-11} 
%                                                                           &                         &                        & CAL            & TS           & CAL                                 & TS                                & CAL                                     & TS                                    & CAL                                      & TS                                     \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}}      & \multirow{2}{*}{}       & Train                  & 10             &              & 9                                   &                                   & 10                                      &                                       & 8                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 7                                   &                                   & 10                                      &                                       & 7                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:20} & Train                  & 9              &              & 0                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 1                                   &                                   & 9                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  & 10             &              & 2                                   &                                   & 10                                      &                                       & 2                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 1                                   &                                   & 9                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  & 10             &              & 3                                    &                                   & 8                                       &                                       & 2                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 2                                    &                                   & 9                                       &                                       & 1                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  & 10             &              & 6                                   &                                   & 10                                      &                                       & 6                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 3                                   &                                   & 10                                      &                                       & 3                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:7} & Train                  & 9              &              & 0                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 0                                   &                                   & 7                                       &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  & 9             &              & 2                                   &                                   & 9                                      &                                       & 1                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 8             &              & 1                                   &                                   & 8                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  &              &              & 2                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  & 10             &              & 3                                   &                                   & 10                                      &                                       & 3                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 2                                   &                                   & 10                                      &                                       & 2                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:3} & Train                  & 9              &              & 1                                   &                                   & 8                                       &                                       & 0                                       &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 1                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  &              &              & 1                                   &                                   &                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                   &                                   &                                        &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  &              &              & 1                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                    &                                   &                                        &                                       & 0                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  &              &              &                                    &                                   &                                       &                                       &                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              &                                    &                                   &                                       &                                       &                                         &                                        \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques in terms of episode completion \tr{Will reorder the structure}}
% \label{eptable}
% \end{table*}




% \subsection{CAL vs Timestamp model}
% \label{tsvscal}

% Having motivated the Timestamp model in Section \ref{sec:CAL-TS}, we show here the effectiveness of Timestamp model in the light of prediction of the following affordances - \textit{Red Light} ,\textit{Vehicle Distance} and \textit{Relative Angle}. We compare in tables \ref{tab:redl},  \ref{tab:veh} and \ref{tab:relative}, CAL and Timestamp Model for the three methods - Uniform Skip, SLO and SLN across 3 compression ratios - \textit{100:20}, \textit{100:7} and \textit{100:3}. We report the micro and macro accuracies for Red Light, direction based bucket-MAE of relative angle , MAE of vehicle distance and \% improvement of Timestamp model over CAL model for every affordance.

% It is observed that Timestamp model shows an improved performance in affordance predictions for all the methods for each affordance in comparison. This is because the CAL model takes continuous frames into consideration in the frame buffer, while the Timestamp model integrates the normalised timestamp difference between the subsequent frames. This leads to the better performance in Timestamp model for the data gradation methods, where both uniformly and non-uniformly skipped frames are present. We have boldfaced the highest improvement for each gradation method under each metric of affordance.

% Besides, we observe in table \ref{tab:relative} that Uniform skip which is an uniformly-skipping-frames method, has a higher MAE for Left turn under CAL model. The reason lies in the number of left turns present in our dataset, shown in Figure \ref{fig:distrib} (\textit{Right}). Owing to its inherent nature, Uniform skip tends to skip frames uniformly, as a result of which it ends up missing a large number of frames belonging to left turn. However, using Timestamp model, the respective Left Turn MAE for Uniform skip is lower due to the inclusion of timestamp information. Hence, we are able to show that inclusion of timestamp information in the perception module of driving model yields a better performance, in the process of making self-driving data efficient.


% \begin{table}[]
% \caption{\textbf{Comparison of CAL and Timestamp Model on Centerline Distance affordance}}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.09                     & 0.07                           & \textbf{22.22}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.10                           & 9.09                                \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.09                     & 0.08                           & \textbf{11.11}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-N}                                            & 100:20                                                                                            & 0.07                     & 0.06                           & \textbf{14.28}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.11                            & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.12                     & 0.12                           & 0.0                                 \\ \hline
% \end{tabular}
% \label{tab:cenaff}
% \end{table}

% \begin{table*}[]
% \centering
% \begin{tabular}{|c|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.63                                                                         & 94.98                                                                          & 96.22                                                                         & 95.41                                                                         & 0.59                                                                           & 0.43                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 93.53                                                                         & 93.53                                                                         & 95.58                                                                         & 95.15                                                                         &  2.05                                                                         & 1.62                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 92.64                                                                         & 92.15                                                                         & 95.29                                                                         & 94.92                                                                         & 2.65                                                                          & 2.77                                                                          \\ \hline
% \multirow{3}{*}{SIFT + Loss-O}                                          & 100:20                                                                                            & 96.83                                                                         & 86.43                                                                         & 97.99                                                                         & 93.25                                                                         & 1.16                                                                           & 6.82                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 96.74                                                                          & 90.17                                                                          & 97.01                                                                         & 92.32                                                                          & 0.27                                                                          & 2.15                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 90.53                                                                         & 89.97                                                                         & 97.63                                                                         & 91.69                                                                         & 7.1                                                                          & 1.72                                                                         \\ \hline

% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance using varying spaced frame buffers}}
% \label{tab:redl_data}
% \end{table*}


% \begin{table*}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{3}{c|}{CAL}                                                                                                                                                         & \multicolumn{3}{c|}{Timestamp}                                                                                                                                                   & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{3-11} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.29                                                    & 0.02                                                        & 0.09                                                     & 0.20                                                    & 0.02                                                        & 0.06                                                     & 31.0                                                    & 0.0                                                         & 33.33                                                     \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.36                                                    & 0.03                                                        & 0.15                                                     & 0.37                                                    & 0.03                                                        & 0.11                                                     & -2.7                                                    & 0.0                                                         & 26.67                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.44                                                    & 0.03                                                        & 0.13                                                     & 0.38                                                    & 0.03                                                        & 0.10                                                    & 13.63                                                    & 0.0                                                         & 23.08                                                      \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.20                                                    & 0.07                                                        & 0.11                                                     & 0.12                                                    & 0.04                                                        & 0.13                                                     & 40.0                                                     & 42.85                                                         & -18.18                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.24                                                    & 0.05                                                        & 0.21                                                     & 0.20                                                    & 0.04                                                        & 0.15                                                     & 16.67                                                    &    20.0                                                      & 28.57                                                     \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.17                                                     & 0.27                                                    & 0.04                                                        & 0.15                                                     & -3.8                                                     & 20.0                                                        & 11.76                                                      \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Relative Angle affordance using varying spaced frame buffers}}
% \label{tab:relative_data}
% \end{table*}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   &  0.07                    & 0.05                           & 28.57                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                  & 0.03                     & 0.02                           & 33.33                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.07                     & 0.04                           & 42.85                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & 22.22                                 \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance using varying spaced frame buffers}}
% \label{tab:veh_data}
% \end{table}

% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.08                     & 0.08                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.07                     & 0.07                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.12                         & 0.11                               & 8.33                                    \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.15                     & 0.09                           & 40.0                                \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.15                     & 0.13                           & 13.33                               \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.17                     & 0.16                           & 5.88                                \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Centerline Distance affordance using varying spaced frame buffers}}
% \label{tab:cen_data}
% \end{table}



% \begin{table*}[h!]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 95.32                                               & 94.7                                                & 95.54                                               & 94.82                                               & 0.22                                                    & 0.12                                                    & 0.39                                                      & 0.03                                                          & 0.09                                                       & 0.28                                                      & 0.03                                                          & 0.07                                                       & 11.0                                                    & 0.0         & 2.0                                                      & 0.05 & 0.04                     & 1.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 88.34                                               & 86.96                                               & 89.94                                               & 87.79                                               & 1.6                                                    & 0.83                                                    & 0.19                                                      & 0.07                                                          & 0.08                                                       & 0.17                                                      & 0.04                                                          & 0.08                                                       & 2.0                                                    & 3.0         & 0.0                                                      & 0.05 & 0.04                     & 1.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp (TS) Model for compression ratio 100:20}
% \label{CALvsTS_100_20}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 91.94                                               & 91.08                                                & 94.58                                               & 95.02                                               & 3.08                                                    & 3.94                                                    & 0.38                                                      & 0.04                                                          & 0.11                                                       & 0.27                                                      & 0.04                                                          & 0.09                                                       & 11.0                                                    & 0.0         & 2.0                                                      & 0.06 & 0.05                     & 1.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 89.7                                               & 89.8                                               & 91.76                                               & 91.4                                               & 2.06                                                    & 1.6                                                    & 0.19                                                      & 0.05                                                          & 0.13                                                       & 0.21                                                      & 0.05                                                          & 0.11                                                       & -2.0                                                    & 0.0         & 2.0                                                      & 0.08 & 0.06                     & 2.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp (TS) Model for compression ratio 100:7}
% \label{CALvsTS_100_7}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 91.26                                               & 90.36                                                & 93.58                                               & 92.60                                               & 2.32                                                    & 2.24                                                    & 0.44                                                      & 0.06                                                          & 0.15                                                       & 0.32                                                      & 0.05                                                          & 0.09                                                       & 12.0                                                    & 1.0         & 6.0                                                      & 0.09 & 0.07                     & 2.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 87.68                                               & 88.54                                               & 91.36                                               & 90.78                                               & 3.68                                                    & 2.24                                                    & 0.26                                                      & 0.05                                                          & 0.16                                                       & 0.23                                                      & 0.07                                                          & 0.11                                                       & 3.0                                                    & -2.0         & 5.0                                                      & 0.10 & 0.09                     & 1.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp(TS) Model for compression ratio 100:3}
% \label{CALvsTS_100_3}
% \end{table*}





==> experiment2.tex <==
% \tr{
% - Comparison of approximate online subset selection methods:\\
% -- synthetic data: our method, PRL 2020, sub-modular. Can we compare against other methods?\\
% -- Video data: our method, PRL 2020, sub-modular.\\
% -- Sequential application \\
% -- comparison of PRL with variation in $\rho$
% - Data efficient autonomous driving:\\
% -- 
% }


In this section, we provide our experimental setup by describing the dataset and the subset selection methods. We then show a comparison of approximate online subset selection methods over synthetic data and our collected driving data from the CARLA simulator \cite{dosovitskiy2017carla}. Next, we compare the performances of various subset selection methods in the autonomous driving application from two aspects: episode completion and affordance prediction.

\subsection{Experimental Setup}

\textbf{Dataset}: We use the open-source driving simulator CARLA\cite{dosovitskiy2017carla} for generating our driving dataset. CARLA simulates an urban driving scenario where there are several other non-player agents like other vehicles, pedestrians, traffic lights and speed signs aiding the player agent vehicle.
In order to collect the training data, the agent vehicle was navigated using the Conditional Affordance Learning controller \cite{sauer2018conditional} based on the ground truth affordances like red light, hazard stop etc. which have been described later in this section. The affordances have been determined and categorised following \cite{sauer2018conditional}. We generated the driving data comprising of 262 episodes and a total of approximately 100,000 frames. We performed the experiments on our generated dataset and compared the subsets obtained using different selection methods.

% where the agent vehicle is driven by the game AI.
For each episode run, we collect: (1) images from camera attached to the agent vehicle, and (2) the corresponding six affordances (Discrete: Red Light, Hazard Stop, Speed Sign ; Continuous: Relative Angle, Centerline Distance, Vehicle Distance) \cite{sauer2018conditional}. Affordances are signals useful for navigation in the environment. We used approximately $85\%$ of the collected dataset as the training set, and the remaining as the test set.
 
 We ensured the similar distribution of affordances in both the training and test set. Figure \ref{fig:distrib} illustrates the distribution of four affordances per class label, in training and test set. Red light and Hazard Stop have two classes - \textit{True}, \textit{False}, Speed sign has four classes - \textit{None} , \textit{30kmph}, \textit{60kmph}, \textit{90kmph}, while in case of Relative angle which is the orientation angle of the agent vehicle, we have grouped the values into buckets corresponding to \textit{Left turn}, \textit{Straight} and \textit{Right turn}. We can divide the entire range of Relative Angle affordance across 20 buckets ranging from -1.0 to +1.0. Note that buckets corresponding to (-1.0 to -0.1), (-0.1 to 0.1) and (0.1 to 1.0) approximately indicate the left turn, straight road and right turn respectively.
 
 \begin{figure}[h!]
    %\centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_red.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:red}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_rel.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:relang}
    \caption{}
    \end{subfigure}
    % \captionsetup{justification=centering}
    % \caption{\textbf{Distribution of affordances: (\textit{Left}) : Red Light and (\textit{Right}) : Relative Angle in training and test set}}
    % \label{fig:distrib}
    
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_speed.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:spd}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_haz.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:haz}
    \caption{}
    \end{subfigure}
    %\captionsetup{justification=centering}
    \caption{\textbf{Distribution of affordances: (a) : Red Light (b) : Relative Angle (c) : Speed Sign (d) : Hazard Stop in training and test set}} 
    \label{fig:distrib}
    % \begin{subfigure}{0.48\columnwidth}
    % \centering
    % \includegraphics[width=\textwidth,height=2.5cm]{figures/speedsign.eps}
    % %\caption{Red light Affordance Distribution}
    % \label{fig:turn}
    % \end{subfigure}
    
    
\end{figure}

%\subsubsection{Subset selection on Autonomous Driving}
\textbf{Subset selection on Autonomous Driving:}
We use Conditional Affordance Learning \cite{sauer2018conditional} (CAL) model as the driving model to be trained on the dataset we collected using the CARLA \cite{dosovitskiy2017carla} simulator. We train the driving model on NVIDIA Tesla P100 for 50 epochs using Adam Optimizer with learning rate varying between $10^{-3}$ to $10^{-4}$.

We report results with the following methods of selection for two compression ratios 100:20 and 100:7:

\textbf{Whole Set (WS)}: This comprises of the dataset with no reduction.

\textbf{Uniform Skip (US)}: The data is sampled uniformly from the whole dataset, based on the compression ratio.

\textbf{Only SIFT (OS)}: Following Equation \ref{eqn:eq1}, this subset is obtained by selecting images based only on SIFT dissimilarity.

\textbf{Only Loss (OL)}: This subset is obtained by selecting images with highest losses.

\textbf{Multi-Criteria Loss (MCL)}\cite{das2020multi} : The subset is formed by using the multiple-criteria-based subset selection method (Equation \ref{eqn:oldsiftloss}), based on the compression ratio. We used the pairwise criteria (SIFT dissimilarity) and pointwise criteria (loss) as the components of this method.

\textbf{Submodular Bucketwise Multi-task Loss (SBML)}\cite{buchbinder2014submodular} : The subset is obtained by adapting the submodular approach proposed in \cite{buchbinder2014submodular}, in our framework with pairwise (SIFT dissimilarity) and pointwise metric (bucket-wise Relative Angle affordance aided with other multi task losses). 

\textbf{Convex Total Loss (CTL)}: This subset is obtained by adopting our proposed subset selection method (Equation \ref{eqn:newsiftloss}) using SIFT and total loss, based on the compression ratio.

\textbf{Convex Bucketwise Multi-task Loss (CBML)}: This subset is formed by adopting our proposed subset selection method (Equation \ref{eqn:newsiftloss}) using SIFT and bucket-wise Relative Angle affordance aided with other multi task losses, based on the compression ratio.

% \begin{table*}[]
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion}}
% \label{tab:epsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{c|}{Straight}                                                                                                                                               & \multicolumn{3}{c|}{One-Turn}                                                                                                                                             & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set episode completion count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{10}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{10}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SLO/\\ SLN\end{tabular} & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   & \begin{tabular}[c]{@{}l@{}}SIFT/\\ SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   \\ \hline
% 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   \\ \hline
% 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 1                                                       & 88.88                                                   & SLN                                                   & 10                                                      & 0                                                       & SLO                                                   & 1                                                       & 88.88                                                   \\ \hline
% %                                                                              & \multicolumn{12}{c|}{Whole Set test poses completion count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
% %                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{7}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    \\ \hline
% % 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}      & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% % 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 2                                                       & 71.42                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% % 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \scriptsize
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for relative angle affordance prediction}}
% \label{tab:relsumm}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{9}{c|}{Relative Angle buckets}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-10} 
%                                                                              & \multicolumn{3}{c|}{Left-Turn}                                                                                                                                                & \multicolumn{3}{c|}{Straight-Road}                                                                                                                                             & \multicolumn{3}{c|}{Right-Turn}                                                                                                                                               \\ \cline{2-10} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & SIFT                                                  & 0.02                                                        & 11.76                                                   & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.01                                                        & 33.33                                                   & SLN                                                  & 0.01                                                        & 12.5                                                   \\ \hline
% 100:7                                                                        & SIFT                                                  & 0.03                                                        & 16.67                                                   & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.01                                                        & 50.0                                                    & SLN                                                  & 0.01                                                        & 25.0                                                   \\ \hline
% 100:3                                                                        & SLN                                                   & 0.06                                                        & 28.57                                                   & SLO                                                    & 0.02                                                        & 60.0                                                    & SLN                                                   & 0.02                                                        & 25.0                                                    \\ \hline
% \end{tabular}
% \end{table*}
% We use Conditional Affordance Learning model \cite{sauer2018conditional} (CAL) as the driving model to be trained on the dataset we collected using the CARLA \cite{dosovitskiy2017carla} simulator. We train the driving model on NVIDIA Tesla P100 for 50 epochs using Adam Optimizer with learning rate varying between $10^{-3}$ to $10^{-4}$.

 
 \textbf{Subset selection and Training Times}:
%  \tr{write in 2 - 3 sentences how our methods are saving time as well as storage space refering to table \ref{tab:time}}
Table \ref{tab:time} shows the amount of total time taken for training and subset selection for each compression ratio. Compression ratio of 100:20 takes about 1/3rd the total time taken to train the whole set (WS). In terms of storage space, the whole set acquires about 14.5GB of data, which after compression reduces to 2.9GB for compression ratio of 100:20. This follows for the other compression ratio too and hence saves both time and space, essential in the current IoT setting with massively huge data.

 
%  \begin{table}[h]
% \captionsetup{justification=centering}
% \caption{\textbf{Time complexity of proposed methods}}
% \footnotesize
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Compression ratio    & WS  & 100:20 & 100:7 & 100:3 \\ \hline
% Training Time (hours)  & 30 & 8   & 3 & 1.5   \\ \hline
% Subset selection Time (hours) & 0  & 2   & 1.5 & 1   \\ \hline
% Total Time     & 30 & 10   & 4.5 & 2.5   \\ \hline
% \end{tabular}
% \label{tab:time}
% \end{table}

% \begin{table}[h]
% \captionsetup{justification=centering}
% \caption{\textbf{Time complexity of proposed method}}
% \footnotesize
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Compression ratio    & WS  & 100:20 & 100:7\\ \hline
% Training Time (hours)  & 42 & 11   & 7\\ \hline
% Subset selection Time (hours) & 0  & 3   & 1.5\\  \hline
% Total Time     & 42 & 14   & 8.5\\ \hline
% \end{tabular}
% \label{tab:time}
% \end{table}

\begin{table}[]
\caption{\textbf{Time complexity of selection methods}}
\footnotesize
\begin{tabular}{|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}                         & WS                 & \multirow{2}{*}{}                                         & 100:20 & 100:7 \\ \cline{1-2} \cline{4-5} 
\begin{tabular}[c]{@{}l@{}}Training Time\\ (hours)\end{tabular}                     & 42                 &                                                           & 11     & 7     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Subset Selection\\ (hours)\end{tabular}} & \multirow{3}{*}{0} & MCL                                                       & 2      & 1     \\ \cline{3-5} 
                                                                                    &                    & SBML                                                      & 5      & 2.5   \\ \cline{3-5} 
                                                                                    &                    & \begin{tabular}[c]{@{}l@{}}Proposed\\ Method\end{tabular} & 1.5    & 0.75  \\ \hline
\end{tabular}
\label{tab:time}
\end{table}


% \begin{table}[h!]
% \captionsetup{justification=centering}
% \caption{\textbf{Prediction accuracy of speed sign on test set using CAL model trained on whole dataset}}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Affordance & None  & 30kmph & 60kmph & 90kmph\\ \hline
% Speed Sign & 98.99 & 0.0   & 100.0 & 0.0\\ \hline
% \end{tabular}
% \label{speedacc}
% \end{table}

% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions}}
% \label{tab:ep}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 3                                                          & 8        & 2                                                          & 9        & 3                                                          & 9        & 3                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &        &                                                           &         &                                                           &        &                                                           &         &                                                           \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{9}                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{8}                                                          \\ \hline
% \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 2                                                          & 8        & 2                                                          & 9        & 3                                                          & 7        & 3                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 9        & 4                                                          & 9        & 4                                                          & 8        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         &                                                           \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{6}                                                          & 10       & \textbf{6}                                                          & 10       & \textbf{8}                                                          & 10       & \textbf{8}                                                          \\ \hline
% \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 1                                                          & 8        & 0                                                          & 9        & 2                                                          & 8        & 2                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 8        & 0                                                          & 8        & 0                                                          & 8        & 1                                                          & 9        & 0                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         & 0                                                          \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{5}                                                          & 10       & \textbf{5}                                                          & 10       & \textbf{6}                                                          & 9       & \textbf{6}                                                          \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.28                                                                     & 0.02                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.23                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLN                                            & 0.10                                                                     & 0.01                                                                         & 0.04                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.07                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                         \\ \cline{2-8} 
%                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff}
% \end{table*}

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 97.39                                                                     & 97.41                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 96.72                                                                     &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 96.11                                                                     & 96.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 93.49                                                                     & 91.96                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 92.63                                                                     & 91.94                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 89.55                                                                     & 87.23                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                       &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 97.12                                                                     & 97.04                                                                      &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.06                                                                     & 93.09                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 94.16                                                                     & 93.54                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 94.42                                                                      & 93.72                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 99.44                                                                     & 99.72                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.14                                                                     & 99.47                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.11                                                                     & 99.56                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.33                                                                     & 99.66                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.42                                                                     & 97.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.31                                                                     & 98.99                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                       &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.45                                                                     & 98.76                                                                      &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 98.57                                                                     & 97.67                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.29                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.12                                                                      & 98.23                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:hazaff}
% \end{table}
% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|p{12mm}|p{8mm}|l|p{15.5mm}|l|p{15.5mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & MAE           & \%Improvement         & MAE            & \%Improvement           \\ \cline{3-6} 
%                                                                              &                                                        & \multicolumn{2}{l|}{Vehicle Distance} & \multicolumn{2}{l|}{Centerline Distance} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.03          &                       & 0.05           &                         \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.05           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                    &            &                    \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.04          &                   & 0.06           &                    \\ \hline
% \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.06           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.09          &                 & 0.08           &                      \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                  &            &                      \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.07          &                   & 0.06           &                     \\ \hline
% \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.07          &                       & 0.09           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.11          &                  & 0.08           &                     \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                  &            &                      \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.06          &                  & 0.06           &                     \\ \hline
% \end{tabular}
% \end{table}

\textbf{Metrics reported}: We have reported metrics for the two subtasks: episode completion and affordance accuracies. An episode corresponds to a source-destination pair which is provided to the agent vehicle prior to running the simulator. The episode completion is measured in terms of the number of successfully completed episodes. The accuracies of discrete affordances are measured in terms of the standard metrics - Micro and Macro Accuracy, while the continuous affordances are measured in terms of Mean Absolute Error (MAE). 

\textbf{Affordance Selection}: We have reported results for five affordances - \textit{Red light}, \textit{Hazard Stop}, \textit{Relative Angle}, \textit{Centerline Distance} and \textit{Vehicle Distance}. Considering the setup of our dataset collection, from Figure \ref{fig:distrib}, we can observe that the two affordances \textit{Speed Sign} and \textit{Hazard Stop} suffer from class imbalance.

In case of Speed Sign, only 1.5\% of the entire data belongs to other classes of speed signs (0.7\% 30kmph, 0.4\% 60kmph and 0.3\% 90kmph), and are hence predicted incorrectly by the driving model trained on the whole dataset. The predicted accuracies of each class from the test set are as follows: 98.99\% for \textit{None}, 0.0\% for \textit{30kmph}, 100.0\% for \textit{60kmph} and 0.0\% for \textit{90kmph}. Owing to this reason, we refrain from reporting accuracies on this affordance. Alongside, prediction accuracy of this affordance does not have an impact on episode completion.


% Table \ref{speedacc} shows the predicted accuracies of each class from the test set which comprises of 0.4\% 30kmph , 0.2\% 60kmph, 0.04\% as 90kmph and the remaining as \textit{None}. 

\textbf{Multi-task criteria}: Autonomous vehicles need a high level of understanding of the environment it needs to interact with. There are multiple criteria/tasks to be considered while reaching a destination or in other words, completing an episode. Conditional Affordance Learning \cite{sauer2018conditional} has considered six of such tasks or affordances in its driving model. The affordance \textit{Relative Angle} is the orientation of the car with respect to the road and decides the steer value of the agent vehicle. Hence, this affordance becomes critical in episode completion. However, we notice a large skew in the distribution of affordances in Figure \ref{fig:distrib}b which essentially portrays the importance of selection of instances from the minority buckets (turn buckets) for the end-task of driving. There is also no established end-to-end connection between the selection of affordances and a successful episode. Therefore, this comes out as a challenge in selecting affordances for a chosen subset which will be significant in episode completion.

\subsection{Comparison of approximate online subset selection methods}

\vspace{-2.7mm}
\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/conv_prl_subm_syn_rename_again.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:synbox}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
     \centering
     \includegraphics[width=\textwidth,height=2.5cm]{figures/conv_prl_subm_real_rename.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:realbox}
    \caption{}
     \end{subfigure}
     \caption{\textbf{Objective function values for proposed method , \cite{das2020multi} method and Submodular method for (a) Synthetic data (b) CARLA driving data samples}}
     \label{fig:convsub}
 \end{figure}  
% We compare the performance of the online subset selection methods empirically in terms of their objective function values. 
% We show in Figure \ref{fig:convsub} the objective function values for the proposed method, \citep{das2020multi} method and the submodular approach \citep{buchbinder2014submodular}. For the synthesized data, we generated 10 random samples of dimension $100 \times 100$. Since the submodular approach is a randomized algorithm, we made 100 runs for each sample and show a box plot of the submodular method's objective function values. 

In this section, we compare the optimal subsets reported by the baseline method \cite{das2020multi}, submodular method and the proposed convex optimization based method in terms of final objective function values. 
Figure \ref{fig:convsub}a shows the objective function values for the three approaches, for 10 randomly synthesized problem instances ($d$ matrix of dimension $100\times 100$ and $L$ vector of dimension $100$ in equations \ref{eq:joint}, \ref{eq:submod} , \ref{eqn:newsiftloss}). For the submodular method, we report a box plot of results over 100 runs of the algorithm to capture the randomness. While all three methods find approximate solutions, the proposed convex method consistently finds lower values of objective function, followed by \cite{das2020multi}, and submodular optimization. For real data (CARLA data for our further experiments), we report the same in Figure \ref{fig:convsub}b , for 10 episodes in our collected data. We can clearly observe that function values attained by our proposed method lies below that of the other approximate methods, thus proving our method to be an efficient approach. 

We show in Table \ref{tab:inctime} the impact of online selection on the objective function values. We observe the change in objective function values across increasing time-steps. The values show a gradual decline with increasing time-steps which affirms the efficiency of the online paradigm.

% We show in Figure \ref{fig:rhoPRL} the change in objective function values with variation in $\rho$. We can observe that the pointwise metric has a very. When the pointwise metric is given the entire weightage ($\rho = 0 $), only 1 representative gets selected from the existing or incoming set, whichever yields the highest value, irrespective of the compression ratio. The consistent difference in objective function values between \citep{das2020multi} and the proposed method mark the efficiency of the proposed method and also brings out empirically one of the drawbacks of \citep{das2020multi}.


% We can observe that the gap in objective function values between \citep{das2020multi} and the proposed method decreases with increase in $\rho$ which marks higher weightage on pairwise metric. However, . Thus, this brings out empirically one of the drawbacks of \citep{das2020multi} explained in Section \ref{sec:subset}.

% We also reported in Table \ref{tab:measure} the mean \% difference between the objective function values of convex and submodular approach, and the mean time taken to optimise the synthesized data samples.

\begin{table}[]
\footnotesize
\caption{\textbf{Objective function values for proposed method on CARLA driving data with increasing time sequence}}
\label{tab:inctime}
\begin{tabular}{|l|l|l|l|l|}
\hline
Time Sequence                                                       & t = 1 & t = 2 & t = 3 & t = 4 \\ \hline
\begin{tabular}[c]{@{}l@{}}Objective function\\ values\end{tabular} & 0.127 & 0.11  & 0.106 & 0.105 \\ \hline
\end{tabular}
\end{table}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.45\columnwidth,height=2.5cm]{figures/seq_time.pdf}
%      \caption{\textbf{Objective function values for proposed method on CARLA driving data with increasing time sequence}}
%      \label{fig:inctime}
%  \end{figure}


% \vspace{-2.7mm}
% \begin{figure}[h!]
%     \centering
%     %\caption{\textbf{Objective function values for proposed function , PRL function and submodular function for (a) Synthetic data (b) CARLA driving data samples}}
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/seq_time.pdf}
%     % \caption{\textbf{Objective function values for our proposed function on incoming set of CARLA driving data in sequence of time}}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:inctime}
%     %\caption{}
%     \end{subfigure}
%     \hspace{1mm}
%     \begin{subfigure}{0.45\columnwidth}
%      \centering
%      \includegraphics[width=\textwidth,height=2.5cm]{figures/rho_var_MCL.pdf}
%     %  \caption{\textbf{Objective function values for our proposed function and PRL function on Synthetic data sample with variation of $\rho$}}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:rhoPRL}
%     %\caption{}
%      \end{subfigure}
%      \caption{(a)\textbf{Objective function values for proposed method on CARLA driving data in sequence of time} (b) \textbf{Objective function values for proposed method and \citep{das2020multi} on synthetic data sample with variation of $\rho$.}}
%      \label{fig:incrho}
%  \end{figure}

% \begin{figure}[h!]
%     \centering
%     \caption{\textbf{Objective function values for our proposed function on incoming set of CARLA driving data in sequence of time}}
%     \includegraphics[width=0.5\columnwidth,height=2.5cm]{figures/seq_time.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:inctime}
% \end{figure}

Next, we discuss the application of the subset selection methods on autonomous driving.

% \begin{figure}[h!]
%     \centering
%     \caption{\textbf{Objective function values for our proposed function and PRL function on Synthetic data sample with variation of $\rho$}}
%     \includegraphics[width=0.5\columnwidth,height=2.5cm]{figures/rho_var_PRL.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:rhoPRL}
% \end{figure}




% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{left}) 100:20 , (\textit{middle}) 100:7, (\textit{right}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure*}

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
    
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_20.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_20.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redllight_15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turn_15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_3.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_3.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7, (\textit{bottom}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure}

% In case of Hazard Stop, only 0.5 \% of data has presence of hazard stops, while test set has none. Overall, all the methods are able to predict the majority class (i.e no hazard stop) leading to an accuracy close to 100\%. In order to avoid the trivial case, we exclude this affordance from our results.



% \tr{Speed sign: Only about 1\% (0.5\% 30kmph, 0.1\% 60kmph and 0.3\% 90kmph) of the data belongs to other speed signs which are all predicted wrongly by the CAL model even with full dataset. Prediction accuracy of this affordance also does not affect episode completion. (give classwise accuracy and number of data points.) \\
% Hazard stop: The data has extreme skew only 0.6\% of the training data has hazard stop as true and there are no test instances with this.\\}
% \subsection{Comparison of data gradation methods with Whole Set}

% In this section, we provide a summary of results enlisting the best method from the two sets of experiments that we perform while comparing selection methods with whole set - episode completion and affordance prediction. 

% We consider four tasks under episode completion which had been originally defined in \cite{dosovitskiy2017carla}:
% \begin{enumerate}
%     \item Straight : The episode comprises of points which is a straight road.
%     \item One-Turn : The episode comprises of points which include a left or right turn in its path.
%     \item Straight Dynamic : It is similar to Straight task in the presence of other vehicles and pedestrians.
%     \item One-Turn Dynamic : It is similar to One-Turn task in the presence of other vehicles and pedestrians.
% \end{enumerate}

% In table \ref{tab:epsumm}, we show the best performing method for each task under episode completion along with the number of successfully completed episodes and its difference with that of the whole set. We can observe that the method SLN completes the most number of episodes (out of a total of 10 episodes) among all other gradation methods. It fails for only 33\% episodes in the difficult task of taking turns. The detailed results on episode completion is explained in the next subsection.




% \begin{table*}[]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in training conditions}}
% \label{tab:trainepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{l|}{Straight}                                                                                                                                               & \multicolumn{3}{l|}{One-Turn}                                                                                                                                             & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set Episode Completion Count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{9}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{9}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SLO/\\ SLN\end{tabular} & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   & \begin{tabular}[c]{@{}l@{}}SIFT/\\ SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   \\ \hline
% 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   \\ \hline
% 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 1                                                       & 88.88                                                   & SLN                                                   & 10                                                      & 0                                                       & SLO                                                   & 1                                                       & 88.88                                                   \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in testing conditions}\tr{Combine this with the training table}}
% \label{tab:testepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{l|}{Straight}                                                                                                                                             & \multicolumn{3}{l|}{One-Turn}                                                                                                                                             & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set Episode Completion Count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   & \begin{tabular}[c]{@{}l@{}}SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% 100:7                                                                        & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 2                                                       & 71.42                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% 100:3                                                                        & SLN                                                   & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLN\end{tabular}    & 1                                                       & 85.71                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   \\ \hline
% \end{tabular}
% \end{table*}

% In table \ref{tab:relsumm}, we show the best method for each compression ratio under the respective relative angle buckets along with its difference with that of whole set.  We explicitly focus on the relative angle affordance since it is a key factor in episode completion. We can observe that SLN turns out as the best performing method for the turn buckets while Uniform Skip turns out the best for Straight road. This can be attributed to the observation we made where SLN turned out as the best method in episode completion task. We have given a detailed analysis on the affordance predictions in the next subsections.




% \begin{table*}[]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in training conditions}}
% \label{tab:trainepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{9}{|c|}{Episode Completion Tasks}                                                                                                                                                                                                                                                                                                                                  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{2}{c|}{Straight}                                                        & \multicolumn{2}{c|}{One-Turn}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Straight \\ Dynamic\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}} \\ \cline{2-9} 
%                                                                              & Best Method                                                             & Difference & Best Method             & Difference & Best Method                                & Difference                          & Best Method                             & Difference                            \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SIFT+Loss-O/\\ SIFT+Loss-N\end{tabular} & 0          & SIFT+Loss-N             & 3          & SIFT/SIFT+Loss-N                           & 0                                   & SIFT+Loss-N                             & 3                                     \\ \hline
% 100:7                                                                        & SIFT+Loss-N                                                             & 0          & SIFT+Loss-N             & 6          & SIFT+Loss-N                                & 0                                   & SIFT+Loss-N                             & 6                                     \\ \hline
% 100:3                                                                        & SIFT+Loss-N                                                             & 0          & SIFT+Loss-O/SIFT+Loss-N & 8          & SIFT+Loss-N                                & 0                                   & SIFT+Loss-O                             & 8                                     \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in testing conditions}}
% \label{tab:testepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{9}{|c|}{Episode Completion Tasks}                                                                                                                                                                                                                                                                                                                             \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{2}{c|}{Straight}                                                   & \multicolumn{2}{c|}{One-Turn}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Straight \\ Dynamic\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}} \\ \cline{2-9} 
%                                                                              & Best Method                                                        & Difference & Best Method             & Difference & Best Method                             & Difference                             & Best Method                             & Difference                            \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT+Loss-O/\\ SIFT+Loss-N\end{tabular} & 0          & SIFT+Loss-N             & 4          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 4                                     \\ \hline
% 100:7                                                                        & SIFT+Loss-N                                                        & 0          & SIFT+Loss-N             & 5          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 5                                     \\ \hline
% 100:3                                                                        & SIFT+Loss-N                                                        & 0          & SIFT+Loss-O/SIFT+Loss-N & 6          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 6                                     \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \label{tab:relsumm}
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for relative angle affordance prediction}}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{6}{c|}{Relative Angle buckets}                                                                                                                                                                                                                                                                                                                     \\ \cline{2-7} 
%                                                                              & \multicolumn{2}{c|}{Left-Turn}                                                                                      & \multicolumn{2}{c|}{Straight-Road}                                                                                  & \multicolumn{2}{c|}{Right-Turn}                                                                                     \\ \cline{2-7} 
%                                                                              & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} \\ \hline
% 100:20                                                                       & SIFT                             & 0.02                                                                             & Uniform Skip                     & 0.01                                                                             & SIFT+Loss-N                      & 0.01                                                                             \\ \hline
% 100:7                                                                        & SIFT                             & 0.03                                                                             & Uniform Skip                     & 0.01                                                                             & SIFT+Loss-N                      & 0.01                                                                             \\ \hline
% 100:3                                                                        & SIFT+Loss-N                      & 0.06                                                                             & SIFT+Loss-O                      & 0.02                                                                             & SIFT+Loss-N                      & 0.02                                                                             \\ \hline
% \end{tabular}
% \end{table*}
% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:20 compression ratio}}
% \label{tab:ep5}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 3                                                          & 8        & 3                                                          & 9        & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
%                                                                              & Only SIFT                                                   & 10       & 7                                                          & 10       & 7                                                          & 10       & 7                                                          & 9        & 6                                                          \\ \cline{2-10} 
%                                                                             & Only Loss                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & PRL                                                    & 9        &  8                                                         & 9        & 8                                                          & 7       &  7                                                         & 7        & 7                                                          \\ \cline{2-10} 
%                                                     & SubM                                                    & 9        &  7                                                         & 9        & 7                                                          & 9       &  7                                                         & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & STL                                                    & 10       & 8                                                         & 10       & 7                                                          & 10       & 9                                                          & 10       & 9 
%                                 \\ \cline{2-10} 
%                                                                              & SML                                                    & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       &\textbf{10}                                \\        \hline
% % \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 2                                                          & 8        & 2                                                          & 9        & 3                                                          & 7        & 3                                                          \\ \cline{2-10} 
% %                                                                              & SIFT                                                   & 9        & 4                                                          & 9        & 4                                                          & 8        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
% %                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         &                                                           \\ \cline{2-10} 
% %                                                                              & SLN                                                    & 10       & \textbf{6}                                                          & 10       & \textbf{6}                                                          & 10       & \textbf{8}                                                          & 10       & \textbf{8}                                                          \\ \hline
% % \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 1                                                          & 8        & 0                                                          & 9        & 2                                                          & 8        & 2                                                          \\ \cline{2-10} 
% %                                                                              & SIFT                                                   & 8        & 0                                                          & 8        & 0                                                          & 8        & 1                                                          & 9        & 0                                                          \\ \cline{2-10} 
% %                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         & 0                                                          \\ \cline{2-10} 
% %                                                                              & SLN                                                    & 10       & \textbf{5}                                                          & 10       & \textbf{5}                                                          & 10       & \textbf{6}                                                          & 9       & \textbf{6}                                                          \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:7 compression ratio}}
% \label{tab:ep15}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:7}                                                      & \begin{tabular}[c]{@{}l@{}}Only SIFT\end{tabular} & 9        & 5                                                          & 9        & 5                                                           & 9        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
%                                                                             & Only Loss                                                   & 10        & 6                                                          & 10       & 6                                                          &    9    & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & PRL                                                    & 9        & 5                                                            & 9        & 5                                                          & 7        &  4                                                         & 7        & 4                                                          \\ \cline{2-10}
%                                                                              & SubM                                                    & 9        & 3                                                            & 9        & 3                                                          & 9        & 2                                                          & 9        & 2                                                          \\ \cline{2-10}
%                                                                              & STL                                                    & 10       & 7                                                          & 10        & 7                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}  
%                                 \\ \cline{2-10} 
%                                                                              & SML                                                    & 10       & \textbf{8}                                                           & 10       & \textbf{8}                                                          & 10       &\textbf{9}                                                           & 10       & \textbf{9}                                 \\        \hline
% \end{tabular}
% \end{table*}

\begin{table*}[]
%\footnotesize
\scriptsize
\centering
\captionsetup{justification=centering}
\caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:20 and 100:7 compression ratio}}
\label{tab:ep5_15}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
                                                                             &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
                                                                             & WS    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
\multirow{4}{*}{100:20}                                                      & US & 9        & 3                                                          & 8        & 3                                                          & 9        & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
                                                                             & OS                                                   & 10       & 7                                                          & 10       & 7                                                          & 10       & 7                                                          & 9        & 6                                                          \\ \cline{2-10} 
                                                                            & OL                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
                                                                             & MCL                                                    & 9        &  8                                                         & 9        & 8                                                          & 7       &  7                                                         & 7        & 7                                                          \\ \cline{2-10} 
                                                    & SBML                                                    & 9        &  7                                                         & 9        & 7                                                          & 9       &  7                                                         & 9        & 7                                                          \\ \cline{2-10} 
                                                                             & CTL                                                    & 10       & 8                                                         & 10       & 7                                                          & 10       & 9                                                          & 10       & 9 
                                \\ \cline{2-10} 
                                                                             & CBML                                                    & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       &\textbf{10}                                \\        \hline
                                                        \hline
\multirow{4}{*}{100:7}                                                      & \begin{tabular}[c]{@{}l@{}}MCL\end{tabular} & 9        & 5                                                            & 9        & 5                                                          & 7        &  4                                                         & 7        & 4                                                          \\ \cline{2-10}
                                                                             & SBML                                                    & 9        & 3                                                            & 9        & 3                                                          & 9        & 2                                                          & 9        & 2                                                          \\ \cline{2-10}
                                                                             & CTL                                                    & 10       & 7                                                          & 10        & 7                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}  
                                \\ \cline{2-10} 
                                                                             & CBML                                                    & 10       & \textbf{8}                                                           & 10       & \textbf{8}                                                          & 10       &\textbf{9}                                                           & 10       & \textbf{9}                                 \\        \hline                                                    
\end{tabular}
\end{table*}



\subsection{Comparison of Methods: Episode Completion}



In this section, we will study the performance of different subset selection techniques on the basis of episode completion which is the main intended objective.

We consider four tasks under episode completion which had been originally defined in \cite{dosovitskiy2017carla}:
\begin{enumerate}
    \item Straight : The episode comprises of pairs of points which are straight roads.
    \item One-Turn : The episode comprises of pairs of points which include left or right turn in their paths.
    \item Straight Dynamic : Similar to \textit{Straight} task, it occurs in the presence of other vehicles and pedestrians.
    \item One-Turn Dynamic : Similar to \textit{One-Turn} task in the presence of other vehicles and pedestrians.
\end{enumerate}

We show in Table \ref{tab:ep5_15} the performance of CAL model\cite{sauer2018conditional}  trained on subsets, obtained by various selection techniques, by simulating it with the CARLA \cite{dosovitskiy2017carla} simulator.


We report number of successfully completed episodes (out of a total of 10 episodes) for each subtask in training and test conditions. We observe that the tasks - \textit{Straight} and \textit{Straight Dynamic} are fairly easy to accomplish for all subset selection methods. The challenge arises in the other two tasks where we see a large number of unsuccessful episodes.

The completion of episodes in turns, largely depends on the affordance \textit{Relative Angle} which as we mentioned, provides the steering angle of the agent vehicle. We observe that Uniform Skip (US) is unable to complete majority of the turns in training or test conditions. This is due to the inherent nature of selection of US method, which does not take the important frame sequences into consideration.


\begin{figure*}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/deviation_dist_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/turn_123_26.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \caption{}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/turn_94_31.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    \centering
    \begin{subfigure}{0.4\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_r1_MCL_New.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.4\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_r25_e1_MCL_New.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    % \centering
    % \begin{subfigure}{0.4\columnwidth}
    % \centering
    % % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_r4_e1_MCL_New.pdf}
    % %\caption{Red light Affordance Distribution}
    % \caption{}
    % \label{fig:tskip5}
    % \end{subfigure}
    \centering
    \begin{subfigure}{0.4\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_r1_e2_MCL_New.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.4\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_r25_e2_MCL_New.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    % \centering
    % \begin{subfigure}{0.4\columnwidth}
    % \centering
    % % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_r4_e2_MCL_New.pdf}
    % %\caption{Red light Affordance Distribution}
    % \caption{}
    % \label{fig:tskip5}
    % \end{subfigure}
    \caption{\textbf{Fraction of selected instances for sample episodes (a) and (b) with turns in figures (c), (d), and (e), (f) for $\rho = \{0.1 , 0.25\}$ respectively. The proposed method selects more fraction of instances from the area with turns, which becomes crucial for the task of episode completion.}}
    \label{fig:deviate}
\end{figure*}


% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/relangle_episode.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/relloss_episode.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{A temporal plot of an episode with (a) the relative angle affordance value (b) its corresponding relative angle loss values in the respective frames.}}
%     \label{fig:lossrel}
% \end{figure}
%\vspace{-1mm}
\begin{figure*}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/deviation_dist_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/deviation_episode_error_MCL_whole_label.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \caption{}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/deviation_episode_error_MCL_whole.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_MCL.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{Anecdotal example of a sample episode showing (a) the region of failure by MCL (b) the corresponding errors and (c) fraction of selected instances from those regions. CBML selects more fraction of instances from regions important for episode completion.}}
    \label{fig:deviate}
\end{figure*}
% One of the 

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
    
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_20.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_20.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redllight_15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turn_15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_3.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_3.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7, (\textit{bottom}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure}

On the other hand, OS, OL, MCL, SBML complete some of the turn episodes, with CBML completing the highest of all methods (100\% both in training and test conditions) followed by CTL. This is due to the consideration of pointwise metric - bucketwise relative angle aided with remaining multi task losses in Equation \ref{eqn:newsiftloss} along with pairwise metric SIFT dissimilarity, which leads to the selection of important frames. We also report the episode completion numbers for 100:7 compression ratio in Table \ref{tab:ep5_15}, for two baselines - MCL and SBML and the proposed method. We can observe that CTL and CBML continue to perform better compared to the other baselines with CBML completing 80\% and 90\% episodes in training and test conditions even after dropping 93\% of the frames.

% As mentioned under Multi-task criteria, we observe that Relative Angle affordance turns out to be vital in the task of episode completion. We can divide the entire range of Relative Angle affordance value across 20 buckets ranging from -1.0 to +1.0. Note that buckets corresponding to (-1.0 to -0.1) and (0.1 to 1.0) approximately indicate the left and right turns. 

% In Figure \ref{fig:lossrel}, we show an entire sequence of frames of an episode with its corresponding \textit{Relative Angle} affordance value and its respective loss value.  As seen from the figure, which is one of the left turn episodes, we can notice the higher relative angle loss values at the turn. This essentially shows us the need for selection of such frames in order to have successful episodes. So, using the above intuition, we fine-tune the weights corresponding to the bucket-wise relative angle loss values and feed in our subset selection framework SML.


% One of the possible reasons of success can be attributed to Figure \ref{fig:bucketprop5} where we see that SML has a higher fraction of selected instances for most of the buckets than all other methods which essentially portrays its effectiveness. Only Loss also selects fairly large fraction of instances for some of the buckets. However, it only concentrates on the frames which incur a high loss value. The completion of an episode relies on various other factors like perceptual difference and having only frames with high end-task losses in the compressed sequence does not lead to an effective result.


We show an anecdotal example of a failed episode from MCL \cite{das2020multi} method in Figure \ref{fig:deviate} and try to analyse the reason behind it. In Figure \ref{fig:deviate}a, we show a plot of an episode with distance covered vs Relative Angle affordance. The cumulative distance is chosen as an axis of reference in order to make the comparison spatially similar for all the methods. Overall, the agent vehicle in the simulator is resilient to errors. However, we can observe the gradual deviation of MCL \cite{das2020multi} method and its accumulated errors which lead to an incomplete episode. We can also relate the region of failures to the corresponding relative angle errors in Figure \ref{fig:deviate}b where we observe that overall, MCL \cite{das2020multi} is having a higher error compared to proposed method CBML and model trained on the whole set. This occurs because we fine-tune the weights corresponding to the bucket-wise relative angle loss values and feed in our subset selection framework CBML along with pairwise metric. We also show the fraction of selected instances by both the selection methods, in Figure \ref{fig:deviate}c from the same region, and we can observe that CBML selects more fraction of instances in the area right before the turn and during the turn, which eventually help in its completion.
We discuss the next subtask - affordance prediction in the following subsection.



% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_left.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_straight.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_right.pdf}
    
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for subset selection methods for 100:20 compression ratio}}
%     \label{fig:fracall}
% \end{figure*}


% We show in Figure \ref{fig:deviate} three instances of the points of deviation where three of the baselines - Only SIFT, Only Loss and PRL fail in completing their respective episodes. The buckets correspond to the areas in the town where the models trained using Only SIFT, Only Loss and PRL had deviated leading to incomplete episode. We can clearly observe that the error corresponding to SML and STL are considerably lower which make them reach the end goal.

% We show in Figure \ref{fig:deviate} three instances of the points of deviation where three of the baselines - Only SIFT, Only Loss and PRL fail in completing their respective episodes. We have run the simulator using the ground truth affordances and the individual trained model's predicted affordances. We kept a track of the predicted relative angle along with the covered cumulative distance. Note that the change in relative angle values (y-axis) arise when turns appear. We can observe in both the plots, that the agent vehicle started deviating more using the Only Loss and PRL method right before turns, leading to intersection with the sidewalk thus failing to complete the episode.  The points immediately before the turn are important for consideration since those mark the intersecting points or junctions. We can see in both the plots that our gradation method - STL and SML appear to predict values closer to the ground truth during the intersection points while Only Loss (left) and PRL (right) methods  begin deviating at the intersections leading to failures. The loss values in these buckets (-0.1 to 0.1) are not considerably higher due to presence of large number of training samples in these buckets since the relative angle values for the straight roads also fall in them. Hence, Only Loss selects lesser number of instances from these buckets leading to failure.  On the other side, PRL takes SIFT and Loss into consideration, but due to its drawback as described in section, it also fails in completing all the turns. Both SML and STL take pairwise and pointwise metric into consideration during selection of frames and result in more successful episodes. SML performs better than STL due to the inclusion of SIFT and weighted losses which help in selection of more important frames. 
% A wrong prediction in relative angle at certain points may take the vehicle to waypoints from which recovering back without manual intervention would not be possible.
% STL even though predicts closer to ground truth values than SML at the junctions, yet it is not able to complete all the episodes since the turns after the intersection is vital too and we can observe in the plots that STL predicts better at those.
% It can also be seen that the number of successfully completed episodes with STL is considerably less than SML but reasonably better than the other methods. The consideration of both pairwise and pointwise metric (total loss) lead to its better selection of frames, however the weighted multi-task loss has led to an added benefit.
% Note that 100:7 and 100:3 is very high in comparison to the 63000 frames dataset we collected. The original model \cite{sauer2018conditional} was trained on 10x amount of data we have used in our experiments. We expect that the successful completion rate will increase with increasing dataset size.

% We have also performed experiments on the subset selection method using only relative angle loss as the pointwise metric, to which it did not yield good results. One potential future work can be to use different components of the six affordance losses and weighing them according to its importance in episode completion. 

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 97.39                                                                     & 97.41                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 96.72                                                                     & 97.03                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & Only SIFT                                                   & 96.11                                                                     & 96.07                                                                     &                                                          &                                                          \\ \cline{2-6}
%                         & Only Loss                                                   & 92.31                                                                     & 91.08                                                                     &                                                          &                                                          \\ \cline{2-6}
%                         & PRL                                            &  91.63                                                                    & 89.73                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & STL                                            & 96.38                                                                     & 96.05                                                                     &                                                          &
%                       \\ \cline{2-6} 
%                         & SML                                            & 93.98                                                                     & 92.83                                                                     &                                                          &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 92.63                                                                     & 91.94                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 89.55                                                                     & 87.23                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 94.72                                                                      & 94.54                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 97.12                                                                     & 97.04                                                                      &                                                          &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.06                                                                     & 93.09                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 94.16                                                                     & 93.54                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 90.12                                                                     & 94.41                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 94.42                                                                      & 93.72                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \label{tab:redlaff}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Method                                              & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                             & WS                                                  & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                     & US                                                  & 96.72                                                    & 97.03                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 96.11                                                    & 96.07                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 92.31                                                    & 91.08                                                    \\ \cline{2-4} 
%                                                             & PRL                                                 & 91.63                                                    & 89.73                                                    \\ \cline{2-4} 
%                                                             & STL                                                 & 96.38                                                    & 96.05                                                    \\ \cline{2-4} 
%                                                             & SML                                                 & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \label{tab:hazaff}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Method                                              & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                             & WS                                                  & 99.44                                                    & 99.72                                                    \\ \hline
% \multirow{6}{*}{100:20}                                     & US                                                  & 99.14                                                    & 99.47                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     \\ \cline{2-4} 
%                                                             & PRL                                                 & 99.43                                                    & 98.39                                                    \\ \cline{2-4} 
%                                                             & STL                                                 & 99.31                                                    & 99.61                                                    \\ \cline{2-4} 
%                                                             & SML                                                 & 99.45                                                    & 99.71                                                    \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
% \label{tab:redrhazaff}
% \begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                                              & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
%                                                                              & PRL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
%                         & SubM                                                 & 99.25                                                    &                                                     & 94.33                                                    &                                                     \\ \cline{2-6}                                                     & STL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
%                                                                              & SML                                                 & 99.45                                                    & \begin{tabular}[c]{@{}l@{}}99.71\\ (1.32\%)\end{tabular}                                           & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{table}




% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 99.44                                                                     & 99.72                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.14                                                                     & 99.47                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & Only SIFT                                                   & 99.11                                                                     & 99.56                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & Only Loss                                                   & 99.41                                                                     & 99.6                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & PRL                                            & 99.43                                                                     & 98.39                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLT                                            & 99.23                                                                     & 99.61                                                                     &                                                          &
%                         \\ \cline{2-6} 
%                         & SLM                                            & \textbf{99.45}                                                                     & \textbf{99.71}                                                                     &                                                          &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.42                                                                     & 97.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 99.31                                                                     & 98.99                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 99.39                                                                      & 98.37                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 99.45                                                                     & 98.76                                                                      &                                                          &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 98.57                                                                     & 97.67                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 99.29                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 99.39                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 99.12                                                                      & 98.23                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:hazaff}
% \end{table}
% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|p{12mm}|p{8mm}|l|p{15.5mm}|l|p{15.5mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & MAE           & \%Improvement         & MAE            & \%Improvement           \\ \cline{3-6} 
%                                                                              &                                                        & \multicolumn{2}{l|}{Vehicle Distance} & \multicolumn{2}{l|}{Centerline Distance} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.03          &                       & 0.05           &                         \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.05           &                         \\ \cline{2-6} 
%                                                                              & Only SIFT                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6}
%                                                                              & Only Loss                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6}
%                                                                              & PRL                                                    & 0.05          &                   & 0.06           &                    \\ \cline{2-6} 
%                                                                              & SLT                                                    & 0.05          & 44.44                  & 0.05           & 37.5
%                                           \\ \cline{2-6} 
%                                                                              & SLM                                                    & \textbf{0.04}          &    55.55               & 0.05           & 37.5                                  
%                                                                              \\ \hline
% % \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.06           &                         \\ \cline{2-6} 
% %                                                                              & SIFT                                                   & 0.09          &                 & 0.08           &                      \\ \cline{2-6} 
% %                                                                              & SLO                                                    & 0.09          & 0.09                 &            &                      \\ \cline{2-6} 
% %                                                                              & SLN                                                    & 0.07          &                   & 0.06           &                     \\ \hline
% % \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.07          &                       & 0.09           &                         \\ \cline{2-6} 
% %                                                                              & SIFT                                                   & 0.11          &                  & 0.08           &                     \\ \cline{2-6} 
% %                                                                              & SLO                                                    & 0.09          & 0.09                 &            &                      \\ \cline{2-6} 
% %                                                                              & SLN                                                    & 0.06          &                  & 0.06           &                     \\ \hline
% \end{tabular}
% \end{table}




%\tr{TBD}

% \begin{table}[]
% \begin{tabular}{|l|p{2mm}|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ratio\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\\ (Macro)\end{tabular}}                   & \multicolumn{4}{c|}{MAE}                                                                                                                                                                                \\ \cline{3-8} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}CAL\\ RL\end{tabular}        & \begin{tabular}[c]{@{}l@{}}TS\\ RL\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ CD\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ CD\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                       &                                                                              & \begin{tabular}[c]{@{}l@{}}95.86\\ (95.16)\end{tabular} & \begin{tabular}[c]{@{}l@{}}95.86\\ (95.16)\end{tabular}                                               &\begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05 \end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                                 & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                                \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:20}}                                 &
% \begin{tabular}[c]{@{}l@{}}95.32\\ (94.7)\end{tabular} & \begin{tabular}[c]{@{}l@{}}95.54\\ (94.82)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.06\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}91.36\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                &                                                  &                                                &                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}89.18\\ (87.25)\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}}90.52 \\(88.26)\end{tabular}                                                & 0.07                                                 & 0.06                                                & 0.09                                                 & 0.10                                                \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:7}}                                 & \begin{tabular}[c]{@{}l@{}}91.94 \\ (91.08)\end{tabular} & \begin{tabular}[c]{@{}l@{}}94.58\\ (95.02)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.10\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8}
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}90.28\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 

% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}89.7\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.08                                                 &                                                 & 0.11                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}85.76\\ (83.67)\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.07                                                 &                                                 & 0.11                                                &                                                 \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:3}}                                 & \begin{tabular}[c]{@{}l@{}} 91.72\\ (91.27)\end{tabular} & \begin{tabular}[c]{@{}l@{}}93.58\\ (92.60)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}} 0.06\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}} 0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8}
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}90.04\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.10\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}87.68\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.08                                                 &                                                 & 0.12                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                &                                                  &                                                 &                                                 &                                                 \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques in terms of affordance accuracies}
% \label{afftable}
% \end{table}

% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.15                                                      & 0.02                                                          & 0.08                                                       & 0.09                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                              & 0.08                                                           & 0.07                                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 95.32                                                    & 94.7                                                     & 0.39                                                      & 0.03                                                          & 0.09                                                       & 0.09                                                          & 95.54                                                    & 94.82                                                    & 0.28                                                          & 0.03                                                              & 0.07                                                           & 0.09                                                          \\ \hline
% SIFT                                                                               & 91.36                                                    & 88.12                                                         & 0.17                                                      & 0.06                                                          & 0.09                                                       & 0.09                                                          & 91.9                                                         & 90.75                                                         & 0.16                                                          & 0.05                                                              & 0.14                                                           & 0.09                                                              \\ \hline
% SIFT+Loss-O                                                                        & 88.34                                                         & 86.96                                                         & 0.19                                                      & 0.07                                                          & 0.08                                                       & 0.09                                                              & 89.94                                                         & 87.79                                                         & 0.17                                                          & 0.04                                                              & 0.08                                                           & 0.08                                                              \\ \hline
% SIFT+Loss-N                                                                        & 89.18                                                    & 88.25                                                    & 0.18                                                      & 0.05                                                          & 0.07                                                       & 0.09                                                          & 90.52                                                    & 89.26                                                    & 0.16                                                          & 0.05                                                              & 0.08                                                           & 0.08                                                          \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:20}
% \label{afftable1}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.19                                                      & 0.03                                                          & 0.08                                                       & 0.08                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                              & 0.08                                                           & 0.07                                                               \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 91.94                                                    & 91.08                                                     & 0.38                                                      & 0.04                                                          & 0.11                                                       & 0.11                                                          & 94.58                                                    & 95.02                                                    & 0.27                                                          & 0.04                                                              & 0.09                                                           & 0.10                                                          \\ \hline
% SIFT                                                                               & 90.28                                                    & 90.1                                                         & 0.18                                                     & 0.06                                                          & 0.14                                                       & 0.11                                                          & 90.1                                                         & 88.58                                                         & 0.17                                                           & 0.05                                                              & 0.16                                                           & 0.09                                                              \\ \hline
% SIFT+Loss-O                                                                        & 89.7                                                         & 89.8                                                         & 0.19                                                      & 0.05                                                          & 0.13                                                       &  0.11                                                             & 91.76                                                         & 91.4                                                         & 0.21                                                          & 0.05                                                              & 0.11                                                           & 0.11                                                              \\ \hline
% SIFT+Loss-N                                                                        & 87.04                                                    &                                                     & 0.21                                                      & 0.10                                                          & 0.06                                                       & 0.12                                                          & 91.32                                                    &                                                     & 0.19                                                          & 0.08                                                              & 0.06                                                           & 0.14                                                          \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:7}
% \label{afftable2}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.19                                                      & 0.03                                                          & 0.08                                                       & 0.08                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                               & 0.08                                                           & 0.07                                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 91.26                                                    & 90.36                                                      & 0.44                                                      & 0.6                                                          & 0.15                                                       & 0.11                                                          & 93.58                                                    & 92.60                                                    & 0.32                                                          & 0.05                                                              & 0.09                                                           & 0.11                                                          \\ \hline
% SIFT                                                                               & 90.04                                                    & 90.34                                                         & 0.32                                                     & 0.06                                                          & 0.15                                                       & 0.11                                                          & 91.87                                                         & 89.02                                                         & 0.28                                                          & 0.05                                                              & 0.14                                                           &  0.09                                                             \\ \hline
% SIFT+Loss-O                                                                        & 87.68                                                         & 88.54                                                         & 0.26                                                      & 0.05                                                          & 0.16                                                       & 0.11                                                              & 91.36                                                         & 90.78                                                         & 0.23                                                          & 0.07                                                              & 0.11                                                           & 0.13                                                              \\ \hline
% SIFT+Loss-N                                                                        & 86.08                                                    & 85.54                                                    & 0.22                                                      & 0.08                                                          & 0.06                                                       & 0.13                                                          &                                                     &                                                     &                                                           &                                                               &                                                            &                                                           \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:3}
% \label{afftable3}
% \end{table*}




% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ratio\end{tabular}} & \multirow{2}{*}{Tasks}                                     & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Train\\ Poses\end{tabular}}                               & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Poses\end{tabular}}                                \\ \cline{4-7} 
%                                                                           &                                                                              &                                                            & \begin{tabular}[c]{@{}l@{}}CAL\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ Model\end{tabular} \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}}      & \multirow{4}{*}{}                                                            & Straight                                                   & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 9                                                    &                                                    & 7                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 8                                                    &                                                    & 7                                                    &                                                    \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:20}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 0                                                    & 0                                                   & 1                                                    & 0                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &  8                                                   & 9                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 0                                                    & 0                                                   & 1                                                    & 0                                                   \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 2                                                    &                                                    & 1                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    &                                                    & 9                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 2                                                    &                                                    & 1                                                    &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &  10                                                   & 9                                                   & 10                                                    & 9                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 9                                                   & 9                                                    & 8                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   & 10                                                    & 10                                                   & 10                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 6                                                    &                                                    & 3                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    & 10                                                   & 10                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 6                                                    &                                                    & 3                                                    &                                                    \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:7}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 10                                                   & 7                                                     & 10                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\
                                    
%                                 \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:3}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 9                                                   & 8                                                    & 9                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
                                                                          
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\
%                                     \hline
% \end{tabular}
% \label{eptable}
% \end{table}





% \begin{table*}[h!]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training conditions}}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Episodes}                             \\ \cline{3-6} 
%                                                                              &                          & Straight & One-Turn & Straight Dynamic & One-Turn Dynamic \\ \hline
%                                                                              & Whole Set                & 10       & 9        & 10               & 9                \\ \hline
% \multirow{4}{*}{100:20}                                                      & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 10       & 2        & 10               & 2                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 10       & 3        & 8                & 2                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 6        & 10               & 6                \\ \hline
% \multirow{4}{*}{100:7}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 9        & 2        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 2        & 9                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 3        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:3}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8         & 1        & 8                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 8                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10         & 1         & 10                 & 0                 \\ \hline
% \end{tabular}
% \label{tab:eptabletrain}
% \end{table*}


% \begin{table*}[h!]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in test conditions}}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Episodes}                             \\ \cline{3-6} 
%                                                                              &                          & Straight & One-Turn & Straight Dynamic & One-Turn Dynamic \\ \hline
%                                                                              & Whole Set                & 10       & 7        & 10               & 7                \\ \hline
% \multirow{4}{*}{100:20}                                                      & Uniform Skip             & 9        & 1        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT                     & 10       & 1        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 10       & 2        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 3        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:7}                                                       & Uniform Skip             & 9        & 0        & 7                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8        & 1        & 8                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 9                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 2        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:3}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8         & 1        & 7                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 8                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10         & 1         & 10                 & 1                 \\ \hline
% \end{tabular}
% \label{tab:eptabletest}
% \end{table*}


\begin{table*}
\noindent\scriptsize
\begin{minipage}[b]{0.4\linewidth}
    \centering
\caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
\label{tab:redrhazaff}
\begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
                                                                             &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
                                                                             & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
\multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
                                                                             & OS & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
                                                                             & OL & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
                                                                             & MCL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
                        & SBML                                                 & 99.25                                                    & 99.60                                                    & 94.33                                                    & 93.91                                                    \\ \cline{2-6}                                                     & CTL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
                                                                             & CBML                                                 & 99.45                                                    & 99.71                                            & 93.98                                                    & 92.83                                                    \\ \hline
\end{tabular}
\end{minipage}
\hspace{2cm}
\begin{minipage}[b]{0.4\linewidth}
\caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
\label{tab:vehcen}
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
                                                                             &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
\multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
                                                                             & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
                                                                             & OS & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
                                                                             & OL & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
                                                                             & MCL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                                                    & SBML                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
                                                                            & CTL                                                 & 0.05
                                                                 &0.05                                 \\ \cline{2-4} 
                                                                             & CBML                                                 & 0.04
                                                                 &0.05                                 \\ \hline
\end{tabular}
\end{minipage}
\end{table*}


\subsection{Comparison of Methods: Affordance Accuracies}

% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
% \label{tab:redrhazaff}
% \begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                                              & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
%                                                                              & PRL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
%                         & SubM                                                 & 99.25                                                    & 99.60                                                    & 94.33                                                    & 93.91                                                    \\ \cline{2-6}                                                     & STL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
%                                                                              & SML                                                 & 99.45                                                    & \begin{tabular}[c]{@{}l@{}}99.71\\ (1.32\%)\end{tabular}                                           & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & PRL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
%                                                     & SubM                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
%                                                                             & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.05\\ (44.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \cline{2-4} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.04\\ (55.55\%)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}
% \begin{table}
% \scriptsize
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.06                                                     & 0.01                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.20                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.20                                                     & 0.04                                                     & 0.25                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.17                                                     & 0.02                                                     & 0.16                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.12                                                     & 0.02                                                     & 0.18                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.18                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.11                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.10\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \scriptsize
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:7}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (70.0\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{table}
% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.23                                                     & 0.03                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.16                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.15                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.11                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.10                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.10\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.34                                                     & 0.03                                                     & 0.17                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.18                                                     & 0.02                                                     & 0.12                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}


% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.04                                                     & 0.01                                                     & 0.07                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.21                                                     & 0.02                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.18                                                     & 0.03                                                     & 0.14                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.12                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & MCL                                                 & 0.12                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SBML                                                 & 0.08                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & CTL                                                 & 0.08 & 0.01 & 0.09                                                    \\ \cline{2-5} 
%                                                                              & CBML                                                 & \0.08 & 0.01 & 0.08 \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
                                                                       
%                                                                              & MCL                                                 & 0.30                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SBML                                                 & 0.32                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & CTL                                                 & 0.10 & 0.03                                                     & 0.09 \\ \cline{2-5} 
%                                                                              & CBML                                                 & 0.11 & 0.01 & 0.08  \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}


% \begin{table}[]
% \centering
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & PRL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
%                                                     & SubM                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
%                                                                             & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.05\\ (44.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \cline{2-4} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.04\\ (55.55\%)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \hline
% \end{tabular}
% \end{table}
% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip5_US_SLN_SIFT_1.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip15_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip30_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE for relative angle}}
%     \label{fig:bucketmae}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_15p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:7 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turns_30p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_road_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:3 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
%     %\footnotesize
%     \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance}}
%     \begin{tabular}{|c|p{0.2mm}|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.32                                                                         & 94.7                                                                          & 95.54                                                                         & 94.82                                                                         & 0.22                                                                          & 0.12                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 91.94                                                                         & 91.08                                                                         & 94.58                                                                         & 95.02                                                                         & \textbf{3.08}                                                                          & \textbf{3.94}                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 91.26                                                                         & 90.36                                                                         & 93.58                                                                         & 92.60                                                                         & 2.32                                                                          & 2.24                                                                          \\ \hline
% \multirow{3}{*}{SLO}                                          & 100:20                                                                                            & 88.34                                                                         & 86.96                                                                         & 89.94                                                                         & 87.79                                                                         & 1.6                                                                           & 0.83                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 89.7                                                                          & 89.8                                                                          & 91.76                                                                         & 91.4                                                                          & 2.06                                                                          & 1.6                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 87.68                                                                         & 88.54                                                                         & 91.36                                                                         & 90.78                                                                         & \textbf{3.68}                                                                          & \textbf{2.24}                                                                          \\ \hline
% \multirow{3}{*}{SLN}                                          & 100:20                                                                                            & 89.18                                                                         & 88.25                                                                         & 90.52                                                                         & 89.26                                                                         & 1.34                                                                           & \textbf{1.01}                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 88.04                                                                          & 88.5                                                                          & 91.32                                                                         & 89.17                                                                          & \textbf{5.28}                                                                          & 0.67                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 86.4                                                                         & 86.22                                                                         & 88.0                                                                         & 86.71                                                                         & 1.6                                                                          & 0.49                                                                          \\ \hline
                                    
% \end{tabular}
% \label{tab:redl}
% \end{minipage}
% \hspace{4cm}
% \begin{minipage}[b]{0.4\linewidth}
%     %\footnotesize
%     \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
%     \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & 16.67                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & \textbf{22.22}                                 \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.08                     & 0.06                           & \textbf{25.0}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.10                     & 0.09                           & 10.0                                 \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & \textbf{16.67}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.05                     & 0.05                           & 0.0                                 \\ \hline
% \end{tabular}
% %\caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
% \label{tab:veh}
% \end{minipage}
% \end{table*}


% \begin{table*}[]
% \footnotesize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance}}
% \centering
% \begin{tabular}{|c|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.32                                                                         & 94.7                                                                          & 95.54                                                                         & 94.82                                                                         & 0.22                                                                          & 0.12                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 91.94                                                                         & 91.08                                                                         & 94.58                                                                         & 95.02                                                                         & \textbf{3.08}                                                                          & \textbf{3.94}                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 91.26                                                                         & 90.36                                                                         & 93.58                                                                         & 92.60                                                                         & 2.32                                                                          & 2.24                                                                          \\ \hline
% \multirow{3}{*}{SLO}                                          & 100:20                                                                                            & 88.34                                                                         & 86.96                                                                         & 89.94                                                                         & 87.79                                                                         & 1.6                                                                           & 0.83                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 89.7                                                                          & 89.8                                                                          & 91.76                                                                         & 91.4                                                                          & 2.06                                                                          & 1.6                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 87.68                                                                         & 88.54                                                                         & 91.36                                                                         & 90.78                                                                         & \textbf{3.68}                                                                          & \textbf{2.24}                                                                          \\ \hline
% \multirow{3}{*}{SLN}                                          & 100:20                                                                                            & 89.18                                                                         & 88.25                                                                         & 90.52                                                                         & 89.26                                                                         & 1.34                                                                           & \textbf{1.01}                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 88.04                                                                          & 88.5                                                                          & 91.32                                                                         & 89.17                                                                          & \textbf{5.28}                                                                          & 0.67                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 86.4                                                                         & 86.22                                                                         & 88.0                                                                         & 86.71                                                                         & 1.6                                                                          & 0.49                                                                          \\ \hline
                                    
% \end{tabular}
% \label{tab:redl}
% \end{table*}


% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Relative Angle affordance}}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{3}{c|}{CAL}                                                                                                                                                         & \multicolumn{3}{c|}{Timestamp}                                                                                                                                                   & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{3-11} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.39                                                    & 0.03                                                        & 0.09                                                     & 0.28                                                    & 0.03                                                        & 0.07                                                     & 28.21                                                    & 0.0                                                         & 22.22                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.38                                                    & 0.04                                                        & 0.11                                                     & 0.27                                                    & 0.04                                                        & 0.09                                                     & \textbf{28.94}                                                    & 0.0                                                         & 18.18                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.44                                                    & 0.06                                                        & 0.15                                                     & 0.32                                                    & 0.05                                                        & 0.09                                                     & 27.27                                                    & \textbf{16.66}                                                         & \textbf{40.0}                                                      \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                                                            & 0.19                                                    & 0.07                                                        & 0.08                                                     & 0.17                                                    & 0.04                                                        & 0.08                                                     & 10.52                                                     & \textbf{3.0}                                                         & 15.38                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.19                                                    & 0.05                                                        & 0.13                                                     & 0.20                                                    & 0.05                                                        & 0.11                                                     & -5.0                                                    & 0.0                                                         & 15.38                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.16                                                     & 0.23                                                    & 0.05                                                        & 0.11                                                     & \textbf{11.53}                                                     & 0.0                                                        & \textbf{31.25}                                                      \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                                                            & 0.18                                                    & 0.05                                                        & 0.07                                                     & 0.16                                                    & 0.05                                                        & 0.07                                                     & 11.11                                                     & 0.0                                                         & 0.0                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.21                                                    & 0.07                                                        & 0.06                                                     & 0.20                                                    & 0.07                                                        & 0.05                                                     & 4.76                                                    & 0.0                                                         & 16.66                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.16                                                     &    0.22                                                 & 0.05                                                        & 0.05                                                     & \textbf{15.38}                                                     & 0.0                                                        & \textbf{68.75}                                                      \\ \hline
% \end{tabular}
% \label{tab:relative}
% \end{table*}

% \begin{table}[]
% \footnotesize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & 16.67                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & \textbf{22.22}                                 \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.08                     & 0.06                           & \textbf{25.0}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.10                     & 0.09                           & 10.0                                 \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & \textbf{16.67}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.05                     & 0.05                           & 0.0                                 \\ \hline
% \end{tabular}
% \label{tab:veh}
% \end{table}

% \begin{table}[]
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \begin{tabular}{|p{7mm}|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods                                                & MAE  & \%Improvement & MAE            & \% Improvement          \\ \hline
% \multicolumn{4}{|c|}{Vehicle Distance}                                                                                                      & \multicolumn{2}{c|}{Centerline Distance} \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &               & 0.09           &                         \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.05 &               & 0.09           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.06 & 16.67         & 0.09           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.05 & 0.0           & 0.08           & 11.11                   \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.04 & 20.0          & 0.07           & 22.22                   \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &               & 0.11           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.07 & -14.28        & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.08 & -25.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.06 & 0.0           & 0.11           & 0.0                     \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               & 0.11           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.10 & -10.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.10 & -10.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.05 & 44.44         & 0.12           & -8.3                    \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% %\captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods                                                & MAE  & \%Improvement \\ \hline
% \multicolumn{4}{|c|}{Vehicle Distance}                                                                                                      \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &               \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.05 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.06 & 16.67         \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.05 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.04 & 20.0          \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.07 & -14.28        \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.08 & -25.0         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.06 & 0.0           \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.10 & -10.0         \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.10 & -10.0         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.05 & 44.44         \\ \hline
% \multicolumn{4}{|c|}{Centerline Distance}                                                                                                   \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.09 &               \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.09 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.08 & 11.11         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.07 & 22.22         \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.11 & 0.0           \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.12 & -8.3          \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% %\captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \centering
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  & \% Improvement \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &                \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                                   & 0.05 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.06 & 16.67               \\ \cline{2-4} 
%                                                             & SLO  & 0.05 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.04 & \textbf{20.0}               \\ \hline
% \multirow{4}{*}{100:7}                                      &\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.07 & -14.28               \\ \cline{2-4} 
%                                                             & SLO  & 0.08 & -25.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.06 & 0.0               \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.10 & -10.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.10 & -10.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.05     & \textbf{44.44}               \\ \hline
% \end{tabular}
% \label{tab:vehaff}
% \end{table}

% \begin{table}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Centerline Distance} \tr{combine this with vehicle distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \centering
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  & \% Improvement \\ \hline
%                                                             & Whole Set    & 0.09 &                \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.09 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.08 & 11.11               \\ \cline{2-4} 
%                                                             & SLN  & 0.07 & \textbf{22.22}               \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.11 & 0.0               \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.12     & -8.3               \\ \hline
% \end{tabular}
% \label{tab:centaff}
% \end{table}
\begin{figure}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_left_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_left_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_straight_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_straight_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_right_15.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_right_plot_15.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{(a) Fraction of selected instances and (b) Mean Absolute Error (MAE) for Relative Angle affordance for all subset selection methods. Selection of more fraction of instances in turn buckets lead to lower MAE in CBML for 100:20 compression ratio.}}
    \label{fig:fracmae_100_20}
\end{figure}

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_left_100_7_15.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/mae_left_100_7_plot_15.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_straight_100_7_15.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/mae_straight_100_7_plot_15.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
    
    
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_right_100_7_15.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/mae_right_100_7_plot_15.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{(a) Fraction of selected instances and (b) Mean Absolute Error (MAE) for Relative Angle affordance for two baselines (MCL and SBML) and the proposed methods. Selection of more fraction of instances in turns lead to lower MAE in CBML for 100:7 compression ratio.}}
%     \label{fig:fracmae_100_7}
% \end{figure}
In this section, we will study the performance of different subset selection methods on the basis of their performance in affordance predictions.

We show in tables \ref{tab:redrhazaff}, \ref{tab:vehcen} the performance of Conditional Affordance Learning (CAL) \cite{sauer2018conditional} driving model for four affordances, on subsets obtained by different subset selection techniques for 100:20 compression ratio. 
% We report the best improvement of our proposed methods (STL,SML) for each affordance over the baselines (Uniform Skip (US), Only SIFT, Only Loss, PRL, SubM).
We notice in Table \ref{tab:redrhazaff} that all the methods are able to classify the affordances reasonably well. This is due to weighted cross-entropy losses used for the large number of imbalanced classes as seen initially in Figure \ref{fig:distrib}. From Table \ref{tab:vehcen}, we can see that CTL and CBML outpeform all other methods in predicting vehicle distance affordance. In case of centerline distance, all the methods work similarly with OS and OL performing the worst.

% We notice in table \ref{tab:redlaff} that the \textit{Red Light} accuracies are more for Uniform Skip than all other subset selection methods. Figure \ref{fig:distribhist} (\textit{left)} is a clear indication of the above statement, where we see that the distribution of Uniform Skip for Red Light is higher than all the other gradation methods. It is evident that Uniform Skip method, due to its inherent nature of selection, selects more number of \textit{Red Light True} instances. For example, if the agent vehicle is stuck in traffic, the Uniform Skip method will tend to choose frames uniformly leading to higher selection of true red light instances. However, in case of SLN, since the SIFT dissimilarity and multi-task loss values dominate the selection procedure, it selects the appropriate instances based on them. Since it tries to keep the compression ratio intact while trying to avoid repetitive instances, it tends to drop more frames with \textit{Red Light true} instances leading to a lower accuracy. However, this affordance is not directly related to the episode completion objective.

% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.28                                                                     & 0.02                                                                         & 0.10                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & Only SIFT                                                   & 0.23                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & Only Loss                                                   & 0.16                                                                     & 0.02                                                                         & 0.10                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & PRL                                            & 0.15                                                                     & 0.02                                                                         & 0.10                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLT                                            & 0.11                                                                     & 0.02                                                                         & 0.10                                                                      & 60.71                                                        & 33.33                                                            & 0.0
%                         \\ \cline{2-8} 
%                         & SLM                                            & 0.10                                                                     & 0.02                                                                         & 0.09                                                                      & 64.28                                                        & 33.33                                                            & 10.0
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.46                                                                     & 0.03                                                                         & 0.20                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.51                                                                     & 0.03                                                                         & 0.18                                                                      &                                                         &                                                             &                                                         \\ \cline{2-8} 
% %                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff}
% \end{table*}


% \begin{table}[]
% \centering
% \scriptsize

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.23                                                     & 0.03                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.16                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.15                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.11                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.10                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.10\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \centering
% \scriptsize
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.34                                                     & 0.03                                                     & 0.17                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.18                                                     & 0.02                                                     & 0.12                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{table}



% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     \centering
%     \includegraphics[height=3cm]{figures/preds_allmeth_100_20.png}
%     \caption{\textbf{Bucket-wise MAE of relative angle for 100:20 compression ratio}}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
% \end{figure}

% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Only SIFT\end{tabular} & 0.34                                                                     & 0.03                                                                         & 0.17                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & Only Loss                                                   & 0.18                                                                     & 0.02                                                                         & 0.12                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & PRL                                                   & 0.38                                                                     & 0.03                                                                         & 0.18                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & SLT                                            & 0.12                                                                     & 0.03                                                                         & 0.10                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLM                                            & 0.12                                                                     & 0.02                                                                         &    0.09                                                                   &                                                         &                                                             &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.46                                                                     & 0.03                                                                         & 0.20                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.51                                                                     & 0.03                                                                         & 0.18                                                                      &                                                         &                                                             &                                                         \\ \cline{2-8} 
% %                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff_100_7}
% \end{table*}
 
In case of \textit{Relative Angle} affordance, we have grouped the values into three different buckets meant for Left Turn, Straight Road, Right Turn. We observe in Figure \ref{fig:fracmae_100_20} that our proposed method achieves the lowest MAE for turns in comparison to other subset selection methods. We can also observe in Figure \ref{fig:fracmae_100_20}a that CBML selects more fraction of instances for both Left and Right turns while relaxes comparatively in the Straight Road buckets. SBML also has close fraction of instances to our method for left turn in Figure \ref{fig:fracmae_100_20}a, however it drops down in the fraction of right turns.
% This is a result of selection of instances using both the pairwise and weighted multi-task pointwise metric as we discussed in Section \ref{sec:subset}.

Figure \ref{fig:fracmae_100_20}b portrays the effective nature of our subset selection methods (CTL, CBML) over the other baselines in terms of Mean Absolute Error. We observe that the MAE for straight road buckets for all selection methods are very low in range. This is essentially due to the skewness in Relative Angle affordance. On the other hand, both CTL and CBML outperform all other methods in the turn buckets which have in usual, lesser number of datapoints. The difference in MAE becomes more evident with increase in compression ratio. It is indicative of the fact that our proposed method gives more importance to the frames which are non-redundant (during turns especially) and also having higher losses, thus leading to the lower MAE values in extreme buckets. Thus, we can clearly see that our proposed methods CTL and CBML are performing better quantitatively in terms of affordance predictions and qualitatively in terms of deployment of the trained model in simulator and measuring the episode completion rate.


% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{AISTATS2021PaperPack/figures/mae_bucket_100_20.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{AISTATS2021PaperPack/figures/mae_bucket_100_7.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE of relative angle for 100:20 and 100:7 compression ratio}}
%     \label{fig:maebuck}
% \end{figure}


% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/leftbucket_allmeth.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/straightbucket_allmeth.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/rightbucket_allmeth.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}








% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlysift_sim_fail.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlyloss_sim_fail.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prl_sim_fail.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Buckets in simulator episodes leading to failures for \textit{Only SIFT}(left), \textit{Only Loss}(middle) and \textit{PRL}(right) }}
%     \label{fig:deviate}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/sift_sml_stl_13_27.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlyloss_sml_stl_48_41.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prl_sml_stl_87_95.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Buckets in simulator episodes leading to failures for \textit{Only SIFT}(left), \textit{Only Loss}(middle) and \textit{PRL}(right) }}
%     \label{fig:deviate}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip5_US_SLN_SIFT_1.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip15_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip30_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE for relative angle}}
%     \label{fig:bucketmae}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_15p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:7 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turns_30p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_road_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:3 compression ratio}}
%     \label{fig:bucketprop30}
% \end{figure*}
% The same can be observed in table \ref{tab:relaff} where the Straight-Road MAE for all gradation methods have a narrow margin. This happens due to the more number of straight road instances than the turns in our dataset, as depicted in Figure \ref{fig:distrib} (\textit{Right}). However, SLN maintains an overall lower MAE across the buckets, thus proving its selection method efficient.
 
% We also show a similar plot for distribution of predicted affordances in Figure \ref{fig:distribhistpred} where we observe that the predictions also follow similar pattern as the distribution of ground truth affordances in Figure \ref{fig:distribhist}.


% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 96.26                                                    & 95.43                                                    \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 95.54                                                    & 94.82                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 91.9                                                     & 90.75                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 89.94                                                    & 87.79                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 90.52                                                    & 89.26                                                    \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 94.58                                                    & 95.02                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 90.1                                                     & 88.58                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 91.76                                                    & 91.4                                                     \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 91.32                                                    & 89.17                                                    \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 93.58                                                    & 92.60                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 91.87                                                    & 89.02                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 91.36                                                    & 90.78                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &                                                          &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Red Light affordance}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 0.15                                                    & 0.02                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.28                                                    & 0.03                                                        & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.16                                                    & 0.05                                                        & 0.14                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.17                                                    & 0.04                                                        & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.16                                                    & 0.05                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.27                                                    & 0.04                                                        & 0.09                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.17                                                    & 0.05                                                        & 0.16                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.21                                                    & 0.05                                                        & 0.11                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.19                                                    & 0.08                                                        & 0.06                                                     \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.32                                                    & 0.05                                                        & 0.09                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.28                                                    & 0.05                                                        & 0.14                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.23                                                    & 0.06                                                        & 0.11                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &                                                         &                                                             &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}
% \label{tab:relaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  \\ \hline
% \-\-                                                        & Whole Set    & 0.02 \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.04 \\ \cline{2-3} 
%                                                             & SIFT         & 0.04 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.04 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.05 \\ \cline{2-3} 
%                                                             & SIFT         & 0.07 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.06 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.07 \\ \cline{2-3} 
%                                                             & SIFT         & 0.09 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.09 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  &      \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Vehicle Distance affordance}
% \label{tab:vehaff}
% \end{table}




% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 95.86                                                    & 95.16                                                    \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 95.32 (-6.32)                                                   & 94.7 (-6.45)                                                   \\ \cline{2-4} 
%                                                             & SIFT         & 91.36 (-2.18)                                                    & 88.12 (0.13)                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 88.34 (0.84)                                                   & 86.96 (1.29)                                                   \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 89.18                                                   & 88.25                                                    \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 91.94 (-3.93)                                                   & 91.08 (-2.58)                                                   \\ \cline{2-4} 
%                                                             & SIFT         & 90.28 (-2.24)                                                    & 90.1 (-1.6)                                                   \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 89.7 (-1.66)                                                   & 89.8 (-1.3)                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &    88.04                                                 & 88.5                                                    \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 91.26                                                    & 90.36                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 90.04                                                    & 90.34                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 87.68                                                    & 88.54                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &                                                          &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Red Light affordance}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 0.15                                                    & 0.02                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.39 (0.21)                                                   & 0.03 (-0.02)                                                       & 0.09 (0.02)                                                    \\ \cline{2-5} 
%                                                             & SIFT         & 0.17 (-0.01)                                                   & 0.06 (-0.01)                                                       & 0.09 (0.01)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.19 (0.01)                                                   & 0.07                                                       & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.18                                                    & 0.05                                                        & 0.07                                                     \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.38 (0.18)                                                   & 0.04 (-0.03)                                                       & 0.11 (0.05)                                                    \\ \cline{2-5} 
%                                                             & SIFT         & 0.18 (-0.02)                                                   & 0.06 (-0.01)                                                       & 0.14 (0.08)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.19 (0.01)                                                   & 0.05 (-0.02)                                                       & 0.13 (0.07)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &    0.20                                                 & 0.07                                                        & 0.06                                                     \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.44                                                    & 0.06                                                        & 0.15                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.32                                                    & 0.06                                                        & 0.15                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.26                                                    & 0.05                                                        & 0.16                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &                                                         &                                                             &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}
% \label{tab:relaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  \\ \hline
% \-\-                                                        & Whole Set    & 0.02 \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.05 (0.01) \\ \cline{2-3} 
%                                                             & SIFT         & 0.06 (0.02) \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.05 (0.01) \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.06 (0.0) \\ \cline{2-3} 
%                                                             & SIFT         & 0.07 (0.01)\\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.08 (0.02) \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.06 \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.09 \\ \cline{2-3} 
%                                                             & SIFT         & 0.10 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.10 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  &      \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Vehicle Distance affordance}
% \label{tab:vehaff}
% \end{table}


% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 95.54                                                                         & 94.82                                                                         & 0.28                                                                         & 0.03                                                                             & 0.07                                                                          & 0.04                                  \\ \hline
% SIFT                                                   & 91.9                                                                          & 90.75                                                                         & 0.16                                                                         & 0.05                                                                             & 0.14                                                                          & 0.04                                      \\ \hline
% SIFT+Loss-O                                            & 89.94                                                                         & 87.79                                                                         & 0.17                                                                         & 0.04                                                                             & 0.08                                                                          & 0.04                                      \\ \hline
% SIFT+Loss-N                                            & 90.52                                                                         & 89.26                                                                         & 0.16                                                                         & 0.05                                                                             & 0.08                                                                          & 0.04                                      \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:20}
% \label{tab:grade_20}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.58                                                                         & 95.02                                                                         & 0.27                                                                         & 0.04                                                                             & 0.09                                                                          & 0.05                                  \\ \hline
% SIFT                                                   & 90.1                                                                          & 88.58                                                                         & 0.17                                                                         & 0.05                                                                             & 0.16                                                                          & 0.07                                      \\ \hline
% SIFT+Loss-O                                            & 91.76                                                                         & 91.4                                                                         & 0.21                                                                         & 0.05                                                                             & 0.11                                                                          & 0.06                                      \\ \hline
% SIFT+Loss-N                                            & 91.32                                                                         & 89.17                                                                         & 0.19                                                                         & 0.08                                                                             & 0.06                                                                          & 0.04                                      \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:7}
% \label{tab_grade_7}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 93.58                                                                         & 92.60                                                                         & 0.32                                                                         & 0.05                                                                             & 0.09                                                                          & 0.07                                   \\ \hline
% SIFT                                                   & 91.87                                                                          & 89.02                                                                         & 0.28                                                                         & 0.05                                                                             & 0.14                                                                          & 0.09                                      \\ \hline
% SIFT+Loss-O                                            & 91.36                                                                         & 90.78                                                                         & 0.23                                                                         & 0.07                                                                             & 0.11                                                                          & 0.09                                       \\ \hline
% SIFT+Loss-N                                            &                                                                          &                                                                          &                                                                          &                                                                              &                                                                           &                                       \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:3}
% \label{tab:grade_3}
% \end{table*}

% Considering the first type of observation for each compression ratio (or table), we notice that the Timestamp model shows an improved performance for each affordance in comparison. This is because the CAL model takes continuous frames into consideration, while in the Timestamp model, we have integrated the normalised timestamp difference between the subsequent frames. This leads to the better performance in Timestamp model, for all the data gradation methods where both uniformly and non-uniformly skipped frames are present.

% Following the second type of observation for each data gradation method under the same model (CAL or Timestamp), we notice that the \textit{Red Light} accuracies are more for Uniform Skip than all other subset selection methods. The reason becomes evident from Figure \ref{fig:distribhist} (\textit{top left)} where we see that the Uniform Skip method, due to its inherent nature of selection, selects more number of \textit{Red Light True} instances compared to the other methods. In case of \textit{Relative Angle} affordance, we have grouped the corresponding values into three different bins meant for Left Turn, Straight Road, Right Turn. We can observe from Figure \ref{fig:distribhist} (\textit{top right}) that SIFT+Loss-N (SLN) selects more number of instances belonging to the turn category. This is a result of selection of instances using the pointwise metric as we discussed in Section \ref{improved}. Even SIFT and SIFT+Loss-O perform close to SIFT+Loss-N in the selection method due to their selection mechanisms. The similar distribution in the values of Uniform Skip and Whole Set is trivial.

% We observe that even though the Uniform Skip method has similar distribution to that of WS, it is not what should ideally be for a decreased set of instances. This is because the reduced subset unless has enough instances of turns, the driving model would not be able to predict its next waypoint. SIFT and Sift+Loss-O have more instances of left turn instances than Uniform Skip. However, SIFT+Loss-N has a significantly higher number of instances for both the turns. Taking this into consideration, we observe from each table, that under each model (CAL or Timestamp), the gradation methods SIFT, SIFT+Loss-O and SIFT+Loss-N perform significantly better under turns than the Uniform Skip model.

% We show a bucketwise plot of relative angle for different compression ratios in Figure \ref{fig:bucketmae}, which portrays the effective nature of the gradation methods over Uniform Skip. The buckets corresponding to (-0.1 - 0.1) refer to the straight road instances, and the buckets to its left are meant for left turns while to its right, for right turns. We observe that the MAE for straight road buckets for all gradation methods are very low and close to one another. This happens due to the more number of straight road instances than the turns, as depicted in Figure \ref{fig:distrib} (\textit{Right}). Owing to the selection of large number of straight road instances in Uniform Skip selection, the MAE for straight road is lesser compared to the other selection methods. However, predicting its next waypoint on straight road is an easier task compared to turns, which we will observe in the next subsection.

% Lastly, with increasing degree of compression ratio, the performance of the gradation methods shifts away from that of the Whole Set, which is trivial. However, we observe that the difference between the performance of CAL and Timestamp model for each gradation method, becomes more vivid with increasing compression ratio. 



% We observe that the accuracies of the discrete affordance (Red Light) of the models trained using subsets are different by a comparatively wider margin, whereas that of the continuous affordances (Relative Angle and Centerline Distance) differ by a narrow margin. Uniform skip even though performs the best among all subsets in terms of red light affordance accuracy, it fails in selecting images necessary to be present during the turns.
% We show in Figure \ref{fig:distribhist} the distribution of two of the affordances (\textit{Red Light} and \textit{Relative Angle}) in all the selection methods for the compression ratio 100:20. We observe that distribution of both the affordances for Uniform Skip (US) is similar to that of the Whole Set (WS), which is trivial. However, the distribution differs for the other selection methods. In case of red light, SLN (Sift+Loss-N) selects comparatively more number of \textit{Red Light True} instances than the other two methods, namely SIFT and SLO (Sift + Loss-O), but lesser than that of US (Uniform Skip). This leads to the decrease in Red Light accuracy for the selection methods. The reason behind the decrease in selection of \textit{Red Light True} instances is that since the frames captured while in traffic are redundant, the selection methods try to skip the frames. \\
% The figure to the right showing the distribution of affordances for relative angle, we observe that even though the US method has similar distribution to that of WS, it is not what should ideally be for a decreased set of instances. This is because the reduced subset unless has enough instances of turns, the training model would not be able to predict its next waypoint. SIFT and SLO have more instances of left turn instances than US. However, SLN has a significantly higher number of instances for both the turns. The average MAE for SLN is slightly higher than that of US or SIFT. This is because the more number of test instances are concentrated towards the \textit{Straight} task, which has lesser number of selected frames due to redundancy. We show a bucketwise plot of relative angle which portrays the effective nature of SLN.
%\textcolor{red}{More explanation}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth,height=3.5cm]{figures/redlight.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:distribhist}
% \end{figure}



% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_pred5.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_pred5.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_pred15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_pred15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%      \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_30.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relative_30.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of predicted affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7 , (\textit{bottom}) 100:3 compression ratio: WS : Whole Set; US : Uniform Skip; SLO : SIFT+Loss-O; SLN : SIFT+Loss-N}}
%     \label{fig:distribhistpred}
% \end{figure}
% \begin{figure}[h!]
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redl.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:relhist}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turns.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:turnhist}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/haz.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:relhist}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/speed.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:turnhist}
%     \end{subfigure}
%     \captionsetup{justification=centering}
%     \caption{Comparison of distribution of affordances among the selection methods for 100:20 compression ratio: WS : Whole Set; US : Uniform Skip; SLO : SIFT+Loss-O; SLN : SIFT+Loss-N}
%     \label{fig:distribhist}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth,height=4cm]{figures/test_turns_skip5.png}
%     \caption{Bucket-wise MAE for relative angle}
%     \label{fig:turnskip5}
% \end{figure}









% \begin{table*}[]
% %\centering
% \begin{tabular}{|l|p{7mm}|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{3}{*}{Ratio}  & \multirow{3}{*}{Poses} & \multicolumn{8}{c|}{Tasks}                                                                                                                                                                                                                                                    \\ \cline{4-11} 
%                                                                           &                         &                        & \multicolumn{2}{l|}{Straight} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}One\\ Turn\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}One\\ Turn\\Dynamic\end{tabular}} \\ \cline{4-11} 
%                                                                           &                         &                        & CAL            & TS           & CAL                                 & TS                                & CAL                                     & TS                                    & CAL                                      & TS                                     \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}}      & \multirow{2}{*}{}       & Train                  & 10             &              & 9                                   &                                   & 10                                      &                                       & 8                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 7                                   &                                   & 10                                      &                                       & 7                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:20} & Train                  & 9              &              & 0                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 1                                   &                                   & 9                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  & 10             &              & 2                                   &                                   & 10                                      &                                       & 2                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 1                                   &                                   & 9                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  & 10             &              & 3                                    &                                   & 8                                       &                                       & 2                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 2                                    &                                   & 9                                       &                                       & 1                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  & 10             &              & 6                                   &                                   & 10                                      &                                       & 6                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 3                                   &                                   & 10                                      &                                       & 3                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:7} & Train                  & 9              &              & 0                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 0                                   &                                   & 7                                       &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  & 9             &              & 2                                   &                                   & 9                                      &                                       & 1                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 8             &              & 1                                   &                                   & 8                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  &              &              & 2                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  & 10             &              & 3                                   &                                   & 10                                      &                                       & 3                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 2                                   &                                   & 10                                      &                                       & 2                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:3} & Train                  & 9              &              & 1                                   &                                   & 8                                       &                                       & 0                                       &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 1                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  &              &              & 1                                   &                                   &                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                   &                                   &                                        &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  &              &              & 1                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                    &                                   &                                        &                                       & 0                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  &              &              &                                    &                                   &                                       &                                       &                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              &                                    &                                   &                                       &                                       &                                         &                                        \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques in terms of episode completion \tr{Will reorder the structure}}
% \label{eptable}
% \end{table*}




% \subsection{CAL vs Timestamp model}
% \label{tsvscal}

% Having motivated the Timestamp model in Section \ref{sec:CAL-TS}, we show here the effectiveness of Timestamp model in the light of prediction of the following affordances - \textit{Red Light} ,\textit{Vehicle Distance} and \textit{Relative Angle}. We compare in tables \ref{tab:redl},  \ref{tab:veh} and \ref{tab:relative}, CAL and Timestamp Model for the three methods - Uniform Skip, SLO and SLN across 3 compression ratios - \textit{100:20}, \textit{100:7} and \textit{100:3}. We report the micro and macro accuracies for Red Light, direction based bucket-MAE of relative angle , MAE of vehicle distance and \% improvement of Timestamp model over CAL model for every affordance.

% It is observed that Timestamp model shows an improved performance in affordance predictions for all the methods for each affordance in comparison. This is because the CAL model takes continuous frames into consideration in the frame buffer, while the Timestamp model integrates the normalised timestamp difference between the subsequent frames. This leads to the better performance in Timestamp model for the data gradation methods, where both uniformly and non-uniformly skipped frames are present. We have boldfaced the highest improvement for each gradation method under each metric of affordance.

% Besides, we observe in table \ref{tab:relative} that Uniform skip which is an uniformly-skipping-frames method, has a higher MAE for Left turn under CAL model. The reason lies in the number of left turns present in our dataset, shown in Figure \ref{fig:distrib} (\textit{Right}). Owing to its inherent nature, Uniform skip tends to skip frames uniformly, as a result of which it ends up missing a large number of frames belonging to left turn. However, using Timestamp model, the respective Left Turn MAE for Uniform skip is lower due to the inclusion of timestamp information. Hence, we are able to show that inclusion of timestamp information in the perception module of driving model yields a better performance, in the process of making self-driving data efficient.


% \begin{table}[]
% \caption{\textbf{Comparison of CAL and Timestamp Model on Centerline Distance affordance}}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.09                     & 0.07                           & \textbf{22.22}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.10                           & 9.09                                \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.09                     & 0.08                           & \textbf{11.11}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-N}                                            & 100:20                                                                                            & 0.07                     & 0.06                           & \textbf{14.28}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.11                            & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.12                     & 0.12                           & 0.0                                 \\ \hline
% \end{tabular}
% \label{tab:cenaff}
% \end{table}

% \begin{table*}[]
% \centering
% \begin{tabular}{|c|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.63                                                                         & 94.98                                                                          & 96.22                                                                         & 95.41                                                                         & 0.59                                                                           & 0.43                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 93.53                                                                         & 93.53                                                                         & 95.58                                                                         & 95.15                                                                         &  2.05                                                                         & 1.62                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 92.64                                                                         & 92.15                                                                         & 95.29                                                                         & 94.92                                                                         & 2.65                                                                          & 2.77                                                                          \\ \hline
% \multirow{3}{*}{SIFT + Loss-O}                                          & 100:20                                                                                            & 96.83                                                                         & 86.43                                                                         & 97.99                                                                         & 93.25                                                                         & 1.16                                                                           & 6.82                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 96.74                                                                          & 90.17                                                                          & 97.01                                                                         & 92.32                                                                          & 0.27                                                                          & 2.15                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 90.53                                                                         & 89.97                                                                         & 97.63                                                                         & 91.69                                                                         & 7.1                                                                          & 1.72                                                                         \\ \hline

% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance using varying spaced frame buffers}}
% \label{tab:redl_data}
% \end{table*}


% \begin{table*}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{3}{c|}{CAL}                                                                                                                                                         & \multicolumn{3}{c|}{Timestamp}                                                                                                                                                   & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{3-11} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.29                                                    & 0.02                                                        & 0.09                                                     & 0.20                                                    & 0.02                                                        & 0.06                                                     & 31.0                                                    & 0.0                                                         & 33.33                                                     \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.36                                                    & 0.03                                                        & 0.15                                                     & 0.37                                                    & 0.03                                                        & 0.11                                                     & -2.7                                                    & 0.0                                                         & 26.67                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.44                                                    & 0.03                                                        & 0.13                                                     & 0.38                                                    & 0.03                                                        & 0.10                                                    & 13.63                                                    & 0.0                                                         & 23.08                                                      \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.20                                                    & 0.07                                                        & 0.11                                                     & 0.12                                                    & 0.04                                                        & 0.13                                                     & 40.0                                                     & 42.85                                                         & -18.18                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.24                                                    & 0.05                                                        & 0.21                                                     & 0.20                                                    & 0.04                                                        & 0.15                                                     & 16.67                                                    &    20.0                                                      & 28.57                                                     \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.17                                                     & 0.27                                                    & 0.04                                                        & 0.15                                                     & -3.8                                                     & 20.0                                                        & 11.76                                                      \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Relative Angle affordance using varying spaced frame buffers}}
% \label{tab:relative_data}
% \end{table*}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   &  0.07                    & 0.05                           & 28.57                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                  & 0.03                     & 0.02                           & 33.33                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.07                     & 0.04                           & 42.85                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & 22.22                                 \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance using varying spaced frame buffers}}
% \label{tab:veh_data}
% \end{table}

% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.08                     & 0.08                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.07                     & 0.07                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.12                         & 0.11                               & 8.33                                    \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.15                     & 0.09                           & 40.0                                \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.15                     & 0.13                           & 13.33                               \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.17                     & 0.16                           & 5.88                                \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Centerline Distance affordance using varying spaced frame buffers}}
% \label{tab:cen_data}
% \end{table}



% \begin{table*}[h!]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 95.32                                               & 94.7                                                & 95.54                                               & 94.82                                               & 0.22                                                    & 0.12                                                    & 0.39                                                      & 0.03                                                          & 0.09                                                       & 0.28                                                      & 0.03                                                          & 0.07                                                       & 11.0                                                    & 0.0         & 2.0                                                      & 0.05 & 0.04                     & 1.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 88.34                                               & 86.96                                               & 89.94                                               & 87.79                                               & 1.6                                                    & 0.83                                                    & 0.19                                                      & 0.07                                                          & 0.08                                                       & 0.17                                                      & 0.04                                                          & 0.08                                                       & 2.0                                                    & 3.0         & 0.0                                                      & 0.05 & 0.04                     & 1.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp (TS) Model for compression ratio 100:20}
% \label{CALvsTS_100_20}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 91.94                                               & 91.08                                                & 94.58                                               & 95.02                                               & 3.08                                                    & 3.94                                                    & 0.38                                                      & 0.04                                                          & 0.11                                                       & 0.27                                                      & 0.04                                                          & 0.09                                                       & 11.0                                                    & 0.0         & 2.0                                                      & 0.06 & 0.05                     & 1.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 89.7                                               & 89.8                                               & 91.76                                               & 91.4                                               & 2.06                                                    & 1.6                                                    & 0.19                                                      & 0.05                                                          & 0.13                                                       & 0.21                                                      & 0.05                                                          & 0.11                                                       & -2.0                                                    & 0.0         & 2.0                                                      & 0.08 & 0.06                     & 2.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp (TS) Model for compression ratio 100:7}
% \label{CALvsTS_100_7}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 91.26                                               & 90.36                                                & 93.58                                               & 92.60                                               & 2.32                                                    & 2.24                                                    & 0.44                                                      & 0.06                                                          & 0.15                                                       & 0.32                                                      & 0.05                                                          & 0.09                                                       & 12.0                                                    & 1.0         & 6.0                                                      & 0.09 & 0.07                     & 2.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 87.68                                               & 88.54                                               & 91.36                                               & 90.78                                               & 3.68                                                    & 2.24                                                    & 0.26                                                      & 0.05                                                          & 0.16                                                       & 0.23                                                      & 0.07                                                          & 0.11                                                       & 3.0                                                    & -2.0         & 5.0                                                      & 0.10 & 0.09                     & 1.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp(TS) Model for compression ratio 100:3}
% \label{CALvsTS_100_3}
% \end{table*}





==> experiment3.tex <==
% \tr{
% - Comparison of approximate online subset selection methods:\\
% -- synthetic data: our method, PRL 2020, sub-modular. Can we compare against other methods?\\
% -- Video data: our method, PRL 2020, sub-modular.\\
% -- Sequential application \\
% -- comparison of PRL with variation in $\rho$
% - Data efficient autonomous driving:\\
% -- 
% }


In this section, we provide our experimental setup by describing the dataset and the subset selection methods. We then show a comparison of approximate online subset selection methods over synthetic data and our collected driving data from the CARLA simulator \cite{dosovitskiy2017carla}. Next, we compare the performances of various subset selection methods in the autonomous driving application from two aspects: episode completion and affordance prediction.

\subsection{Experimental Setup}

\textbf{Dataset}: We use the open-source driving simulator CARLA\cite{dosovitskiy2017carla} for generating our driving dataset. CARLA simulates an urban driving scenario where there are several other non-player agents like other vehicles, pedestrians, traffic lights and speed signs aiding the player agent vehicle.
In order to collect the training data, the agent vehicle was navigated using the Conditional Affordance Learning controller \cite{sauer2018conditional} based on the ground truth affordances like red light, hazard stop etc. which have been described later in this section. The affordances have been determined and categorised following \cite{sauer2018conditional}. We generated the driving data comprising of 262 episodes and a total of approximately 100,000 frames. We performed the experiments on our generated dataset and compared the subsets obtained using different selection methods.

% where the agent vehicle is driven by the game AI.
For each episode run, we collect: (1) images from camera attached to the agent vehicle, and (2) the corresponding six affordances (Discrete: Red Light, Hazard Stop, Speed Sign ; Continuous: Relative Angle, Centerline Distance, Vehicle Distance) \cite{sauer2018conditional}. Affordances are signals useful for navigation in the environment. We used approximately $85\%$ of the collected dataset as the training set, and the remaining as the test set.
 
 We ensured the similar distribution of affordances in both the training and test set. Figure \ref{fig:distrib} illustrates the distribution of four affordances per class label, in training and test set. Red light and Hazard Stop have two classes - \textit{True}, \textit{False}, Speed sign has four classes - \textit{None} , \textit{30kmph}, \textit{60kmph}, \textit{90kmph}, while in case of Relative angle which is the orientation angle of the agent vehicle, we have grouped the values into buckets corresponding to \textit{Left turn}, \textit{Straight} and \textit{Right turn}. We can divide the entire range of Relative Angle affordance across 20 buckets ranging from -1.0 to +1.0. Note that buckets corresponding to (-1.0 to -0.1), (-0.1 to 0.1) and (0.1 to 1.0) approximately indicate the left turn, straight road and right turn respectively.
 
 \begin{figure}[h!]
    %\centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_red.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:red}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_rel.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:relang}
    \caption{}
    \end{subfigure}
    % \captionsetup{justification=centering}
    % \caption{\textbf{Distribution of affordances: (\textit{Left}) : Red Light and (\textit{Right}) : Relative Angle in training and test set}}
    % \label{fig:distrib}
    
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_speed.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:spd}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/distrib_haz.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:haz}
    \caption{}
    \end{subfigure}
    %\captionsetup{justification=centering}
    \caption{\textbf{Distribution of affordances: (a) : Red Light (b) : Relative Angle (c) : Speed Sign (d) : Hazard Stop in training and test set}} 
    \label{fig:distrib}
    % \begin{subfigure}{0.48\columnwidth}
    % \centering
    % \includegraphics[width=\textwidth,height=2.5cm]{figures/speedsign.eps}
    % %\caption{Red light Affordance Distribution}
    % \label{fig:turn}
    % \end{subfigure}
    
    
\end{figure}

%\subsubsection{Subset selection on Autonomous Driving}
\textbf{Subset selection on Autonomous Driving:}
We use Conditional Affordance Learning \cite{sauer2018conditional} (CAL) model as the driving model to be trained on the dataset we collected using the CARLA \cite{dosovitskiy2017carla} simulator. We train the driving model on NVIDIA Tesla P100 for 50 epochs using Adam Optimizer with learning rate varying between $10^{-3}$ to $10^{-4}$.

We report results with the following methods of selection for two compression ratios 100:20 and 100:7:

\textbf{Whole Set (WS)}: This comprises of the dataset with no reduction.

\textbf{Uniform Skip (US)}: The data is sampled uniformly from the whole dataset, based on the compression ratio.

\textbf{Only SIFT (OS)}: Following Equation \ref{eqn:eq1}, this subset is obtained by selecting images based only on SIFT dissimilarity.

\textbf{Only Loss (OL)}: This subset is obtained by selecting images with highest losses.

\textbf{Multi-Criteria Loss (MCL)}\cite{das2020multi} : The subset is formed by using the multiple-criteria-based subset selection method (Equation \ref{eqn:oldsiftloss}), based on the compression ratio. We used the pairwise criteria (SIFT dissimilarity) and pointwise criteria (loss) as the components of this method.

\textbf{Submodular Bucketwise Multi-task Loss (SBML)}\cite{buchbinder2014submodular} : The subset is obtained by adapting the submodular approach proposed in \cite{buchbinder2014submodular}, in our framework with pairwise (SIFT dissimilarity) and pointwise metric (bucket-wise Relative Angle affordance aided with other multi task losses). 

\textbf{Convex Total Loss (CTL)}: This subset is obtained by adopting our proposed subset selection method (Equation \ref{eqn:newsiftloss}) using SIFT and total loss, based on the compression ratio.

\textbf{Convex Bucketwise Multi-task Loss (CBML)}: This subset is formed by adopting our proposed subset selection method (Equation \ref{eqn:newsiftloss}) using SIFT and bucket-wise Relative Angle affordance aided with other multi task losses, based on the compression ratio.

% \begin{table*}[]
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion}}
% \label{tab:epsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{c|}{Straight}                                                                                                                                               & \multicolumn{3}{c|}{One-Turn}                                                                                                                                             & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set episode completion count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{10}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{10}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SLO/\\ SLN\end{tabular} & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   & \begin{tabular}[c]{@{}l@{}}SIFT/\\ SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   \\ \hline
% 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   \\ \hline
% 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 1                                                       & 88.88                                                   & SLN                                                   & 10                                                      & 0                                                       & SLO                                                   & 1                                                       & 88.88                                                   \\ \hline
% %                                                                              & \multicolumn{12}{c|}{Whole Set test poses completion count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
% %                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{7}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    \\ \hline
% % 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}      & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% % 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 2                                                       & 71.42                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% % 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \scriptsize
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for relative angle affordance prediction}}
% \label{tab:relsumm}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{9}{c|}{Relative Angle buckets}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \cline{2-10} 
%                                                                              & \multicolumn{3}{c|}{Left-Turn}                                                                                                                                                & \multicolumn{3}{c|}{Straight-Road}                                                                                                                                             & \multicolumn{3}{c|}{Right-Turn}                                                                                                                                               \\ \cline{2-10} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Difference\\ in MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & SIFT                                                  & 0.02                                                        & 11.76                                                   & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.01                                                        & 33.33                                                   & SLN                                                  & 0.01                                                        & 12.5                                                   \\ \hline
% 100:7                                                                        & SIFT                                                  & 0.03                                                        & 16.67                                                   & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.01                                                        & 50.0                                                    & SLN                                                  & 0.01                                                        & 25.0                                                   \\ \hline
% 100:3                                                                        & SLN                                                   & 0.06                                                        & 28.57                                                   & SLO                                                    & 0.02                                                        & 60.0                                                    & SLN                                                   & 0.02                                                        & 25.0                                                    \\ \hline
% \end{tabular}
% \end{table*}
% We use Conditional Affordance Learning model \cite{sauer2018conditional} (CAL) as the driving model to be trained on the dataset we collected using the CARLA \cite{dosovitskiy2017carla} simulator. We train the driving model on NVIDIA Tesla P100 for 50 epochs using Adam Optimizer with learning rate varying between $10^{-3}$ to $10^{-4}$.

 
 \textbf{Subset selection and Training Times}:
%  \tr{write in 2 - 3 sentences how our methods are saving time as well as storage space refering to table \ref{tab:time}}
Table \ref{tab:time} shows the amount of total time taken for training and subset selection for each compression ratio. Compression ratio of 100:20 takes about 1/3rd the total time taken to train the whole set (WS). In terms of storage space, the whole set acquires about 14.5GB of data, which after compression reduces to 2.9GB for compression ratio of 100:20. This follows for the other compression ratio too and hence saves both time and space, essential in the current IoT setting with massively huge data.

 
%  \begin{table}[h]
% \captionsetup{justification=centering}
% \caption{\textbf{Time complexity of proposed methods}}
% \footnotesize
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Compression ratio    & WS  & 100:20 & 100:7 & 100:3 \\ \hline
% Training Time (hours)  & 30 & 8   & 3 & 1.5   \\ \hline
% Subset selection Time (hours) & 0  & 2   & 1.5 & 1   \\ \hline
% Total Time     & 30 & 10   & 4.5 & 2.5   \\ \hline
% \end{tabular}
% \label{tab:time}
% \end{table}

% \begin{table}[h]
% \captionsetup{justification=centering}
% \caption{\textbf{Time complexity of proposed method}}
% \footnotesize
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% Compression ratio    & WS  & 100:20 & 100:7\\ \hline
% Training Time (hours)  & 42 & 11   & 7\\ \hline
% Subset selection Time (hours) & 0  & 3   & 1.5\\  \hline
% Total Time     & 42 & 14   & 8.5\\ \hline
% \end{tabular}
% \label{tab:time}
% \end{table}

\begin{table}[]
\caption{\textbf{Time complexity of selection methods}}
\footnotesize
\begin{tabular}{|l|l|l|l|l|}
\hline
\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}                         & WS                 & \multirow{2}{*}{}                                         & 100:20 & 100:7 \\ \cline{1-2} \cline{4-5} 
\begin{tabular}[c]{@{}l@{}}Training Time\\ (hours)\end{tabular}                     & 42                 &                                                           & 11     & 7     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Subset Selection\\ (hours)\end{tabular}} & \multirow{3}{*}{0} & MCL                                                       & 2      & 1     \\ \cline{3-5} 
                                                                                    &                    & SBML                                                      & 5      & 2.5   \\ \cline{3-5} 
                                                                                    &                    & \begin{tabular}[c]{@{}l@{}}Proposed\\ Method\end{tabular} & 1.5    & 0.75  \\ \hline
\end{tabular}
\label{tab:time}
\end{table}


% \begin{table}[h!]
% \captionsetup{justification=centering}
% \caption{\textbf{Prediction accuracy of speed sign on test set using CAL model trained on whole dataset}}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Affordance & None  & 30kmph & 60kmph & 90kmph\\ \hline
% Speed Sign & 98.99 & 0.0   & 100.0 & 0.0\\ \hline
% \end{tabular}
% \label{speedacc}
% \end{table}

% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions}}
% \label{tab:ep}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 3                                                          & 8        & 2                                                          & 9        & 3                                                          & 9        & 3                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &        &                                                           &         &                                                           &        &                                                           &         &                                                           \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{9}                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{8}                                                          \\ \hline
% \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 2                                                          & 8        & 2                                                          & 9        & 3                                                          & 7        & 3                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 9        & 4                                                          & 9        & 4                                                          & 8        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         &                                                           \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{6}                                                          & 10       & \textbf{6}                                                          & 10       & \textbf{8}                                                          & 10       & \textbf{8}                                                          \\ \hline
% \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 1                                                          & 8        & 0                                                          & 9        & 2                                                          & 8        & 2                                                          \\ \cline{2-10} 
%                                                                              & SIFT                                                   & 8        & 0                                                          & 8        & 0                                                          & 8        & 1                                                          & 9        & 0                                                          \\ \cline{2-10} 
%                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         & 0                                                          \\ \cline{2-10} 
%                                                                              & SLN                                                    & 10       & \textbf{5}                                                          & 10       & \textbf{5}                                                          & 10       & \textbf{6}                                                          & 9       & \textbf{6}                                                          \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.28                                                                     & 0.02                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.23                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLN                                            & 0.10                                                                     & 0.01                                                                         & 0.04                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.07                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLO                                            &                                                                      &                                                                          &                                                                       &                                                         &                                                             &                                                         \\ \cline{2-8} 
%                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff}
% \end{table*}

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 97.39                                                                     & 97.41                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 96.72                                                                     &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 96.11                                                                     & 96.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 93.49                                                                     & 91.96                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 92.63                                                                     & 91.94                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 89.55                                                                     & 87.23                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                       &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 97.12                                                                     & 97.04                                                                      &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.06                                                                     & 93.09                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 94.16                                                                     & 93.54                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 94.42                                                                      & 93.72                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 99.44                                                                     & 99.72                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.14                                                                     & 99.47                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.11                                                                     & 99.56                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.33                                                                     & 99.66                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.42                                                                     & 97.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.31                                                                     & 98.99                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                       &                                                                       &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.45                                                                     & 98.76                                                                      &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 98.57                                                                     & 97.67                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SIFT                                                   & 99.29                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLO                                            &                                                                      &                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & SLN                                            & 99.12                                                                      & 98.23                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:hazaff}
% \end{table}
% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|p{12mm}|p{8mm}|l|p{15.5mm}|l|p{15.5mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & MAE           & \%Improvement         & MAE            & \%Improvement           \\ \cline{3-6} 
%                                                                              &                                                        & \multicolumn{2}{l|}{Vehicle Distance} & \multicolumn{2}{l|}{Centerline Distance} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.03          &                       & 0.05           &                         \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.05           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                    &            &                    \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.04          &                   & 0.06           &                    \\ \hline
% \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.06           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.09          &                 & 0.08           &                      \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                  &            &                      \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.07          &                   & 0.06           &                     \\ \hline
% \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.07          &                       & 0.09           &                         \\ \cline{2-6} 
%                                                                              & SIFT                                                   & 0.11          &                  & 0.08           &                     \\ \cline{2-6} 
%                                                                              & SLO                                                    &           &                  &            &                      \\ \cline{2-6} 
%                                                                              & SLN                                                    & 0.06          &                  & 0.06           &                     \\ \hline
% \end{tabular}
% \end{table}

\textbf{Metrics reported}: We have reported metrics for the two subtasks: episode completion and affordance accuracies. An episode corresponds to a source-destination pair which is provided to the agent vehicle prior to running the simulator. The episode completion is measured in terms of the number of successfully completed episodes. The accuracies of discrete affordances are measured in terms of the standard metrics - Micro and Macro Accuracy, while the continuous affordances are measured in terms of Mean Absolute Error (MAE). 

\textbf{Affordance Selection}: We have reported results for five affordances - \textit{Red light}, \textit{Hazard Stop}, \textit{Relative Angle}, \textit{Centerline Distance} and \textit{Vehicle Distance}. Considering the setup of our dataset collection, from Figure \ref{fig:distrib}, we can observe that the two affordances \textit{Speed Sign} and \textit{Hazard Stop} suffer from class imbalance.

In case of Speed Sign, only 1.5\% of the entire data belongs to other classes of speed signs (0.7\% 30kmph, 0.4\% 60kmph and 0.3\% 90kmph), and are hence predicted incorrectly by the driving model trained on the whole dataset. The predicted accuracies of each class from the test set are as follows: 98.99\% for \textit{None}, 0.0\% for \textit{30kmph}, 100.0\% for \textit{60kmph} and 0.0\% for \textit{90kmph}. Owing to this reason, we refrain from reporting accuracies on this affordance. Alongside, prediction accuracy of this affordance does not have an impact on episode completion.


% Table \ref{speedacc} shows the predicted accuracies of each class from the test set which comprises of 0.4\% 30kmph , 0.2\% 60kmph, 0.04\% as 90kmph and the remaining as \textit{None}. 

\textbf{Multi-task criteria}: Autonomous vehicles need a high level of understanding of the environment it needs to interact with. There are multiple criteria/tasks to be considered while reaching a destination or in other words, completing an episode. Conditional Affordance Learning \cite{sauer2018conditional} has considered six of such tasks or affordances in its driving model. The affordance \textit{Relative Angle} is the orientation of the car with respect to the road and decides the steer value of the agent vehicle. Hence, this affordance becomes critical in episode completion. However, we notice a large skew in the distribution of affordances in Figure \ref{fig:distrib}b which essentially portrays the importance of selection of instances from the minority buckets (turn buckets) for the end-task of driving. There is also no established end-to-end connection between the selection of affordances and a successful episode. Therefore, this comes out as a challenge in selecting affordances for a chosen subset which will be significant in episode completion.

\subsection{Comparison of approximate online subset selection methods}

\vspace{-2.7mm}
\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=2.5cm]{figures/conv_prl_subm_syn_rename_again.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:synbox}
    \caption{}
    \end{subfigure}
    \begin{subfigure}{0.45\columnwidth}
     \centering
     \includegraphics[width=\textwidth,height=2.5cm]{figures/conv_prl_subm_real_rename.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:realbox}
    \caption{}
     \end{subfigure}
     \caption{\textbf{Objective function values for proposed method , \cite{das2020multi} method and Submodular method for (a) Synthetic data (b) CARLA driving data samples}}
     \label{fig:convsub}
 \end{figure}  
% We compare the performance of the online subset selection methods empirically in terms of their objective function values. 
% We show in Figure \ref{fig:convsub} the objective function values for the proposed method, \citep{das2020multi} method and the submodular approach \citep{buchbinder2014submodular}. For the synthesized data, we generated 10 random samples of dimension $100 \times 100$. Since the submodular approach is a randomized algorithm, we made 100 runs for each sample and show a box plot of the submodular method's objective function values. 

In this section, we compare the optimal subsets reported by the baseline method \cite{das2020multi}, submodular method and the proposed convex optimization based method in terms of final objective function values. 
Figure \ref{fig:convsub}a shows the objective function values for the three approaches, for 10 randomly synthesized problem instances ($d$ matrix of dimension $100\times 100$ and $L$ vector of dimension $100$ in equations \ref{eq:joint}, \ref{eq:submod} , \ref{eqn:newsiftloss}). For the submodular method, we report a box plot of results over 100 runs of the algorithm to capture the randomness. While all three methods find approximate solutions, the proposed convex method consistently finds lower values of objective function, followed by \cite{das2020multi}, and submodular optimization. For real data (CARLA data for our further experiments), we report the same in Figure \ref{fig:convsub}b , for 10 episodes in our collected data. We can clearly observe that function values attained by our proposed method lies below that of the other approximate methods, thus proving our method to be an efficient approach. 

We show in Table \ref{tab:inctime} the impact of online selection on the objective function values. We observe the change in objective function values across increasing time-steps. The values show a gradual decline with increasing time-steps which affirms the efficiency of the online paradigm.

% We show in Figure \ref{fig:rhoPRL} the change in objective function values with variation in $\rho$. We can observe that the pointwise metric has a very. When the pointwise metric is given the entire weightage ($\rho = 0 $), only 1 representative gets selected from the existing or incoming set, whichever yields the highest value, irrespective of the compression ratio. The consistent difference in objective function values between \citep{das2020multi} and the proposed method mark the efficiency of the proposed method and also brings out empirically one of the drawbacks of \citep{das2020multi}.


% We can observe that the gap in objective function values between \citep{das2020multi} and the proposed method decreases with increase in $\rho$ which marks higher weightage on pairwise metric. However, . Thus, this brings out empirically one of the drawbacks of \citep{das2020multi} explained in Section \ref{sec:subset}.

% We also reported in Table \ref{tab:measure} the mean \% difference between the objective function values of convex and submodular approach, and the mean time taken to optimise the synthesized data samples.

\begin{table}[]
\footnotesize
\caption{\textbf{Objective function values for proposed method on CARLA driving data with increasing time sequence}}
\label{tab:inctime}
\begin{tabular}{|l|l|l|l|l|}
\hline
Time Sequence                                                       & t = 1 & t = 2 & t = 3 & t = 4 \\ \hline
\begin{tabular}[c]{@{}l@{}}Objective function\\ values\end{tabular} & 0.127 & 0.11  & 0.106 & 0.105 \\ \hline
\end{tabular}
\end{table}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.45\columnwidth,height=2.5cm]{figures/seq_time.pdf}
%      \caption{\textbf{Objective function values for proposed method on CARLA driving data with increasing time sequence}}
%      \label{fig:inctime}
%  \end{figure}


% \vspace{-2.7mm}
% \begin{figure}[h!]
%     \centering
%     %\caption{\textbf{Objective function values for proposed function , PRL function and submodular function for (a) Synthetic data (b) CARLA driving data samples}}
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/seq_time.pdf}
%     % \caption{\textbf{Objective function values for our proposed function on incoming set of CARLA driving data in sequence of time}}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:inctime}
%     %\caption{}
%     \end{subfigure}
%     \hspace{1mm}
%     \begin{subfigure}{0.45\columnwidth}
%      \centering
%      \includegraphics[width=\textwidth,height=2.5cm]{figures/rho_var_MCL.pdf}
%     %  \caption{\textbf{Objective function values for our proposed function and PRL function on Synthetic data sample with variation of $\rho$}}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:rhoPRL}
%     %\caption{}
%      \end{subfigure}
%      \caption{(a)\textbf{Objective function values for proposed method on CARLA driving data in sequence of time} (b) \textbf{Objective function values for proposed method and \citep{das2020multi} on synthetic data sample with variation of $\rho$.}}
%      \label{fig:incrho}
%  \end{figure}

% \begin{figure}[h!]
%     \centering
%     \caption{\textbf{Objective function values for our proposed function on incoming set of CARLA driving data in sequence of time}}
%     \includegraphics[width=0.5\columnwidth,height=2.5cm]{figures/seq_time.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:inctime}
% \end{figure}

Next, we discuss the application of the subset selection methods on autonomous driving.

% \begin{figure}[h!]
%     \centering
%     \caption{\textbf{Objective function values for our proposed function and PRL function on Synthetic data sample with variation of $\rho$}}
%     \includegraphics[width=0.5\columnwidth,height=2.5cm]{figures/rho_var_PRL.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:rhoPRL}
% \end{figure}




% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/relturns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{left}) 100:20 , (\textit{middle}) 100:7, (\textit{right}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure*}

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
    
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_20.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_20.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redllight_15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turn_15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_3.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_3.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7, (\textit{bottom}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure}

% In case of Hazard Stop, only 0.5 \% of data has presence of hazard stops, while test set has none. Overall, all the methods are able to predict the majority class (i.e no hazard stop) leading to an accuracy close to 100\%. In order to avoid the trivial case, we exclude this affordance from our results.



% \tr{Speed sign: Only about 1\% (0.5\% 30kmph, 0.1\% 60kmph and 0.3\% 90kmph) of the data belongs to other speed signs which are all predicted wrongly by the CAL model even with full dataset. Prediction accuracy of this affordance also does not affect episode completion. (give classwise accuracy and number of data points.) \\
% Hazard stop: The data has extreme skew only 0.6\% of the training data has hazard stop as true and there are no test instances with this.\\}
% \subsection{Comparison of data gradation methods with Whole Set}

% In this section, we provide a summary of results enlisting the best method from the two sets of experiments that we perform while comparing selection methods with whole set - episode completion and affordance prediction. 

% We consider four tasks under episode completion which had been originally defined in \cite{dosovitskiy2017carla}:
% \begin{enumerate}
%     \item Straight : The episode comprises of points which is a straight road.
%     \item One-Turn : The episode comprises of points which include a left or right turn in its path.
%     \item Straight Dynamic : It is similar to Straight task in the presence of other vehicles and pedestrians.
%     \item One-Turn Dynamic : It is similar to One-Turn task in the presence of other vehicles and pedestrians.
% \end{enumerate}

% In table \ref{tab:epsumm}, we show the best performing method for each task under episode completion along with the number of successfully completed episodes and its difference with that of the whole set. We can observe that the method SLN completes the most number of episodes (out of a total of 10 episodes) among all other gradation methods. It fails for only 33\% episodes in the difficult task of taking turns. The detailed results on episode completion is explained in the next subsection.




% \begin{table*}[]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in training conditions}}
% \label{tab:trainepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{l|}{Straight}                                                                                                                                               & \multicolumn{3}{l|}{One-Turn}                                                                                                                                             & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set Episode Completion Count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                     & \multicolumn{3}{l|}{9}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{9}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SLO/\\ SLN\end{tabular} & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   & \begin{tabular}[c]{@{}l@{}}SIFT/\\ SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 6                                                       & 33.33                                                   \\ \hline
% 100:7                                                                        & SLN                                                     & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 66.66                                                   \\ \hline
% 100:3                                                                        & SLN                                                     & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 1                                                       & 88.88                                                   & SLN                                                   & 10                                                      & 0                                                       & SLO                                                   & 1                                                       & 88.88                                                   \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in testing conditions}\tr{Combine this with the training table}}
% \label{tab:testepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{3}{l|}{Straight}                                                                                                                                             & \multicolumn{3}{l|}{One-Turn}                                                                                                                                             & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}}                                                                                           & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular}}                                                                                           \\ \cline{2-13} 
%                                                                              & \multicolumn{12}{c|}{Whole Set Episode Completion Count}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \cline{2-13} 
%                                                                              & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    & \multicolumn{3}{l|}{10}                                                                                                                                                   & \multicolumn{3}{l|}{7}                                                                                                                                                    \\ \cline{2-13} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} & \begin{tabular}[c]{@{}l@{}}Best\\ Method\end{tabular} & \begin{tabular}[c]{@{}l@{}}Episode\\ Count\end{tabular} & \begin{tabular}[c]{@{}l@{}}\%\\ Difference\end{tabular} \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SLO/\\ SLN\end{tabular}    & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   & \begin{tabular}[c]{@{}l@{}}SLN\end{tabular}   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% 100:7                                                                        & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 2                                                       & 71.42                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 3                                                       & 57.14                                                   \\ \hline
% 100:3                                                                        & SLN                                                   & 10                                                      & 0                                                       & \begin{tabular}[c]{@{}l@{}}SLN\end{tabular}    & 1                                                       & 85.71                                                   & SLN                                                   & 10                                                      & 0                                                       & SLN                                                   & 1                                                       & 85.71                                                   \\ \hline
% \end{tabular}
% \end{table*}

% In table \ref{tab:relsumm}, we show the best method for each compression ratio under the respective relative angle buckets along with its difference with that of whole set.  We explicitly focus on the relative angle affordance since it is a key factor in episode completion. We can observe that SLN turns out as the best performing method for the turn buckets while Uniform Skip turns out the best for Straight road. This can be attributed to the observation we made where SLN turned out as the best method in episode completion task. We have given a detailed analysis on the affordance predictions in the next subsections.




% \begin{table*}[]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in training conditions}}
% \label{tab:trainepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{9}{|c|}{Episode Completion Tasks}                                                                                                                                                                                                                                                                                                                                  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{2}{c|}{Straight}                                                        & \multicolumn{2}{c|}{One-Turn}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Straight \\ Dynamic\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}} \\ \cline{2-9} 
%                                                                              & Best Method                                                             & Difference & Best Method             & Difference & Best Method                                & Difference                          & Best Method                             & Difference                            \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT/SIFT+Loss-O/\\ SIFT+Loss-N\end{tabular} & 0          & SIFT+Loss-N             & 3          & SIFT/SIFT+Loss-N                           & 0                                   & SIFT+Loss-N                             & 3                                     \\ \hline
% 100:7                                                                        & SIFT+Loss-N                                                             & 0          & SIFT+Loss-N             & 6          & SIFT+Loss-N                                & 0                                   & SIFT+Loss-N                             & 6                                     \\ \hline
% 100:3                                                                        & SIFT+Loss-N                                                             & 0          & SIFT+Loss-O/SIFT+Loss-N & 8          & SIFT+Loss-N                                & 0                                   & SIFT+Loss-O                             & 8                                     \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for episode completion in testing conditions}}
% \label{tab:testepsumm}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{9}{|c|}{Episode Completion Tasks}                                                                                                                                                                                                                                                                                                                             \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{2}{c|}{Straight}                                                   & \multicolumn{2}{c|}{One-Turn}        & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Straight \\ Dynamic\end{tabular}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}One-Turn\\ Dynamic\end{tabular}} \\ \cline{2-9} 
%                                                                              & Best Method                                                        & Difference & Best Method             & Difference & Best Method                             & Difference                             & Best Method                             & Difference                            \\ \hline
% 100:20                                                                       & \begin{tabular}[c]{@{}l@{}}SIFT+Loss-O/\\ SIFT+Loss-N\end{tabular} & 0          & SIFT+Loss-N             & 4          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 4                                     \\ \hline
% 100:7                                                                        & SIFT+Loss-N                                                        & 0          & SIFT+Loss-N             & 5          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 5                                     \\ \hline
% 100:3                                                                        & SIFT+Loss-N                                                        & 0          & SIFT+Loss-O/SIFT+Loss-N & 6          & SIFT+Loss-N                             & 0                                      & SIFT+Loss-N                             & 6                                     \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% \label{tab:relsumm}
% \captionsetup{justification=centering}
% \caption{\textbf{Summary result listing the best method for relative angle affordance prediction}}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multicolumn{6}{c|}{Relative Angle buckets}                                                                                                                                                                                                                                                                                                                     \\ \cline{2-7} 
%                                                                              & \multicolumn{2}{c|}{Left-Turn}                                                                                      & \multicolumn{2}{c|}{Straight-Road}                                                                                  & \multicolumn{2}{c|}{Right-Turn}                                                                                     \\ \cline{2-7} 
%                                                                              & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} & \multicolumn{1}{c|}{Best Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Difference\\ in MAE\end{tabular}} \\ \hline
% 100:20                                                                       & SIFT                             & 0.02                                                                             & Uniform Skip                     & 0.01                                                                             & SIFT+Loss-N                      & 0.01                                                                             \\ \hline
% 100:7                                                                        & SIFT                             & 0.03                                                                             & Uniform Skip                     & 0.01                                                                             & SIFT+Loss-N                      & 0.01                                                                             \\ \hline
% 100:3                                                                        & SIFT+Loss-N                      & 0.06                                                                             & SIFT+Loss-O                      & 0.02                                                                             & SIFT+Loss-N                      & 0.02                                                                             \\ \hline
% \end{tabular}
% \end{table*}
% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:20 compression ratio}}
% \label{tab:ep5}

% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 3                                                          & 8        & 3                                                          & 9        & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
%                                                                              & Only SIFT                                                   & 10       & 7                                                          & 10       & 7                                                          & 10       & 7                                                          & 9        & 6                                                          \\ \cline{2-10} 
%                                                                             & Only Loss                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & PRL                                                    & 9        &  8                                                         & 9        & 8                                                          & 7       &  7                                                         & 7        & 7                                                          \\ \cline{2-10} 
%                                                     & SubM                                                    & 9        &  7                                                         & 9        & 7                                                          & 9       &  7                                                         & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & STL                                                    & 10       & 8                                                         & 10       & 7                                                          & 10       & 9                                                          & 10       & 9 
%                                 \\ \cline{2-10} 
%                                                                              & SML                                                    & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       &\textbf{10}                                \\        \hline
% % \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 2                                                          & 8        & 2                                                          & 9        & 3                                                          & 7        & 3                                                          \\ \cline{2-10} 
% %                                                                              & SIFT                                                   & 9        & 4                                                          & 9        & 4                                                          & 8        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
% %                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         &                                                           \\ \cline{2-10} 
% %                                                                              & SLN                                                    & 10       & \textbf{6}                                                          & 10       & \textbf{6}                                                          & 10       & \textbf{8}                                                          & 10       & \textbf{8}                                                          \\ \hline
% % \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 9        & 1                                                          & 8        & 0                                                          & 9        & 2                                                          & 8        & 2                                                          \\ \cline{2-10} 
% %                                                                              & SIFT                                                   & 8        & 0                                                          & 8        & 0                                                          & 8        & 1                                                          & 9        & 0                                                          \\ \cline{2-10} 
% %                                                                              & SLO                                                    &         &                                                           &         &                                                           &         &                                                           &         & 0                                                          \\ \cline{2-10} 
% %                                                                              & SLN                                                    & 10       & \textbf{5}                                                          & 10       & \textbf{5}                                                          & 10       & \textbf{6}                                                          & 9       & \textbf{6}                                                          \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:7 compression ratio}}
% \label{tab:ep15}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
%                                                                              &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
% \multirow{4}{*}{100:7}                                                      & \begin{tabular}[c]{@{}l@{}}Only SIFT\end{tabular} & 9        & 5                                                          & 9        & 5                                                           & 9        & 4                                                          & 9        & 4                                                          \\ \cline{2-10} 
%                                                                             & Only Loss                                                   & 10        & 6                                                          & 10       & 6                                                          &    9    & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
%                                                                              & PRL                                                    & 9        & 5                                                            & 9        & 5                                                          & 7        &  4                                                         & 7        & 4                                                          \\ \cline{2-10}
%                                                                              & SubM                                                    & 9        & 3                                                            & 9        & 3                                                          & 9        & 2                                                          & 9        & 2                                                          \\ \cline{2-10}
%                                                                              & STL                                                    & 10       & 7                                                          & 10        & 7                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}  
%                                 \\ \cline{2-10} 
%                                                                              & SML                                                    & 10       & \textbf{8}                                                           & 10       & \textbf{8}                                                          & 10       &\textbf{9}                                                           & 10       & \textbf{9}                                 \\        \hline
% \end{tabular}
% \end{table*}

\begin{table*}[]
%\footnotesize
\scriptsize
\centering
\captionsetup{justification=centering}
\caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training and test conditions for 100:20 and 100:7 compression ratio}}
\label{tab:ep5_15}

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Training\\ Conditions\end{tabular}}                                                            & \multicolumn{4}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Conditions\end{tabular}}                                                                \\ \cline{3-10} 
                                                                             &                                                        & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} & Straight & One-Turn & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & \begin{tabular}[c]{@{}l@{}}One-Turn\\ Dynamic\end{tabular} \\ \hline
                                                                             & WS    & 10       & 10                                                         & 10        & 10                                                          & 10       & 10                                                         & 10        & 10                                                          \\ \hline
\multirow{4}{*}{100:20}                                                      & US & 9        & 3                                                          & 8        & 3                                                          & 9        & 5                                                          & 9        & 5                                                          \\ \cline{2-10} 
                                                                             & OS                                                   & 10       & 7                                                          & 10       & 7                                                          & 10       & 7                                                          & 9        & 6                                                          \\ \cline{2-10} 
                                                                            & OL                                                   & 10       & 6                                                          & 10       & 6                                                          & 10       & 7                                                          & 9        & 7                                                          \\ \cline{2-10} 
                                                                             & MCL                                                    & 9        &  8                                                         & 9        & 8                                                          & 7       &  7                                                         & 7        & 7                                                          \\ \cline{2-10} 
                                                    & SBML                                                    & 9        &  7                                                         & 9        & 7                                                          & 9       &  7                                                         & 9        & 7                                                          \\ \cline{2-10} 
                                                                             & CTL                                                    & 10       & 8                                                         & 10       & 7                                                          & 10       & 9                                                          & 10       & 9 
                                \\ \cline{2-10} 
                                                                             & CBML                                                    & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       & \textbf{10}                                                          & 10       &\textbf{10}                                \\        \hline
                                                        \hline
\multirow{4}{*}{100:7}                                                      & \begin{tabular}[c]{@{}l@{}}MCL\end{tabular} & 9        & 5                                                            & 9        & 5                                                          & 7        &  4                                                         & 7        & 4                                                          \\ \cline{2-10}
                                                                             & SBML                                                    & 9        & 3                                                            & 9        & 3                                                          & 9        & 2                                                          & 9        & 2                                                          \\ \cline{2-10}
                                                                             & CTL                                                    & 10       & 7                                                          & 10        & 7                                                          & 10       & \textbf{9}                                                          & 10       & \textbf{9}  
                                \\ \cline{2-10} 
                                                                             & CBML                                                    & 10       & \textbf{8}                                                           & 10       & \textbf{8}                                                          & 10       &\textbf{9}                                                           & 10       & \textbf{9}                                 \\        \hline                                                    
\end{tabular}
\end{table*}



\subsection{Comparison of Methods: Episode Completion}



In this section, we will study the performance of different subset selection techniques on the basis of episode completion which is the main intended objective.

We consider four tasks under episode completion which had been originally defined in \cite{dosovitskiy2017carla}:
\begin{enumerate}
    \item Straight : The episode comprises of pairs of points which are straight roads.
    \item One-Turn : The episode comprises of pairs of points which include left or right turn in their paths.
    \item Straight Dynamic : Similar to \textit{Straight} task, it occurs in the presence of other vehicles and pedestrians.
    \item One-Turn Dynamic : Similar to \textit{One-Turn} task in the presence of other vehicles and pedestrians.
\end{enumerate}

We show in Table \ref{tab:ep5_15} the performance of CAL model\cite{sauer2018conditional}  trained on subsets, obtained by various selection techniques, by simulating it with the CARLA \cite{dosovitskiy2017carla} simulator.


We report number of successfully completed episodes (out of a total of 10 episodes) for each subtask in training and test conditions. We observe that the tasks - \textit{Straight} and \textit{Straight Dynamic} are fairly easy to accomplish for all subset selection methods. The challenge arises in the other two tasks where we see a large number of unsuccessful episodes.

The completion of episodes in turns, largely depends on the affordance \textit{Relative Angle} which as we mentioned, provides the steering angle of the agent vehicle. We observe that Uniform Skip (US) is unable to complete majority of the turns in training or test conditions. This is due to the inherent nature of selection of US method, which does not take the important frame sequences into consideration.


% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     \centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[height=3cm]{figures/frac_rel_rh1_e1_MCL_New.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     \includegraphics[height=3cm]{figures/frac_rel_rh1_e2_MCL_New.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for sample episodes (a) and (b) with turns for $\rho = \{0.1 , 0.25\}$. The proposed method selects more fraction of instances from the area with turns, which becomes crucial for the task of episode completion.}}
%     \label{fig:deviate}
% \end{figure}


% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     % \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/deviation_dist_PRL.pdf}
%     \includegraphics[width=\textwidth,height=3cm]{figures/turn_123_26.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/turn_94_31.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \centering
%     \begin{subfigure}{0.4\columnwidth}
%     \centering
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_r1_MCL_New.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.4\columnwidth}
%     \centering
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_r25_e1_MCL_New.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     % \centering
%     % \begin{subfigure}{0.4\columnwidth}
%     % \centering
%     % % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_r4_e1_MCL_New.pdf}
%     % %\caption{Red light Affordance Distribution}
%     % \caption{}
%     % \label{fig:tskip5}
%     % \end{subfigure}
%     \centering
%     \begin{subfigure}{0.4\columnwidth}
%     \centering
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_r1_e2_MCL_New.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.4\columnwidth}
%     \centering
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_r25_e2_MCL_New.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     % \centering
%     % \begin{subfigure}{0.4\columnwidth}
%     % \centering
%     % % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
%     % \includegraphics[width=\textwidth,height=3cm]{figures/frac_r4_e2_MCL_New.pdf}
%     % %\caption{Red light Affordance Distribution}
%     % \caption{}
%     % \label{fig:tskip5}
%     % \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for sample episodes (a) and (b) with turns in figures (c), (d), and (e), (f) for $\rho = \{0.1 , 0.25\}$ respectively. The proposed method selects more fraction of instances from the area with turns, which becomes crucial for the task of episode completion.}}
%     \label{fig:deviate}
% \end{figure*}


% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/relangle_episode.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/relloss_episode.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{A temporal plot of an episode with (a) the relative angle affordance value (b) its corresponding relative angle loss values in the respective frames.}}
%     \label{fig:lossrel}
% \end{figure}
%\vspace{-1mm}
\begin{figure*}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/deviation_dist_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/deviation_episode_MCL_whole.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \caption{}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/deviation_episode_error_MCL_whole_label.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.6\columnwidth}
    \centering
    % \includegraphics[width=\textwidth,height=3cm]{figures/frac_PRL.pdf}
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_MCL.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{Anecdotal example of a sample episode showing (a) the region of failure by MCL (b) the corresponding errors and (c) fraction of selected instances from those regions. CBML selects more fraction of instances from regions important for episode completion.}}
    \label{fig:deviate}
\end{figure*}
% One of the 

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
    
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_20.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_20.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redllight_15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turn_15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_100_3.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_100_3.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip30}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of ground-truth affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7, (\textit{bottom}) 100:3 compression ratio}}
%     \label{fig:distribhist}
% \end{figure}

On the other hand, OS, OL, MCL, SBML complete some of the turn episodes, with CBML completing the highest of all methods (100\% both in training and test conditions) followed by CTL. This is due to the consideration of pointwise metric - bucketwise relative angle aided with remaining multi task losses in Equation \ref{eqn:newsiftloss} along with pairwise metric SIFT dissimilarity, which leads to the selection of important frames. We also report the episode completion numbers for 100:7 compression ratio in Table \ref{tab:ep5_15}, for two baselines - MCL and SBML and the proposed method. We can observe that CTL and CBML continue to perform better compared to the other baselines with CBML completing 80\% and 90\% episodes in training and test conditions even after dropping 93\% of the frames.

% As mentioned under Multi-task criteria, we observe that Relative Angle affordance turns out to be vital in the task of episode completion. We can divide the entire range of Relative Angle affordance value across 20 buckets ranging from -1.0 to +1.0. Note that buckets corresponding to (-1.0 to -0.1) and (0.1 to 1.0) approximately indicate the left and right turns. 

% In Figure \ref{fig:lossrel}, we show an entire sequence of frames of an episode with its corresponding \textit{Relative Angle} affordance value and its respective loss value.  As seen from the figure, which is one of the left turn episodes, we can notice the higher relative angle loss values at the turn. This essentially shows us the need for selection of such frames in order to have successful episodes. So, using the above intuition, we fine-tune the weights corresponding to the bucket-wise relative angle loss values and feed in our subset selection framework SML.


% One of the possible reasons of success can be attributed to Figure \ref{fig:bucketprop5} where we see that SML has a higher fraction of selected instances for most of the buckets than all other methods which essentially portrays its effectiveness. Only Loss also selects fairly large fraction of instances for some of the buckets. However, it only concentrates on the frames which incur a high loss value. The completion of an episode relies on various other factors like perceptual difference and having only frames with high end-task losses in the compressed sequence does not lead to an effective result.


We show an anecdotal example of a failed episode from MCL \cite{das2020multi} method in Figure \ref{fig:deviate} and try to analyse the reason behind it. In Figure \ref{fig:deviate}a, we show a plot of an episode with distance covered vs Relative Angle affordance. The cumulative distance is chosen as an axis of reference in order to make the comparison spatially similar for all the methods. Overall, the agent vehicle in the simulator is resilient to errors. However, we can observe the gradual deviation of MCL \cite{das2020multi} method and its accumulated errors which lead to an incomplete episode. We can also relate the region of failures to the corresponding relative angle errors in Figure \ref{fig:deviate}b where we observe that overall, MCL \cite{das2020multi} is having a higher error compared to proposed method CBML and model trained on the whole set. This occurs because we fine-tune the weights corresponding to the bucket-wise relative angle loss values and feed in our subset selection framework CBML along with pairwise metric. We also show the fraction of selected instances by both the selection methods, in Figure \ref{fig:deviate}c from the same region, and we can observe that CBML selects more fraction of instances in the area right before the turn and during the turn, which eventually help in its completion.
We discuss the next subtask - affordance prediction in the following subsection.



% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_left.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \caption{}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_straight.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{AISTATS2021PaperPack/figures/frac_right.pdf}
    
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for subset selection methods for 100:20 compression ratio}}
%     \label{fig:fracall}
% \end{figure*}


% We show in Figure \ref{fig:deviate} three instances of the points of deviation where three of the baselines - Only SIFT, Only Loss and PRL fail in completing their respective episodes. The buckets correspond to the areas in the town where the models trained using Only SIFT, Only Loss and PRL had deviated leading to incomplete episode. We can clearly observe that the error corresponding to SML and STL are considerably lower which make them reach the end goal.

% We show in Figure \ref{fig:deviate} three instances of the points of deviation where three of the baselines - Only SIFT, Only Loss and PRL fail in completing their respective episodes. We have run the simulator using the ground truth affordances and the individual trained model's predicted affordances. We kept a track of the predicted relative angle along with the covered cumulative distance. Note that the change in relative angle values (y-axis) arise when turns appear. We can observe in both the plots, that the agent vehicle started deviating more using the Only Loss and PRL method right before turns, leading to intersection with the sidewalk thus failing to complete the episode.  The points immediately before the turn are important for consideration since those mark the intersecting points or junctions. We can see in both the plots that our gradation method - STL and SML appear to predict values closer to the ground truth during the intersection points while Only Loss (left) and PRL (right) methods  begin deviating at the intersections leading to failures. The loss values in these buckets (-0.1 to 0.1) are not considerably higher due to presence of large number of training samples in these buckets since the relative angle values for the straight roads also fall in them. Hence, Only Loss selects lesser number of instances from these buckets leading to failure.  On the other side, PRL takes SIFT and Loss into consideration, but due to its drawback as described in section, it also fails in completing all the turns. Both SML and STL take pairwise and pointwise metric into consideration during selection of frames and result in more successful episodes. SML performs better than STL due to the inclusion of SIFT and weighted losses which help in selection of more important frames. 
% A wrong prediction in relative angle at certain points may take the vehicle to waypoints from which recovering back without manual intervention would not be possible.
% STL even though predicts closer to ground truth values than SML at the junctions, yet it is not able to complete all the episodes since the turns after the intersection is vital too and we can observe in the plots that STL predicts better at those.
% It can also be seen that the number of successfully completed episodes with STL is considerably less than SML but reasonably better than the other methods. The consideration of both pairwise and pointwise metric (total loss) lead to its better selection of frames, however the weighted multi-task loss has led to an added benefit.
% Note that 100:7 and 100:3 is very high in comparison to the 63000 frames dataset we collected. The original model \cite{sauer2018conditional} was trained on 10x amount of data we have used in our experiments. We expect that the successful completion rate will increase with increasing dataset size.

% We have also performed experiments on the subset selection method using only relative angle loss as the pointwise metric, to which it did not yield good results. One potential future work can be to use different components of the six affordance losses and weighing them according to its importance in episode completion. 

% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 97.39                                                                     & 97.41                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 96.72                                                                     & 97.03                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & Only SIFT                                                   & 96.11                                                                     & 96.07                                                                     &                                                          &                                                          \\ \cline{2-6}
%                         & Only Loss                                                   & 92.31                                                                     & 91.08                                                                     &                                                          &                                                          \\ \cline{2-6}
%                         & PRL                                            &  91.63                                                                    & 89.73                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & STL                                            & 96.38                                                                     & 96.05                                                                     &                                                          &
%                       \\ \cline{2-6} 
%                         & SML                                            & 93.98                                                                     & 92.83                                                                     &                                                          &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 92.63                                                                     & 91.94                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 89.55                                                                     & 87.23                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 94.72                                                                      & 94.54                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 97.12                                                                     & 97.04                                                                      &                                                          &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.06                                                                     & 93.09                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 94.16                                                                     & 93.54                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 90.12                                                                     & 94.41                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 94.42                                                                      & 93.72                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Red Light affordance}}
% \label{tab:redlaff}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Method                                              & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                             & WS                                                  & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                     & US                                                  & 96.72                                                    & 97.03                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 96.11                                                    & 96.07                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 92.31                                                    & 91.08                                                    \\ \cline{2-4} 
%                                                             & PRL                                                 & 91.63                                                    & 89.73                                                    \\ \cline{2-4} 
%                                                             & STL                                                 & 96.38                                                    & 96.05                                                    \\ \cline{2-4} 
%                                                             & SML                                                 & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{table}


% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \label{tab:hazaff}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Method                                              & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                             & WS                                                  & 99.44                                                    & 99.72                                                    \\ \hline
% \multirow{6}{*}{100:20}                                     & US                                                  & 99.14                                                    & 99.47                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    \\ \cline{2-4} 
%                                                             & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     \\ \cline{2-4} 
%                                                             & PRL                                                 & 99.43                                                    & 98.39                                                    \\ \cline{2-4} 
%                                                             & STL                                                 & 99.31                                                    & 99.61                                                    \\ \cline{2-4} 
%                                                             & SML                                                 & 99.45                                                    & 99.71                                                    \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
% \label{tab:redrhazaff}
% \begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                                              & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
%                                                                              & PRL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
%                         & SubM                                                 & 99.25                                                    &                                                     & 94.33                                                    &                                                     \\ \cline{2-6}                                                     & STL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
%                                                                              & SML                                                 & 99.45                                                    & \begin{tabular}[c]{@{}l@{}}99.71\\ (1.32\%)\end{tabular}                                           & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{table}




% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Hazard Stop affordance}}
% \begin{tabular}{|l|l|l|l|l|p{8mm}|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{2}{l|}{\% Improvement}                                                                                 \\ \cline{5-6} 
%                         &                                                        &                                                                           &                                                                           & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 99.44                                                                     & 99.72                                                                     &                                                          &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.14                                                                     & 99.47                                                                      &                                                          &                                                          \\ \cline{2-6} 
%                         & Only SIFT                                                   & 99.11                                                                     & 99.56                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & Only Loss                                                   & 99.41                                                                     & 99.6                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & PRL                                            & 99.43                                                                     & 98.39                                                                     &                                                          &                                                          \\ \cline{2-6} 
%                         & SLT                                            & 99.23                                                                     & 99.61                                                                     &                                                          &
%                         \\ \cline{2-6} 
%                         & SLM                                            & \textbf{99.45}                                                                     & \textbf{99.71}                                                                     &                                                          &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 99.42                                                                     & 97.07                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 99.31                                                                     & 98.99                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 99.39                                                                      & 98.37                                                                      &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 99.45                                                                     & 98.76                                                                      &                                                          &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 98.57                                                                     & 97.67                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SIFT                                                   & 99.29                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLO                                            & 99.39                                                                     & 98.64                                                                     &                                                          &                                                          \\ \cline{2-6} 
% %                         & SLN                                            & 99.12                                                                      & 98.23                                                                     &                                                          &                                                          \\ \hline
% \end{tabular}
% \label{tab:hazaff}
% \end{table}
% \begin{table}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|p{12mm}|p{8mm}|l|p{15.5mm}|l|p{15.5mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                               & MAE           & \%Improvement         & MAE            & \%Improvement           \\ \cline{3-6} 
%                                                                              &                                                        & \multicolumn{2}{l|}{Vehicle Distance} & \multicolumn{2}{l|}{Centerline Distance} \\ \hline
%                                                                              & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.03          &                       & 0.05           &                         \\ \hline
% \multirow{4}{*}{100:20}                                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.05           &                         \\ \cline{2-6} 
%                                                                              & Only SIFT                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6}
%                                                                              & Only Loss                                                   & 0.09          &                  & 0.08          &                      \\ \cline{2-6}
%                                                                              & PRL                                                    & 0.05          &                   & 0.06           &                    \\ \cline{2-6} 
%                                                                              & SLT                                                    & 0.05          & 44.44                  & 0.05           & 37.5
%                                           \\ \cline{2-6} 
%                                                                              & SLM                                                    & \textbf{0.04}          &    55.55               & 0.05           & 37.5                                  
%                                                                              \\ \hline
% % \multirow{4}{*}{100:7}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06          &                       & 0.06           &                         \\ \cline{2-6} 
% %                                                                              & SIFT                                                   & 0.09          &                 & 0.08           &                      \\ \cline{2-6} 
% %                                                                              & SLO                                                    & 0.09          & 0.09                 &            &                      \\ \cline{2-6} 
% %                                                                              & SLN                                                    & 0.07          &                   & 0.06           &                     \\ \hline
% % \multirow{4}{*}{100:3}                                                       & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.07          &                       & 0.09           &                         \\ \cline{2-6} 
% %                                                                              & SIFT                                                   & 0.11          &                  & 0.08           &                     \\ \cline{2-6} 
% %                                                                              & SLO                                                    & 0.09          & 0.09                 &            &                      \\ \cline{2-6} 
% %                                                                              & SLN                                                    & 0.06          &                  & 0.06           &                     \\ \hline
% \end{tabular}
% \end{table}




%\tr{TBD}

% \begin{table}[]
% \begin{tabular}{|l|p{2mm}|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ratio\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\\ (Macro)\end{tabular}}                   & \multicolumn{4}{c|}{MAE}                                                                                                                                                                                \\ \cline{3-8} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}CAL\\ RL\end{tabular}        & \begin{tabular}[c]{@{}l@{}}TS\\ RL\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ RA\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ CD\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ CD\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                       &                                                                              & \begin{tabular}[c]{@{}l@{}}95.86\\ (95.16)\end{tabular} & \begin{tabular}[c]{@{}l@{}}95.86\\ (95.16)\end{tabular}                                               &\begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05 \end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                                 & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                                \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:20}}                                 &
% \begin{tabular}[c]{@{}l@{}}95.32\\ (94.7)\end{tabular} & \begin{tabular}[c]{@{}l@{}}95.54\\ (94.82)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.06\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}91.36\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.09\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                &                                                  &                                                &                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}89.18\\ (87.25)\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}}90.52 \\(88.26)\end{tabular}                                                & 0.07                                                 & 0.06                                                & 0.09                                                 & 0.10                                                \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:7}}                                 & \begin{tabular}[c]{@{}l@{}}91.94 \\ (91.08)\end{tabular} & \begin{tabular}[c]{@{}l@{}}94.58\\ (95.02)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}0.05\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.10\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8}
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}90.28\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 

% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}89.7\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.08                                                 &                                                 & 0.11                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}85.76\\ (83.67)\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.07                                                 &                                                 & 0.11                                                &                                                 \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                    & \multicolumn{1}{c|}{\multirow{3}{*}{100:3}}                                 & \begin{tabular}[c]{@{}l@{}} 91.72\\ (91.27)\end{tabular} & \begin{tabular}[c]{@{}l@{}}93.58\\ (92.60)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.08\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}} 0.06\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}} 0.11\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.11\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8}
% \begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}                    & \multicolumn{1}{c|}{}                                 & \begin{tabular}[c]{@{}l@{}}90.04\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.07\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}0.10\end{tabular}                                                & \begin{tabular}[c]{@{}l@{}}\end{tabular}                                                                                             \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}87.68\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                & 0.08                                                 &                                                 & 0.12                                                 &                                                 \\ \cline{1-1} \cline{3-8} 
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}                     & \multicolumn{1}{c|}{}                                                        & \begin{tabular}[c]{@{}l@{}}\\ ()\end{tabular}                                                        &\begin{tabular}[c]{@{}l@{}} \\()\end{tabular}                                                &                                                  &                                                 &                                                 &                                                 \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques in terms of affordance accuracies}
% \label{afftable}
% \end{table}

% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.15                                                      & 0.02                                                          & 0.08                                                       & 0.09                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                              & 0.08                                                           & 0.07                                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 95.32                                                    & 94.7                                                     & 0.39                                                      & 0.03                                                          & 0.09                                                       & 0.09                                                          & 95.54                                                    & 94.82                                                    & 0.28                                                          & 0.03                                                              & 0.07                                                           & 0.09                                                          \\ \hline
% SIFT                                                                               & 91.36                                                    & 88.12                                                         & 0.17                                                      & 0.06                                                          & 0.09                                                       & 0.09                                                          & 91.9                                                         & 90.75                                                         & 0.16                                                          & 0.05                                                              & 0.14                                                           & 0.09                                                              \\ \hline
% SIFT+Loss-O                                                                        & 88.34                                                         & 86.96                                                         & 0.19                                                      & 0.07                                                          & 0.08                                                       & 0.09                                                              & 89.94                                                         & 87.79                                                         & 0.17                                                          & 0.04                                                              & 0.08                                                           & 0.08                                                              \\ \hline
% SIFT+Loss-N                                                                        & 89.18                                                    & 88.25                                                    & 0.18                                                      & 0.05                                                          & 0.07                                                       & 0.09                                                          & 90.52                                                    & 89.26                                                    & 0.16                                                          & 0.05                                                              & 0.08                                                           & 0.08                                                          \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:20}
% \label{afftable1}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.19                                                      & 0.03                                                          & 0.08                                                       & 0.08                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                              & 0.08                                                           & 0.07                                                               \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 91.94                                                    & 91.08                                                     & 0.38                                                      & 0.04                                                          & 0.11                                                       & 0.11                                                          & 94.58                                                    & 95.02                                                    & 0.27                                                          & 0.04                                                              & 0.09                                                           & 0.10                                                          \\ \hline
% SIFT                                                                               & 90.28                                                    & 90.1                                                         & 0.18                                                     & 0.06                                                          & 0.14                                                       & 0.11                                                          & 90.1                                                         & 88.58                                                         & 0.17                                                           & 0.05                                                              & 0.16                                                           & 0.09                                                              \\ \hline
% SIFT+Loss-O                                                                        & 89.7                                                         & 89.8                                                         & 0.19                                                      & 0.05                                                          & 0.13                                                       &  0.11                                                             & 91.76                                                         & 91.4                                                         & 0.21                                                          & 0.05                                                              & 0.11                                                           & 0.11                                                              \\ \hline
% SIFT+Loss-N                                                                        & 87.04                                                    &                                                     & 0.21                                                      & 0.10                                                          & 0.06                                                       & 0.12                                                          & 91.32                                                    &                                                     & 0.19                                                          & 0.08                                                              & 0.06                                                           & 0.14                                                          \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:7}
% \label{afftable2}
% \end{table*}

% \begin{table*}[]
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\\Data\\ Gradation\\ Method\end{tabular}} & \multicolumn{6}{c|}{CAL Model}                                                                                                                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{Timestamp Model}                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-13} 
%                                                                                   & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} & \multicolumn{2}{c|}{Red Light}                                                                                      & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Relative\\ Angle\end{tabular}}                                                                                                          & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \cline{2-13} 
%                                                                                   & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \multicolumn{1}{c|}{MAE}                                      \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}                                & 95.86                                                    & 95.16                                                    & 0.19                                                      & 0.03                                                          & 0.08                                                       & 0.08                                                          & 96.26                                                         & 95.43                                                         & 0.15                                                          & 0.02                                                               & 0.08                                                           & 0.07                                                              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                             & 91.26                                                    & 90.36                                                      & 0.44                                                      & 0.6                                                          & 0.15                                                       & 0.11                                                          & 93.58                                                    & 92.60                                                    & 0.32                                                          & 0.05                                                              & 0.09                                                           & 0.11                                                          \\ \hline
% SIFT                                                                               & 90.04                                                    & 90.34                                                         & 0.32                                                     & 0.06                                                          & 0.15                                                       & 0.11                                                          & 91.87                                                         & 89.02                                                         & 0.28                                                          & 0.05                                                              & 0.14                                                           &  0.09                                                             \\ \hline
% SIFT+Loss-O                                                                        & 87.68                                                         & 88.54                                                         & 0.26                                                      & 0.05                                                          & 0.16                                                       & 0.11                                                              & 91.36                                                         & 90.78                                                         & 0.23                                                          & 0.07                                                              & 0.11                                                           & 0.13                                                              \\ \hline
% SIFT+Loss-N                                                                        & 86.08                                                    & 85.54                                                    & 0.22                                                      & 0.08                                                          & 0.06                                                       & 0.13                                                          &                                                     &                                                     &                                                           &                                                               &                                                            &                                                           \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques using Conditional Affordance Learning Model and Timestamp Model for compression ratio of 100:3}
% \label{afftable3}
% \end{table*}




% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Ratio\end{tabular}} & \multirow{2}{*}{Tasks}                                     & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Train\\ Poses\end{tabular}}                               & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Test\\ Poses\end{tabular}}                                \\ \cline{4-7} 
%                                                                           &                                                                              &                                                            & \begin{tabular}[c]{@{}l@{}}CAL\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}CAL\\ Model\end{tabular} & \begin{tabular}[c]{@{}l@{}}TS\\ Model\end{tabular} \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}}      & \multirow{4}{*}{}                                                            & Straight                                                   & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 9                                                    &                                                    & 7                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 8                                                    &                                                    & 7                                                    &                                                    \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:20}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 0                                                    & 0                                                   & 1                                                    & 0                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &  8                                                   & 9                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 0                                                    & 0                                                   & 1                                                    & 0                                                   \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   & 10                                                    &                                                    & 10                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 2                                                    &                                                    & 1                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    &                                                    & 9                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 2                                                    &                                                    & 1                                                    &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &  10                                                   & 9                                                   & 10                                                    & 9                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 9                                                   & 9                                                    & 8                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   & 10                                                    & 10                                                   & 10                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   & 6                                                    &                                                    & 3                                                    &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 10                                                    & 10                                                   & 10                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} & 6                                                    &                                                    & 3                                                    &                                                    \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:7}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 10                                                   & 7                                                     & 10                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\
                                    
%                                 \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{12}{*}{100:3}                                                     & Straight                                                   & 9                                                    & 10                                                   & 9                                                    & 10                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} & 8                                                    & 9                                                   & 8                                                    & 9                                                   \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7}                                                                           
                                                                          
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{1-1} \cline{3-7} 
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}    &                                                                              & Straight                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & One Turn                                                   &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\ \cline{3-7} 
%                                                                           &                                                                              & \begin{tabular}[c]{@{}l@{}}One Turn\\ Dynamic\end{tabular} &                                                     &                                                    &                                                     &                                                    \\
%                                     \hline
% \end{tabular}
% \label{eptable}
% \end{table}





% \begin{table*}[h!]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in training conditions}}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Episodes}                             \\ \cline{3-6} 
%                                                                              &                          & Straight & One-Turn & Straight Dynamic & One-Turn Dynamic \\ \hline
%                                                                              & Whole Set                & 10       & 9        & 10               & 9                \\ \hline
% \multirow{4}{*}{100:20}                                                      & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 10       & 2        & 10               & 2                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 10       & 3        & 8                & 2                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 6        & 10               & 6                \\ \hline
% \multirow{4}{*}{100:7}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 9        & 2        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 2        & 9                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 3        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:3}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8         & 1        & 8                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 8                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10         & 1         & 10                 & 0                 \\ \hline
% \end{tabular}
% \label{tab:eptabletrain}
% \end{table*}


% \begin{table*}[h!]
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques in terms of episode completion in test conditions}}
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Episodes}                             \\ \cline{3-6} 
%                                                                              &                          & Straight & One-Turn & Straight Dynamic & One-Turn Dynamic \\ \hline
%                                                                              & Whole Set                & 10       & 7        & 10               & 7                \\ \hline
% \multirow{4}{*}{100:20}                                                      & Uniform Skip             & 9        & 1        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT                     & 10       & 1        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 10       & 2        & 9                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 3        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:7}                                                       & Uniform Skip             & 9        & 0        & 7                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8        & 1        & 8                & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 9                 & 1                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10       & 2        & 10               & 3                \\ \hline
% \multirow{4}{*}{100:3}                                                       & Uniform Skip             & 9        & 0        & 8                & 0                \\ \cline{2-6} 
%                                                                              & SIFT                     & 8         & 1        & 7                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-O              & 9         & 1        & 8                 & 0                \\ \cline{2-6} 
%                                                                              & SIFT+Loss-N              & 10         & 1         & 10                 & 1                 \\ \hline
% \end{tabular}
% \label{tab:eptabletest}
% \end{table*}


\begin{table*}
\noindent\scriptsize
\begin{minipage}[b]{0.4\linewidth}
    \centering
\caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
\label{tab:redrhazaff}
\begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
                                                                             &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
                                                                             & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
\multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
                                                                             & OS & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
                                                                             & OL & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
                                                                             & MCL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
                        & SBML                                                 & 99.25                                                    & 99.60                                                    & 94.33                                                    & 93.91                                                    \\ \cline{2-6}                                                     & CTL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
                                                                             & CBML                                                 & 99.45                                                    & 99.71                                            & 93.98                                                    & 92.83                                                    \\ \hline
\end{tabular}
\end{minipage}
\hspace{2cm}
\begin{minipage}[b]{0.4\linewidth}
\caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
\label{tab:vehcen}
\begin{tabular}{|l|l|l|l|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
                                                                             &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
\multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
                                                                             & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
                                                                             & OS & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
                                                                             & OL & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
                                                                             & MCL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                                                    & SBML                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
                                                                            & CTL                                                 & 0.05
                                                                 &0.05                                 \\ \cline{2-4} 
                                                                             & CBML                                                 & 0.04
                                                                 &0.05                                 \\ \hline
\end{tabular}
\end{minipage}
\end{table*}


\subsection{Comparison of Methods: Affordance Accuracies}

% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Hazard Stop and Red Light affordance}}
% \label{tab:redrhazaff}
% \begin{tabular}{|p{13.5mm}|p{8mm}|p{9mm}|p{9mm}|p{9mm}|p{9mm}|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Method}                             & \multicolumn{2}{c|}{Hazard Stop}                                                                                    & \multicolumn{2}{c|}{Red Light}                                                                                      \\ \cline{3-6} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
%                                                                              & WS                                                  & 99.44                                                    & 99.72                                                    & 97.39                                                    & 97.41                                                    \\ \hline
% \multirow{6}{*}{100:20}                                                      & US                                                  & 99.14                                                    & 99.47                                                    & 96.72                                                    & 97.03                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 99.11                                                    & 99.56                                                    & 96.11                                                    & 96.07                                                    \\ \cline{2-6} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 99.41                                                    & 99.6                                                     & 92.31                                                    & 91.08                                                    \\ \cline{2-6} 
%                                                                              & PRL                                                 & 99.43                                                    & 98.39                                                    & 91.63                                                    & 89.73                                                    \\ \cline{2-6} 
%                         & SubM                                                 & 99.25                                                    & 99.60                                                    & 94.33                                                    & 93.91                                                    \\ \cline{2-6}                                                     & STL                                                 & 99.31                                                    & 99.61                                                    & 96.38                                                    & 96.05                                                    \\ \cline{2-6} 
%                                                                              & SML                                                 & 99.45                                                    & \begin{tabular}[c]{@{}l@{}}99.71\\ (1.32\%)\end{tabular}                                           & 93.98                                                    & 92.83                                                    \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & PRL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
%                                                     & SubM                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
%                                                                             & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.05\\ (44.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \cline{2-4} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.04\\ (55.55\%)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}
% \begin{table}
% \scriptsize
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.06                                                     & 0.01                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.20                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.20                                                     & 0.04                                                     & 0.25                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.17                                                     & 0.02                                                     & 0.16                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.12                                                     & 0.02                                                     & 0.18                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.18                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.11                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.10\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}
% \scriptsize
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:7}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (70.0\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{table}
% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.23                                                     & 0.03                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.16                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.15                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.11                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.10                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.10\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.34                                                     & 0.03                                                     & 0.17                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.18                                                     & 0.02                                                     & 0.12                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}


% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.04                                                     & 0.01                                                     & 0.07                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.21                                                     & 0.02                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.18                                                     & 0.03                                                     & 0.14                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.12                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & MCL                                                 & 0.12                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SBML                                                 & 0.08                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & CTL                                                 & 0.08 & 0.01 & 0.09                                                    \\ \cline{2-5} 
%                                                                              & CBML                                                 & \0.08 & 0.01 & 0.08 \\ \hline
% \end{tabular}
% \end{minipage}
% \hspace{2cm}
% \begin{minipage}[b]{0.4\linewidth}

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
                                                                       
%                                                                              & MCL                                                 & 0.30                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SBML                                                 & 0.32                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & CTL                                                 & 0.10 & 0.03                                                     & 0.09 \\ \cline{2-5} 
%                                                                              & CBML                                                 & 0.11 & 0.01 & 0.08  \\ \hline
% \end{tabular}
% \end{minipage}
% \end{table*}


% \begin{table}[]
% \centering
% \scriptsize
% \caption{\textbf{Comparison of data gradation techniques for 100:20 compression ratio on Vehicle Distance and Centerline Distance}}
% \label{tab:vehcen}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{2}{c|}{MAE}                                                                                                   \\ \cline{3-4} 
%                                                                              &                                                     & \begin{tabular}[c]{@{}l@{}}Vehicle\\ Distance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Centerline\\ Distance\end{tabular} \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.03                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & US                                                  & 0.06                                                       & 0.05                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.09                                                       & 0.08                                                          \\ \cline{2-4} 
%                                                                              & PRL                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
%                                                     & SubM                                                 & 0.05                                                       & 0.06                                                          \\ \cline{2-4}
                            
%                                                                             & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.05\\ (44.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \cline{2-4} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.04\\ (55.55\%)\end{tabular}   & \begin{tabular}[c]{@{}l@{}}0.05\\ (37.5\%)\end{tabular}       \\ \hline
% \end{tabular}
% \end{table}
% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip5_US_SLN_SIFT_1.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip15_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip30_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE for relative angle}}
%     \label{fig:bucketmae}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_15p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:7 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turns_30p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_road_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:3 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{table*}
% \noindent\scriptsize
% \begin{minipage}[b]{0.4\linewidth}
%     \centering
%     %\footnotesize
%     \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance}}
%     \begin{tabular}{|c|p{0.2mm}|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.32                                                                         & 94.7                                                                          & 95.54                                                                         & 94.82                                                                         & 0.22                                                                          & 0.12                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 91.94                                                                         & 91.08                                                                         & 94.58                                                                         & 95.02                                                                         & \textbf{3.08}                                                                          & \textbf{3.94}                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 91.26                                                                         & 90.36                                                                         & 93.58                                                                         & 92.60                                                                         & 2.32                                                                          & 2.24                                                                          \\ \hline
% \multirow{3}{*}{SLO}                                          & 100:20                                                                                            & 88.34                                                                         & 86.96                                                                         & 89.94                                                                         & 87.79                                                                         & 1.6                                                                           & 0.83                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 89.7                                                                          & 89.8                                                                          & 91.76                                                                         & 91.4                                                                          & 2.06                                                                          & 1.6                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 87.68                                                                         & 88.54                                                                         & 91.36                                                                         & 90.78                                                                         & \textbf{3.68}                                                                          & \textbf{2.24}                                                                          \\ \hline
% \multirow{3}{*}{SLN}                                          & 100:20                                                                                            & 89.18                                                                         & 88.25                                                                         & 90.52                                                                         & 89.26                                                                         & 1.34                                                                           & \textbf{1.01}                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 88.04                                                                          & 88.5                                                                          & 91.32                                                                         & 89.17                                                                          & \textbf{5.28}                                                                          & 0.67                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 86.4                                                                         & 86.22                                                                         & 88.0                                                                         & 86.71                                                                         & 1.6                                                                          & 0.49                                                                          \\ \hline
                                    
% \end{tabular}
% \label{tab:redl}
% \end{minipage}
% \hspace{4cm}
% \begin{minipage}[b]{0.4\linewidth}
%     %\footnotesize
%     \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
%     \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & 16.67                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & \textbf{22.22}                                 \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.08                     & 0.06                           & \textbf{25.0}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.10                     & 0.09                           & 10.0                                 \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & \textbf{16.67}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.05                     & 0.05                           & 0.0                                 \\ \hline
% \end{tabular}
% %\caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
% \label{tab:veh}
% \end{minipage}
% \end{table*}


% \begin{table*}[]
% \footnotesize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance}}
% \centering
% \begin{tabular}{|c|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.32                                                                         & 94.7                                                                          & 95.54                                                                         & 94.82                                                                         & 0.22                                                                          & 0.12                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 91.94                                                                         & 91.08                                                                         & 94.58                                                                         & 95.02                                                                         & \textbf{3.08}                                                                          & \textbf{3.94}                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 91.26                                                                         & 90.36                                                                         & 93.58                                                                         & 92.60                                                                         & 2.32                                                                          & 2.24                                                                          \\ \hline
% \multirow{3}{*}{SLO}                                          & 100:20                                                                                            & 88.34                                                                         & 86.96                                                                         & 89.94                                                                         & 87.79                                                                         & 1.6                                                                           & 0.83                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 89.7                                                                          & 89.8                                                                          & 91.76                                                                         & 91.4                                                                          & 2.06                                                                          & 1.6                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 87.68                                                                         & 88.54                                                                         & 91.36                                                                         & 90.78                                                                         & \textbf{3.68}                                                                          & \textbf{2.24}                                                                          \\ \hline
% \multirow{3}{*}{SLN}                                          & 100:20                                                                                            & 89.18                                                                         & 88.25                                                                         & 90.52                                                                         & 89.26                                                                         & 1.34                                                                           & \textbf{1.01}                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 88.04                                                                          & 88.5                                                                          & 91.32                                                                         & 89.17                                                                          & \textbf{5.28}                                                                          & 0.67                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 86.4                                                                         & 86.22                                                                         & 88.0                                                                         & 86.71                                                                         & 1.6                                                                          & 0.49                                                                          \\ \hline
                                    
% \end{tabular}
% \label{tab:redl}
% \end{table*}


% \begin{table*}[]
% %\footnotesize
% \scriptsize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Relative Angle affordance}}
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{3}{c|}{CAL}                                                                                                                                                         & \multicolumn{3}{c|}{Timestamp}                                                                                                                                                   & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{3-11} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.39                                                    & 0.03                                                        & 0.09                                                     & 0.28                                                    & 0.03                                                        & 0.07                                                     & 28.21                                                    & 0.0                                                         & 22.22                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.38                                                    & 0.04                                                        & 0.11                                                     & 0.27                                                    & 0.04                                                        & 0.09                                                     & \textbf{28.94}                                                    & 0.0                                                         & 18.18                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.44                                                    & 0.06                                                        & 0.15                                                     & 0.32                                                    & 0.05                                                        & 0.09                                                     & 27.27                                                    & \textbf{16.66}                                                         & \textbf{40.0}                                                      \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                                                            & 0.19                                                    & 0.07                                                        & 0.08                                                     & 0.17                                                    & 0.04                                                        & 0.08                                                     & 10.52                                                     & \textbf{3.0}                                                         & 15.38                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.19                                                    & 0.05                                                        & 0.13                                                     & 0.20                                                    & 0.05                                                        & 0.11                                                     & -5.0                                                    & 0.0                                                         & 15.38                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.16                                                     & 0.23                                                    & 0.05                                                        & 0.11                                                     & \textbf{11.53}                                                     & 0.0                                                        & \textbf{31.25}                                                      \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                                                            & 0.18                                                    & 0.05                                                        & 0.07                                                     & 0.16                                                    & 0.05                                                        & 0.07                                                     & 11.11                                                     & 0.0                                                         & 0.0                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.21                                                    & 0.07                                                        & 0.06                                                     & 0.20                                                    & 0.07                                                        & 0.05                                                     & 4.76                                                    & 0.0                                                         & 16.66                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.16                                                     &    0.22                                                 & 0.05                                                        & 0.05                                                     & \textbf{15.38}                                                     & 0.0                                                        & \textbf{68.75}                                                      \\ \hline
% \end{tabular}
% \label{tab:relative}
% \end{table*}

% \begin{table}[]
% \footnotesize
% \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance}}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & 16.67                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & \textbf{22.22}                                 \\ \hline
% \multirow{3}{*}{SLO}                                            & 100:20                                                  & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.08                     & 0.06                           & \textbf{25.0}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.10                     & 0.09                           & 10.0                                 \\ \hline
% \multirow{3}{*}{SLN}                                            & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.06                     & 0.05                           & \textbf{16.67}                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.05                     & 0.05                           & 0.0                                 \\ \hline
% \end{tabular}
% \label{tab:veh}
% \end{table}

% \begin{table}[]
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \begin{tabular}{|p{7mm}|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods                                                & MAE  & \%Improvement & MAE            & \% Improvement          \\ \hline
% \multicolumn{4}{|c|}{Vehicle Distance}                                                                                                      & \multicolumn{2}{c|}{Centerline Distance} \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &               & 0.09           &                         \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.05 &               & 0.09           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.06 & 16.67         & 0.09           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.05 & 0.0           & 0.08           & 11.11                   \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.04 & 20.0          & 0.07           & 22.22                   \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &               & 0.11           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.07 & -14.28        & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.08 & -25.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.06 & 0.0           & 0.11           & 0.0                     \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               & 0.11           &                         \\ \cline{2-6} 
%                                                             & SIFT                                                   & 0.10 & -10.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLO                                                    & 0.10 & -10.0         & 0.11           & 0.0                     \\ \cline{2-6} 
%                                                             & SLN                                                    & 0.05 & 44.44         & 0.12           & -8.3                    \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% %\captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance and Centerline Distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods                                                & MAE  & \%Improvement \\ \hline
% \multicolumn{4}{|c|}{Vehicle Distance}                                                                                                      \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &               \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.05 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.06 & 16.67         \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.05 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.04 & 20.0          \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.07 & -14.28        \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.08 & -25.0         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.06 & 0.0           \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.10 & -10.0         \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.10 & -10.0         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.05 & 44.44         \\ \hline
% \multicolumn{4}{|c|}{Centerline Distance}                                                                                                   \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.09 &               \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.09 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.08 & 11.11         \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.07 & 22.22         \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.11 & 0.0           \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &               \\ \cline{2-4} 
%                                                             & SIFT                                                   & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLO                                                    & 0.11 & 0.0           \\ \cline{2-4} 
%                                                             & SLN                                                    & 0.12 & -8.3          \\ \hline
% \end{tabular}
% \end{table}



% \begin{table}[]
% %\captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Vehicle Distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \centering
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  & \% Improvement \\ \hline
%                                                             & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.02 &                \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}                                   & 0.05 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.06 & 16.67               \\ \cline{2-4} 
%                                                             & SLO  & 0.05 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.04 & \textbf{20.0}               \\ \hline
% \multirow{4}{*}{100:7}                                      &\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.06 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.07 & -14.28               \\ \cline{2-4} 
%                                                             & SLO  & 0.08 & -25.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.06 & 0.0               \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.10 & -10.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.10 & -10.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.05     & \textbf{44.44}               \\ \hline
% \end{tabular}
% \label{tab:vehaff}
% \end{table}

% \begin{table}[]
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Centerline Distance} \tr{combine this with vehicle distance}}
% \begin{tabular}{|l|l|l|l|}
% \hline
% \centering
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  & \% Improvement \\ \hline
%                                                             & Whole Set    & 0.09 &                \\ \hline
% \multirow{4}{*}{100:20}                                     & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.09 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.09 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.08 & 11.11               \\ \cline{2-4} 
%                                                             & SLN  & 0.07 & \textbf{22.22}               \\ \hline
% \multirow{4}{*}{100:7}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.11 & 0.0               \\ \hline
% \multirow{4}{*}{100:3}                                      & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.11 &                \\ \cline{2-4} 
%                                                             & SIFT         & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLO  & 0.11 & 0.0               \\ \cline{2-4} 
%                                                             & SLN  & 0.12     & -8.3               \\ \hline
% \end{tabular}
% \label{tab:centaff}
% \end{table}
\begin{figure}[h!]
    %\captionsetup{justification=centering}
     \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_left_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_left_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_straight_15.pdf}
    %\caption{Relative Angle Affordance Distribution}
    \label{fig:tskip15}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_straight_plot_15.pdf}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    
    
    
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/frac_right_15.pdf}
    %\caption{Red light Affordance Distribution}
    \caption{}
    \label{fig:tskip5}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth,height=3cm]{figures/mae_right_plot_15.pdf}
    \caption{}
    %\caption{Red light Affordance Distribution}
    \label{fig:tskip5}
    \end{subfigure}
    \caption{\textbf{(a) Fraction of selected instances and (b) Mean Absolute Error (MAE) for Relative Angle affordance for all subset selection methods. Selection of more fraction of instances in turn buckets lead to lower MAE in CBML for 100:20 compression ratio.}}
    \label{fig:fracmae_100_20}
\end{figure}

% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_left_100_7_15.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/mae_left_100_7_plot_15.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_straight_100_7_15.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/mae_straight_100_7_plot_15.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
    
    
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/frac_right_100_7_15.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/mae_right_100_7_plot_15.pdf}
%     \caption{}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \caption{\textbf{(a) Fraction of selected instances and (b) Mean Absolute Error (MAE) for Relative Angle affordance for two baselines (MCL and SBML) and the proposed methods. Selection of more fraction of instances in turns lead to lower MAE in CBML for 100:7 compression ratio.}}
%     \label{fig:fracmae_100_7}
% \end{figure}
In this section, we will study the performance of different subset selection methods on the basis of their performance in affordance predictions.

We show in tables \ref{tab:redrhazaff}, \ref{tab:vehcen} the performance of Conditional Affordance Learning (CAL) \cite{sauer2018conditional} driving model for four affordances, on subsets obtained by different subset selection techniques for 100:20 compression ratio. 
% We report the best improvement of our proposed methods (STL,SML) for each affordance over the baselines (Uniform Skip (US), Only SIFT, Only Loss, PRL, SubM).
We notice in Table \ref{tab:redrhazaff} that all the methods are able to classify the affordances reasonably well. This is due to weighted cross-entropy losses used for the large number of imbalanced classes as seen initially in Figure \ref{fig:distrib}. From Table \ref{tab:vehcen}, we can see that CTL and CBML outpeform all other methods in predicting vehicle distance affordance. In case of centerline distance, all the methods work similarly with OS and OL performing the worst.

% We notice in table \ref{tab:redlaff} that the \textit{Red Light} accuracies are more for Uniform Skip than all other subset selection methods. Figure \ref{fig:distribhist} (\textit{left)} is a clear indication of the above statement, where we see that the distribution of Uniform Skip for Red Light is higher than all the other gradation methods. It is evident that Uniform Skip method, due to its inherent nature of selection, selects more number of \textit{Red Light True} instances. For example, if the agent vehicle is stuck in traffic, the Uniform Skip method will tend to choose frames uniformly leading to higher selection of true red light instances. However, in case of SLN, since the SIFT dissimilarity and multi-task loss values dominate the selection procedure, it selects the appropriate instances based on them. Since it tries to keep the compression ratio intact while trying to avoid repetitive instances, it tends to drop more frames with \textit{Red Light true} instances leading to a lower accuracy. However, this affordance is not directly related to the episode completion objective.

% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.28                                                                     & 0.02                                                                         & 0.10                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & Only SIFT                                                   & 0.23                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & Only Loss                                                   & 0.16                                                                     & 0.02                                                                         & 0.10                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & PRL                                            & 0.15                                                                     & 0.02                                                                         & 0.10                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLT                                            & 0.11                                                                     & 0.02                                                                         & 0.10                                                                      & 60.71                                                        & 33.33                                                            & 0.0
%                         \\ \cline{2-8} 
%                         & SLM                                            & 0.10                                                                     & 0.02                                                                         & 0.09                                                                      & 64.28                                                        & 33.33                                                            & 10.0
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.46                                                                     & 0.03                                                                         & 0.20                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.51                                                                     & 0.03                                                                         & 0.18                                                                      &                                                         &                                                             &                                                         \\ \cline{2-8} 
% %                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff}
% \end{table*}


% \begin{table}[]
% \centering
% \scriptsize

% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:20 compression ratio}}
% \label{tab:relaff}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                      \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                              \\ \hline
% \multirow{7}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                    \\ \cline{2-5} 
%                                                                              & US                                                  & 0.28                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.23                                                     & 0.03                                                     & 0.09                                                    \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.16                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.15                                                     & 0.02                                                     & 0.10                                                    \\ \cline{2-5}
%                                                     & SubM                                                 & 0.12                                                     & 0.02                                                     & 0.11                                                    \\ \cline{2-5}                         
                                                    
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.11\\ (60.71\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & 0.10                                                    \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.10\\ (64.28\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (10.0\%)\end{tabular} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \centering
% \scriptsize
% % \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance for 100:7 compression ratio}}
% \label{tab:relaff_100_7}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular}} & \multirow{2}{*}{Methods}                            & \multicolumn{3}{c|}{MAE}                                                                                                                                                       \\ \cline{3-5} 
%                                                                              &                                                     & Left Turn                                                & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\end{tabular}  & Right Turn                                               \\ \hline
% \multirow{6}{*}{100:20}                                                      & WS                                                  & 0.05                                                     & 0.01                                                     & 0.06                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ SIFT\end{tabular} & 0.34                                                     & 0.03                                                     & 0.17                                                     \\ \cline{2-5} 
%                                                                              & \begin{tabular}[c]{@{}l@{}}Only\\ Loss\end{tabular} & 0.18                                                     & 0.02                                                     & 0.12                                                     \\ \cline{2-5} 
%                                                                              & PRL                                                 & 0.38                                                     & 0.03                                                     & 0.18                                                     \\ \cline{2-5} 
%                                                             & SubM                                                 & 0.40                                                     & 0.03                                                     & 0.19                                                     \\ \cline{2-5}
%                                                                              & STL                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & 0.03                                                     & \begin{tabular}[c]{@{}l@{}}0.10\\ (41.17\%)\end{tabular} \\ \cline{2-5} 
%                                                                              & SML                                                 & \begin{tabular}[c]{@{}l@{}}0.12\\ (68.42\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.02\\ (33.33\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}0.09\\ (50.0\%)\end{tabular}  \\ \hline
% \end{tabular}
% \end{table}



% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     \centering
%     \includegraphics[height=3cm]{figures/preds_allmeth_100_20.png}
%     \caption{\textbf{Bucket-wise MAE of relative angle for 100:20 compression ratio}}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
% \end{figure}

% \begin{table*}[h!]
% %\footnotesize
% \scriptsize
% \centering
% \captionsetup{justification=centering}
% \caption{\textbf{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}}
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Ratio}  & \multirow{2}{*}{Methods}                               & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{6-8} 
%                         &                                                        &                                                                          &                                                                              &                                                                           & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
%                         & \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 0.05                                                                     & 0.01                                                                         & 0.06                                                                      &                                                         &                                                             &                                                          \\ \hline
% \multirow{4}{*}{100:20} & \begin{tabular}[c]{@{}l@{}}Only SIFT\end{tabular} & 0.34                                                                     & 0.03                                                                         & 0.17                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & Only Loss                                                   & 0.18                                                                     & 0.02                                                                         & 0.12                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & PRL                                                   & 0.38                                                                     & 0.03                                                                         & 0.18                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8}
%                         & SLT                                            & 0.12                                                                     & 0.03                                                                         & 0.10                                                                       &                                                         &                                                             &                                                          \\ \cline{2-8} 
%                         & SLM                                            & 0.12                                                                     & 0.02                                                                         &    0.09                                                                   &                                                         &                                                             &
%                         \\ \hline
% % \multirow{4}{*}{100:7}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.21                                                                     & 0.03                                                                         & 0.08                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.34                                                                     & 0.03                                                                         & 0.11                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.46                                                                     & 0.03                                                                         & 0.20                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLN                                            & 0.11                                                                     & 0.02                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \hline
% % \multirow{4}{*}{100:3}  & \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 0.22                                                                     & 0.03                                                                         & 0.09                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SIFT                                                   & 0.51                                                                     & 0.03                                                                         & 0.16                                                                      &                                                         &                                                             &                                                          \\ \cline{2-8} 
% %                         & SLO                                            & 0.51                                                                     & 0.03                                                                         & 0.18                                                                      &                                                         &                                                             &                                                         \\ \cline{2-8} 
% %                         & SLN                                            & 0.18                                                                     & 0.02                                                                        & 0.09                                                                     &                                                         &                                                                                                                     \\ \hline
% \end{tabular}
% \label{tab:relaff_100_7}
% \end{table*}
 
In case of \textit{Relative Angle} affordance, we have grouped the values into three different buckets meant for Left Turn, Straight Road, Right Turn. We observe in Figure \ref{fig:fracmae_100_20} that our proposed method achieves the lowest MAE for turns in comparison to other subset selection methods. We can also observe in Figure \ref{fig:fracmae_100_20}a that CBML selects more fraction of instances for both Left and Right turns while relaxes comparatively in the Straight Road buckets. SBML also has close fraction of instances to our method for left turn in Figure \ref{fig:fracmae_100_20}a, however it drops down in the fraction of right turns.
% This is a result of selection of instances using both the pairwise and weighted multi-task pointwise metric as we discussed in Section \ref{sec:subset}.

Figure \ref{fig:fracmae_100_20}b portrays the effective nature of our subset selection methods (CTL, CBML) over the other baselines in terms of Mean Absolute Error. We observe that the MAE for straight road buckets for all selection methods are very low in range. This is essentially due to the skewness in Relative Angle affordance. On the other hand, both CTL and CBML outperform all other methods in the turn buckets which have in usual, lesser number of datapoints. The difference in MAE becomes more evident with increase in compression ratio. It is indicative of the fact that our proposed method gives more importance to the frames which are non-redundant (during turns especially) and also having higher losses, thus leading to the lower MAE values in extreme buckets. Thus, we can clearly see that our proposed methods CTL and CBML are performing better quantitatively in terms of affordance predictions and qualitatively in terms of deployment of the trained model in simulator and measuring the episode completion rate.


% \begin{figure}[h!]
%     \centering
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{AISTATS2021PaperPack/figures/mae_bucket_100_20.pdf}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.45\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{AISTATS2021PaperPack/figures/mae_bucket_100_7.pdf}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE of relative angle for 100:20 and 100:7 compression ratio}}
%     \label{fig:maebuck}
% \end{figure}


% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/leftbucket_allmeth.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/straightbucket_allmeth.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/rightbucket_allmeth.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Fraction of selected instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}








% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlysift_sim_fail.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlyloss_sim_fail.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prl_sim_fail.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Buckets in simulator episodes leading to failures for \textit{Only SIFT}(left), \textit{Only Loss}(middle) and \textit{PRL}(right) }}
%     \label{fig:deviate}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
%      \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/sift_sml_stl_13_27.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/onlyloss_sml_stl_48_41.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prl_sml_stl_87_95.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Buckets in simulator episodes leading to failures for \textit{Only SIFT}(left), \textit{Only Loss}(middle) and \textit{PRL}(right) }}
%     \label{fig:deviate}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip5_US_SLN_SIFT_1.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip15_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/skip30_US_SLN_SIFT_1.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Bucket-wise MAE for relative angle}}
%     \label{fig:bucketmae}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_5p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_5p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:20 compression ratio}}
%     \label{fig:bucketprop5}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turn_15p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turn_15p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:7 compression ratio}}
%     \label{fig:bucketprop15}
% \end{figure*}

% \begin{figure*}[h!]
%     %\captionsetup{justification=centering}
    
%     \centering
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_left_turns_30p.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_straight_road_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     %\hspace{25mm}
%     \begin{subfigure}{0.6\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=3cm]{figures/prop_right_turns_30p.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Selected proportion of instances for 100:3 compression ratio}}
%     \label{fig:bucketprop30}
% \end{figure*}
% The same can be observed in table \ref{tab:relaff} where the Straight-Road MAE for all gradation methods have a narrow margin. This happens due to the more number of straight road instances than the turns in our dataset, as depicted in Figure \ref{fig:distrib} (\textit{Right}). However, SLN maintains an overall lower MAE across the buckets, thus proving its selection method efficient.
 
% We also show a similar plot for distribution of predicted affordances in Figure \ref{fig:distribhistpred} where we observe that the predictions also follow similar pattern as the distribution of ground truth affordances in Figure \ref{fig:distribhist}.


% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 96.26                                                    & 95.43                                                    \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 95.54                                                    & 94.82                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 91.9                                                     & 90.75                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 89.94                                                    & 87.79                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 90.52                                                    & 89.26                                                    \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 94.58                                                    & 95.02                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 90.1                                                     & 88.58                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 91.76                                                    & 91.4                                                     \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 91.32                                                    & 89.17                                                    \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 93.58                                                    & 92.60                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 91.87                                                    & 89.02                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 91.36                                                    & 90.78                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &                                                          &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Red Light affordance}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 0.15                                                    & 0.02                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.28                                                    & 0.03                                                        & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.16                                                    & 0.05                                                        & 0.14                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.17                                                    & 0.04                                                        & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.16                                                    & 0.05                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.27                                                    & 0.04                                                        & 0.09                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.17                                                    & 0.05                                                        & 0.16                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.21                                                    & 0.05                                                        & 0.11                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.19                                                    & 0.08                                                        & 0.06                                                     \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.32                                                    & 0.05                                                        & 0.09                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.28                                                    & 0.05                                                        & 0.14                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.23                                                    & 0.06                                                        & 0.11                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &                                                         &                                                             &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}
% \label{tab:relaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  \\ \hline
% \-\-                                                        & Whole Set    & 0.02 \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.04 \\ \cline{2-3} 
%                                                             & SIFT         & 0.04 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.04 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.05 \\ \cline{2-3} 
%                                                             & SIFT         & 0.07 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.06 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.07 \\ \cline{2-3} 
%                                                             & SIFT         & 0.09 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.09 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  &      \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Vehicle Distance affordance}
% \label{tab:vehaff}
% \end{table}




% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Micro\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Accuracy\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 95.86                                                    & 95.16                                                    \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 95.32 (-6.32)                                                   & 94.7 (-6.45)                                                   \\ \cline{2-4} 
%                                                             & SIFT         & 91.36 (-2.18)                                                    & 88.12 (0.13)                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 88.34 (0.84)                                                   & 86.96 (1.29)                                                   \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  & 89.18                                                   & 88.25                                                    \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 91.94 (-3.93)                                                   & 91.08 (-2.58)                                                   \\ \cline{2-4} 
%                                                             & SIFT         & 90.28 (-2.24)                                                    & 90.1 (-1.6)                                                   \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 89.7 (-1.66)                                                   & 89.8 (-1.3)                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &    88.04                                                 & 88.5                                                    \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 91.26                                                    & 90.36                                                    \\ \cline{2-4} 
%                                                             & SIFT         & 90.04                                                    & 90.34                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-O  & 87.68                                                    & 88.54                                                    \\ \cline{2-4} 
%                                                             & SIFT+Loss-N  &                                                          &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Red Light affordance}
% \label{tab:redlaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \-\-                                                        & Whole Set    & 0.15                                                    & 0.02                                                        & 0.08                                                     \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.39 (0.21)                                                   & 0.03 (-0.02)                                                       & 0.09 (0.02)                                                    \\ \cline{2-5} 
%                                                             & SIFT         & 0.17 (-0.01)                                                   & 0.06 (-0.01)                                                       & 0.09 (0.01)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.19 (0.01)                                                   & 0.07                                                       & 0.08                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  & 0.18                                                    & 0.05                                                        & 0.07                                                     \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.38 (0.18)                                                   & 0.04 (-0.03)                                                       & 0.11 (0.05)                                                    \\ \cline{2-5} 
%                                                             & SIFT         & 0.18 (-0.02)                                                   & 0.06 (-0.01)                                                       & 0.14 (0.08)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.19 (0.01)                                                   & 0.05 (-0.02)                                                       & 0.13 (0.07)                                                    \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &    0.20                                                 & 0.07                                                        & 0.06                                                     \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.44                                                    & 0.06                                                        & 0.15                                                     \\ \cline{2-5} 
%                                                             & SIFT         & 0.32                                                    & 0.06                                                        & 0.15                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-O  & 0.26                                                    & 0.05                                                        & 0.16                                                     \\ \cline{2-5} 
%                                                             & SIFT+Loss-N  &                                                         &                                                             &                                                          \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Relative Angle affordance}
% \label{tab:relaff}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|}
% \hline
% \begin{tabular}[c]{@{}l@{}}Compression\\ Ratio\end{tabular} & Methods      & MAE  \\ \hline
% \-\-                                                        & Whole Set    & 0.02 \\ \hline
% \multirow{4}{*}{100:20}                                     & Uniform Skip & 0.05 (0.01) \\ \cline{2-3} 
%                                                             & SIFT         & 0.06 (0.02) \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.05 (0.01) \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.04 \\ \hline
% \multirow{4}{*}{100:7}                                      & Uniform Skip & 0.06 (0.0) \\ \cline{2-3} 
%                                                             & SIFT         & 0.07 (0.01)\\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.08 (0.02) \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  & 0.06 \\ \hline
% \multirow{4}{*}{100:3}                                      & Uniform Skip & 0.09 \\ \cline{2-3} 
%                                                             & SIFT         & 0.10 \\ \cline{2-3} 
%                                                             & SIFT+Loss-O  & 0.10 \\ \cline{2-3} 
%                                                             & SIFT+Loss-N  &      \\ \hline
% \end{tabular}
% \caption{Comparison of data gradation techniques for different compression ratios on Vehicle Distance affordance}
% \label{tab:vehaff}
% \end{table}


% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 95.54                                                                         & 94.82                                                                         & 0.28                                                                         & 0.03                                                                             & 0.07                                                                          & 0.04                                  \\ \hline
% SIFT                                                   & 91.9                                                                          & 90.75                                                                         & 0.16                                                                         & 0.05                                                                             & 0.14                                                                          & 0.04                                      \\ \hline
% SIFT+Loss-O                                            & 89.94                                                                         & 87.79                                                                         & 0.17                                                                         & 0.04                                                                             & 0.08                                                                          & 0.04                                      \\ \hline
% SIFT+Loss-N                                            & 90.52                                                                         & 89.26                                                                         & 0.16                                                                         & 0.05                                                                             & 0.08                                                                          & 0.04                                      \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:20}
% \label{tab:grade_20}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 94.58                                                                         & 95.02                                                                         & 0.27                                                                         & 0.04                                                                             & 0.09                                                                          & 0.05                                  \\ \hline
% SIFT                                                   & 90.1                                                                          & 88.58                                                                         & 0.17                                                                         & 0.05                                                                             & 0.16                                                                          & 0.07                                      \\ \hline
% SIFT+Loss-O                                            & 91.76                                                                         & 91.4                                                                         & 0.21                                                                         & 0.05                                                                             & 0.11                                                                          & 0.06                                      \\ \hline
% SIFT+Loss-N                                            & 91.32                                                                         & 89.17                                                                         & 0.19                                                                         & 0.08                                                                             & 0.06                                                                          & 0.04                                      \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:7}
% \label{tab_grade_7}
% \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{3}{*}{Methods}}         & \multicolumn{6}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Red Light}                                                                                                                                & \multicolumn{3}{c|}{Relative Angle}                                                                                                                                                                                                             & \multicolumn{1}{c|}{Vehicle Distance} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Left-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Straight Road\\ MAE\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Right-Turn\\ MAE\end{tabular}} & \multicolumn{1}{c|}{MAE}              \\ \hline
% \begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}    & 96.26                                                                         & 95.43                                                                         & 0.15                                                                         & 0.02                                                                             & 0.08                                                                          & 0.02                                  \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 93.58                                                                         & 92.60                                                                         & 0.32                                                                         & 0.05                                                                             & 0.09                                                                          & 0.07                                   \\ \hline
% SIFT                                                   & 91.87                                                                          & 89.02                                                                         & 0.28                                                                         & 0.05                                                                             & 0.14                                                                          & 0.09                                      \\ \hline
% SIFT+Loss-O                                            & 91.36                                                                         & 90.78                                                                         & 0.23                                                                         & 0.07                                                                             & 0.11                                                                          & 0.09                                       \\ \hline
% SIFT+Loss-N                                            &                                                                          &                                                                          &                                                                          &                                                                              &                                                                           &                                       \\ \hline
% \end{tabular}
% \caption{Comparison of different data gradation methods for compression ratio 100:3}
% \label{tab:grade_3}
% \end{table*}

% Considering the first type of observation for each compression ratio (or table), we notice that the Timestamp model shows an improved performance for each affordance in comparison. This is because the CAL model takes continuous frames into consideration, while in the Timestamp model, we have integrated the normalised timestamp difference between the subsequent frames. This leads to the better performance in Timestamp model, for all the data gradation methods where both uniformly and non-uniformly skipped frames are present.

% Following the second type of observation for each data gradation method under the same model (CAL or Timestamp), we notice that the \textit{Red Light} accuracies are more for Uniform Skip than all other subset selection methods. The reason becomes evident from Figure \ref{fig:distribhist} (\textit{top left)} where we see that the Uniform Skip method, due to its inherent nature of selection, selects more number of \textit{Red Light True} instances compared to the other methods. In case of \textit{Relative Angle} affordance, we have grouped the corresponding values into three different bins meant for Left Turn, Straight Road, Right Turn. We can observe from Figure \ref{fig:distribhist} (\textit{top right}) that SIFT+Loss-N (SLN) selects more number of instances belonging to the turn category. This is a result of selection of instances using the pointwise metric as we discussed in Section \ref{improved}. Even SIFT and SIFT+Loss-O perform close to SIFT+Loss-N in the selection method due to their selection mechanisms. The similar distribution in the values of Uniform Skip and Whole Set is trivial.

% We observe that even though the Uniform Skip method has similar distribution to that of WS, it is not what should ideally be for a decreased set of instances. This is because the reduced subset unless has enough instances of turns, the driving model would not be able to predict its next waypoint. SIFT and Sift+Loss-O have more instances of left turn instances than Uniform Skip. However, SIFT+Loss-N has a significantly higher number of instances for both the turns. Taking this into consideration, we observe from each table, that under each model (CAL or Timestamp), the gradation methods SIFT, SIFT+Loss-O and SIFT+Loss-N perform significantly better under turns than the Uniform Skip model.

% We show a bucketwise plot of relative angle for different compression ratios in Figure \ref{fig:bucketmae}, which portrays the effective nature of the gradation methods over Uniform Skip. The buckets corresponding to (-0.1 - 0.1) refer to the straight road instances, and the buckets to its left are meant for left turns while to its right, for right turns. We observe that the MAE for straight road buckets for all gradation methods are very low and close to one another. This happens due to the more number of straight road instances than the turns, as depicted in Figure \ref{fig:distrib} (\textit{Right}). Owing to the selection of large number of straight road instances in Uniform Skip selection, the MAE for straight road is lesser compared to the other selection methods. However, predicting its next waypoint on straight road is an easier task compared to turns, which we will observe in the next subsection.

% Lastly, with increasing degree of compression ratio, the performance of the gradation methods shifts away from that of the Whole Set, which is trivial. However, we observe that the difference between the performance of CAL and Timestamp model for each gradation method, becomes more vivid with increasing compression ratio. 



% We observe that the accuracies of the discrete affordance (Red Light) of the models trained using subsets are different by a comparatively wider margin, whereas that of the continuous affordances (Relative Angle and Centerline Distance) differ by a narrow margin. Uniform skip even though performs the best among all subsets in terms of red light affordance accuracy, it fails in selecting images necessary to be present during the turns.
% We show in Figure \ref{fig:distribhist} the distribution of two of the affordances (\textit{Red Light} and \textit{Relative Angle}) in all the selection methods for the compression ratio 100:20. We observe that distribution of both the affordances for Uniform Skip (US) is similar to that of the Whole Set (WS), which is trivial. However, the distribution differs for the other selection methods. In case of red light, SLN (Sift+Loss-N) selects comparatively more number of \textit{Red Light True} instances than the other two methods, namely SIFT and SLO (Sift + Loss-O), but lesser than that of US (Uniform Skip). This leads to the decrease in Red Light accuracy for the selection methods. The reason behind the decrease in selection of \textit{Red Light True} instances is that since the frames captured while in traffic are redundant, the selection methods try to skip the frames. \\
% The figure to the right showing the distribution of affordances for relative angle, we observe that even though the US method has similar distribution to that of WS, it is not what should ideally be for a decreased set of instances. This is because the reduced subset unless has enough instances of turns, the training model would not be able to predict its next waypoint. SIFT and SLO have more instances of left turn instances than US. However, SLN has a significantly higher number of instances for both the turns. The average MAE for SLN is slightly higher than that of US or SIFT. This is because the more number of test instances are concentrated towards the \textit{Straight} task, which has lesser number of selected frames due to redundancy. We show a bucketwise plot of relative angle which portrays the effective nature of SLN.
%\textcolor{red}{More explanation}
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth,height=3.5cm]{figures/redlight.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:distribhist}
% \end{figure}



% \begin{figure}[h!]
%     %\captionsetup{justification=centering}
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_pred5.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_pred5.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_pred15.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relturns_pred15.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
    
%      \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redlight_30.eps}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:tskip5}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/relative_30.eps}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:tskip15}
%     \end{subfigure}
%     \caption{\textbf{Comparison of distribution of predicted affordances among the selection methods for (\textit{top}) 100:20 , (\textit{middle}) 100:7 , (\textit{bottom}) 100:3 compression ratio: WS : Whole Set; US : Uniform Skip; SLO : SIFT+Loss-O; SLN : SIFT+Loss-N}}
%     \label{fig:distribhistpred}
% \end{figure}
% \begin{figure}[h!]
%     %\centering
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/redl.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:relhist}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/turns.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:turnhist}
%     \end{subfigure}
    
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/haz.png}
%     %\caption{Red light Affordance Distribution}
%     \label{fig:relhist}
%     \end{subfigure}
%     \begin{subfigure}{0.48\columnwidth}
%     \centering
%     \includegraphics[width=\textwidth,height=2.5cm]{figures/speed.png}
%     %\caption{Relative Angle Affordance Distribution}
%     \label{fig:turnhist}
%     \end{subfigure}
%     \captionsetup{justification=centering}
%     \caption{Comparison of distribution of affordances among the selection methods for 100:20 compression ratio: WS : Whole Set; US : Uniform Skip; SLO : SIFT+Loss-O; SLN : SIFT+Loss-N}
%     \label{fig:distribhist}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth,height=4cm]{figures/test_turns_skip5.png}
%     \caption{Bucket-wise MAE for relative angle}
%     \label{fig:turnskip5}
% \end{figure}









% \begin{table*}[]
% %\centering
% \begin{tabular}{|l|p{7mm}|l|l|l|l|l|l|l|l|l|}
% \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Gradation\end{tabular}} & \multirow{3}{*}{Ratio}  & \multirow{3}{*}{Poses} & \multicolumn{8}{c|}{Tasks}                                                                                                                                                                                                                                                    \\ \cline{4-11} 
%                                                                           &                         &                        & \multicolumn{2}{l|}{Straight} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}One\\ Turn\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Straight\\ Dynamic\end{tabular}} & \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}One\\ Turn\\Dynamic\end{tabular}} \\ \cline{4-11} 
%                                                                           &                         &                        & CAL            & TS           & CAL                                 & TS                                & CAL                                     & TS                                    & CAL                                      & TS                                     \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Whole\\ Set\end{tabular}}      & \multirow{2}{*}{}       & Train                  & 10             &              & 9                                   &                                   & 10                                      &                                       & 8                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 7                                   &                                   & 10                                      &                                       & 7                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:20} & Train                  & 9              &              & 0                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 1                                   &                                   & 9                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  & 10             &              & 2                                   &                                   & 10                                      &                                       & 2                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 1                                   &                                   & 9                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  & 10             &              & 3                                    &                                   & 8                                       &                                       & 2                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 2                                    &                                   & 9                                       &                                       & 1                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  & 10             &              & 6                                   &                                   & 10                                      &                                       & 6                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 3                                   &                                   & 10                                      &                                       & 3                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:7} & Train                  & 9              &              & 0                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 0                                   &                                   & 7                                       &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  & 9             &              & 2                                   &                                   & 9                                      &                                       & 1                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 8             &              & 1                                   &                                   & 8                                       &                                       & 1                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  &              &              & 2                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  & 10             &              & 3                                   &                                   & 10                                      &                                       & 3                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 10             &              & 2                                   &                                   & 10                                      &                                       & 2                                        &                                        \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}}   & \multirow{8}{*}{100:3} & Train                  & 9              &              & 1                                   &                                   & 8                                       &                                       & 0                                       &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   & 9              &              & 1                                   &                                   & 8                                       &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{SIFT}                                                     &                         & Train                  &              &              & 1                                   &                                   &                                       &                                       & 0                                        &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                   &                                   &                                        &                                       & 0                                        &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular}}   &                         & Train                  &              &              & 1                                    &                                   &                                        &                                       & 1                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              & 1                                    &                                   &                                        &                                       & 0                                         &                                        \\ \cline{1-1} \cline{3-11} 
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-N\end{tabular}}   &                         & Train                  &              &              &                                    &                                   &                                       &                                       &                                         &                                        \\ \cline{3-11} 
%                                                                           &                         & Test                   &              &              &                                    &                                   &                                       &                                       &                                         &                                        \\ \hline
% \end{tabular}
% \captionsetup{justification=centering}
% \caption{Comparison of data gradation techniques in terms of episode completion \tr{Will reorder the structure}}
% \label{eptable}
% \end{table*}




% \subsection{CAL vs Timestamp model}
% \label{tsvscal}

% Having motivated the Timestamp model in Section \ref{sec:CAL-TS}, we show here the effectiveness of Timestamp model in the light of prediction of the following affordances - \textit{Red Light} ,\textit{Vehicle Distance} and \textit{Relative Angle}. We compare in tables \ref{tab:redl},  \ref{tab:veh} and \ref{tab:relative}, CAL and Timestamp Model for the three methods - Uniform Skip, SLO and SLN across 3 compression ratios - \textit{100:20}, \textit{100:7} and \textit{100:3}. We report the micro and macro accuracies for Red Light, direction based bucket-MAE of relative angle , MAE of vehicle distance and \% improvement of Timestamp model over CAL model for every affordance.

% It is observed that Timestamp model shows an improved performance in affordance predictions for all the methods for each affordance in comparison. This is because the CAL model takes continuous frames into consideration in the frame buffer, while the Timestamp model integrates the normalised timestamp difference between the subsequent frames. This leads to the better performance in Timestamp model for the data gradation methods, where both uniformly and non-uniformly skipped frames are present. We have boldfaced the highest improvement for each gradation method under each metric of affordance.

% Besides, we observe in table \ref{tab:relative} that Uniform skip which is an uniformly-skipping-frames method, has a higher MAE for Left turn under CAL model. The reason lies in the number of left turns present in our dataset, shown in Figure \ref{fig:distrib} (\textit{Right}). Owing to its inherent nature, Uniform skip tends to skip frames uniformly, as a result of which it ends up missing a large number of frames belonging to left turn. However, using Timestamp model, the respective Left Turn MAE for Uniform skip is lower due to the inclusion of timestamp information. Hence, we are able to show that inclusion of timestamp information in the perception module of driving model yields a better performance, in the process of making self-driving data efficient.


% \begin{table}[]
% \caption{\textbf{Comparison of CAL and Timestamp Model on Centerline Distance affordance}}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.09                     & 0.07                           & \textbf{22.22}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.10                           & 9.09                                \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.09                     & 0.08                           & \textbf{11.11}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.11                     & 0.11                           & 0.0                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-N}                                            & 100:20                                                                                            & 0.07                     & 0.06                           & \textbf{14.28}                               \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.11                     & 0.11                            & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.12                     & 0.12                           & 0.0                                 \\ \hline
% \end{tabular}
% \label{tab:cenaff}
% \end{table}

% \begin{table*}[]
% \centering
% \begin{tabular}{|c|l|l|l|l|l|l|l|}
% \hline
% \multirow{2}{*}{Methods}                                                & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{2}{c|}{CAL}                                                                                                                                      & \multicolumn{2}{c|}{Timestamp}                                                                                                                                & \multicolumn{2}{c|}{\% Improvement}                                                                                                                           \\ \cline{3-8} 
%                                                                         & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Micro\\ Accuracy\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Macro\\ Accuracy\end{tabular}} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 95.63                                                                         & 94.98                                                                          & 96.22                                                                         & 95.41                                                                         & 0.59                                                                           & 0.43                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 93.53                                                                         & 93.53                                                                         & 95.58                                                                         & 95.15                                                                         &  2.05                                                                         & 1.62                                                                          \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 92.64                                                                         & 92.15                                                                         & 95.29                                                                         & 94.92                                                                         & 2.65                                                                          & 2.77                                                                          \\ \hline
% \multirow{3}{*}{SIFT + Loss-O}                                          & 100:20                                                                                            & 96.83                                                                         & 86.43                                                                         & 97.99                                                                         & 93.25                                                                         & 1.16                                                                           & 6.82                                                                          \\ \cline{2-8} 
%                                                                         & 100:7                                                                                             & 96.74                                                                          & 90.17                                                                          & 97.01                                                                         & 92.32                                                                          & 0.27                                                                          & 2.15                                                                           \\ \cline{2-8} 
%                                                                         & 100:3                                                                                             & 90.53                                                                         & 89.97                                                                         & 97.63                                                                         & 91.69                                                                         & 7.1                                                                          & 1.72                                                                         \\ \hline

% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Red Light affordance using varying spaced frame buffers}}
% \label{tab:redl_data}
% \end{table*}


% \begin{table*}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{3}{c|}{CAL}                                                                                                                                                         & \multicolumn{3}{c|}{Timestamp}                                                                                                                                                   & \multicolumn{3}{c|}{\% Improvement}                                                                                                                                              \\ \cline{3-11} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left-Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight-Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right-Turn\\ MAE\end{tabular} \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.29                                                    & 0.02                                                        & 0.09                                                     & 0.20                                                    & 0.02                                                        & 0.06                                                     & 31.0                                                    & 0.0                                                         & 33.33                                                     \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.36                                                    & 0.03                                                        & 0.15                                                     & 0.37                                                    & 0.03                                                        & 0.11                                                     & -2.7                                                    & 0.0                                                         & 26.67                                                      \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.44                                                    & 0.03                                                        & 0.13                                                     & 0.38                                                    & 0.03                                                        & 0.10                                                    & 13.63                                                    & 0.0                                                         & 23.08                                                      \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.20                                                    & 0.07                                                        & 0.11                                                     & 0.12                                                    & 0.04                                                        & 0.13                                                     & 40.0                                                     & 42.85                                                         & -18.18                                                      \\ \cline{2-11} 
%                                                                         & 100:7                                                                                             & 0.24                                                    & 0.05                                                        & 0.21                                                     & 0.20                                                    & 0.04                                                        & 0.15                                                     & 16.67                                                    &    20.0                                                      & 28.57                                                     \\ \cline{2-11} 
%                                                                         & 100:3                                                                                             & 0.26                                                    & 0.05                                                        & 0.17                                                     & 0.27                                                    & 0.04                                                        & 0.15                                                     & -3.8                                                     & 20.0                                                        & 11.76                                                      \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Relative Angle affordance using varying spaced frame buffers}}
% \label{tab:relative_data}
% \end{table*}

% \begin{table}[]
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                   & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                  & 0.04                     & 0.04                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.05                     & 0.04                           & 20.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   &  0.07                    & 0.05                           & 28.57                                 \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                  & 0.03                     & 0.02                           & 33.33                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                   & 0.07                     & 0.04                           & 42.85                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                   & 0.09                     & 0.07                           & 22.22                                 \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Vehicle Distance affordance using varying spaced frame buffers}}
% \label{tab:veh_data}
% \end{table}

% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Methods}}                          & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Compression\\ Ratio\end{tabular}}} & \multicolumn{1}{c|}{CAL} & \multicolumn{1}{c|}{Timestamp} & \multicolumn{1}{c|}{\% Improvement} \\ \cline{3-5} 
% \multicolumn{1}{|c|}{}                                                  & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE}       & \multicolumn{1}{c|}{MAE}            \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular}} & 100:20                                                                                            & 0.08                     & 0.08                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.07                     & 0.07                           & 0.0                                 \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.12                         & 0.11                               & 8.33                                    \\ \hline
% \multirow{3}{*}{SIFT+Loss-O}                                            & 100:20                                                                                            & 0.15                     & 0.09                           & 40.0                                \\ \cline{2-5} 
%                                                                         & 100:7                                                                                             & 0.15                     & 0.13                           & 13.33                               \\ \cline{2-5} 
%                                                                         & 100:3                                                                                             & 0.17                     & 0.16                           & 5.88                                \\ \hline
% \end{tabular}
% \caption{\textbf{Comparison of CAL and Timestamp Model on Centerline Distance affordance using varying spaced frame buffers}}
% \label{tab:cen_data}
% \end{table}



% \begin{table*}[h!]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 95.32                                               & 94.7                                                & 95.54                                               & 94.82                                               & 0.22                                                    & 0.12                                                    & 0.39                                                      & 0.03                                                          & 0.09                                                       & 0.28                                                      & 0.03                                                          & 0.07                                                       & 11.0                                                    & 0.0         & 2.0                                                      & 0.05 & 0.04                     & 1.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 88.34                                               & 86.96                                               & 89.94                                               & 87.79                                               & 1.6                                                    & 0.83                                                    & 0.19                                                      & 0.07                                                          & 0.08                                                       & 0.17                                                      & 0.04                                                          & 0.08                                                       & 2.0                                                    & 3.0         & 0.0                                                      & 0.05 & 0.04                     & 1.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp (TS) Model for compression ratio 100:20}
% \label{CALvsTS_100_20}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 91.94                                               & 91.08                                                & 94.58                                               & 95.02                                               & 3.08                                                    & 3.94                                                    & 0.38                                                      & 0.04                                                          & 0.11                                                       & 0.27                                                      & 0.04                                                          & 0.09                                                       & 11.0                                                    & 0.0         & 2.0                                                      & 0.06 & 0.05                     & 1.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 89.7                                               & 89.8                                               & 91.76                                               & 91.4                                               & 2.06                                                    & 1.6                                                    & 0.19                                                      & 0.05                                                          & 0.13                                                       & 0.21                                                      & 0.05                                                          & 0.11                                                       & -2.0                                                    & 0.0         & 2.0                                                      & 0.08 & 0.06                     & 2.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp (TS) Model for compression ratio 100:7}
% \label{CALvsTS_100_7}
% \end{table*}


% \begin{table*}[]
% \begin{tabular}{|p{8 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5.2 mm}|p{5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{7.5 mm}|p{5 mm}|p{5 mm}|p{5 mm}|l|}
% \hline
% \multirow{4}{*}{Methods}                               & \multicolumn{18}{c|}{Affordances}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \cline{2-19} 
%                                                       & \multicolumn{6}{c|}{\textbf{Red Light}}                                                                                                                                                                                                                                                                                                    & \multicolumn{9}{c|}{\textbf{Relative Angle}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \multicolumn{3}{c|}{\textbf{Vehicle Distance}}                      \\ \cline{2-19} 
%                                                       & \multicolumn{2}{c|}{CAL}                                                                                  & \multicolumn{2}{c|}{TS}                                                                            & \multicolumn{2}{c|}{\% Improve}                                                                           & \multicolumn{3}{c|}{CAL}                                                                                                                                                               & \multicolumn{3}{c|}{TS}                                                                                                                                                         & \multicolumn{3}{c|}{\% Improve}                                                                                        & CAL  & TS                & \% Improve               \\ \cline{2-19} 
%                                                       & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Micro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Macro\\ Acc\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Straight\\ Road\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Right\\ Turn\\ MAE\end{tabular} & \begin{tabular}[c]{@{}l@{}}Left\\ Turn\end{tabular} & Straight & \begin{tabular}[c]{@{}l@{}}Right \\ Turn\end{tabular} & MAE  & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c|}{MAE} \\ \hline
% \begin{tabular}[c]{@{}l@{}}Uniform\\ Skip\end{tabular} & 91.26                                               & 90.36                                                & 93.58                                               & 92.60                                               & 2.32                                                    & 2.24                                                    & 0.44                                                      & 0.06                                                          & 0.15                                                       & 0.32                                                      & 0.05                                                          & 0.09                                                       & 12.0                                                    & 1.0         & 6.0                                                      & 0.09 & 0.07                     & 2.0                         \\ \hline
% \begin{tabular}[c]{@{}l@{}}SIFT+\\ Loss-O\end{tabular} & 87.68                                               & 88.54                                               & 91.36                                               & 90.78                                               & 3.68                                                    & 2.24                                                    & 0.26                                                      & 0.05                                                          & 0.16                                                       & 0.23                                                      & 0.07                                                          & 0.11                                                       & 3.0                                                    & -2.0         & 5.0                                                      & 0.10 & 0.09                     & 1.0                         \\ \hline
% \end{tabular}
% \caption{Comparison of CAL and Timestamp(TS) Model for compression ratio 100:3}
% \label{CALvsTS_100_3}
% \end{table*}





==> method.tex <==

\newtheorem{remark}{Remark}

In this section, we contextualise the problem of subset selection in the context of autonomous driving. We introduce the underlying framework for online subset selection and illustrate an existing approach and its limitations.


\subsection{Background}
\label{sec:subset}

We introduce the subset selection problem in the context of the application - autonomous driving. The input to the autonomous driving model is a set of episodes, each of which is a sequence of video frames, annotated by corresponding affordances. However, for simplicity, in the context of online frame subset selection, we assume that the episodes have an ordering, and hence the entire data can be thought of as a single dataset $\mathcal{D}$ comprising of video frames $x_i$, and labels $y_i$ corresponding to various learning tasks such as prediction of driving affordances. 
Hence, $\mathcal{D} = \{ (x_i,y_i),\ i=1,\dots,n \}$ where $n$ is the total number of datapoints (annotated video frames) in the dataset. 

Similar to \cite{das2020multi}, we process the data in batches $X_t ,\ t = 1,\dots,T$, where batch size $|X_t| = m$. Hence $mT = n$. We also define the cumulative sets $C_t = \cup_{i=1}^t X_i$. We are interested in constructing representative sets $R_t \subseteq C_t$, such that 
%$R_t$ retains meaningful information from $C_t$ and 
affordance prediction models $M_t$ trained on $R_t$ perform similarly to those trained on $C_t$ and size of $R_t$ is minimized. 
Here, performance is the generalization error, measured as the error on a common test set.

\subsection{Online Subset Selection Formulation}

We define the online subset selection problem primarily defined in \cite{elhamifar2017online} following the above setup. Given a datapoint $i$ from the set $X_{t+1}$ and another datapoint $j$ from the set $R_t$, $R_{t+1}$ is constructed by solving the problem:

\small
\begin{align}
\label{eqn:eq1}
    &\min_{z^o_{ij},z^n_{ij}} & \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij} + \sum_{i,j=1}^m z_{ij}^n d^n_{ij} + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
    &s.t. & \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    & & z_{i,j}^n, z_{i,j}^o \in [0,1]
    \nonumber
\end{align}
\normalsize
where $d^o_{ij}$ denotes the notion of dissimilarity between new frame $i$ (from $X_{t+1}$) and old frame $j$ (from $R_t$), $d^n_{ij}$ denotes the notion of dissimilarity between new frames $i$ and $j$ (from $X_{t+1}$), and $z_{ij}^o, z_{ij}^n $ are relaxed versions of binary assignment variables. $z_{ij}^o=1 $ denotes that the representative of $i^{th}$ new example (from $X_{t+1}$) is $j^{th}$ old example (from $R_t$), and $z_{ij}^n=1$ denotes that representative of $i^{th}$ new example (from $X_{t+1})$ is the $j^{th}$ new example. Note that the indices $i,j$ are internal to sets $R_t$ and $X_{t+1}$ depending on context $o$ (old) or $n$ (new).


\subsection{Multiple Criteria Selection}

We observe that while $d_{ij}$ can be used to encode the perceptual pairwise dissimilarity between video frames $i$ and $j$, the above formulation (Equation \ref{eqn:eq1}) does not incorporate the pointwise attributes of each data point $x_i,y_i$ w.r.t. to the already trained model $M_t$, where $(x_i,y_i)\in X_{t+1}$. Let $L^n_i$ denote the pointwise attribute (here loss value) for datapoint $i$ in $X_{t+1}$ and analogously for $L^o_i$ (denoting loss for datapoint $i$ in $R_t$). \cite{das2020multi} proposes to incorporate it by constructing the $Q$ function as a weighted average of $d$  and $L$ as:

\small
\begin{equation}
Q_{ij} = \rho d_{ij} - (1-\rho) L_j
\label{eq:joint}
\end{equation}
\normalsize

where, $0 \leq \rho \leq 1$ is the weightage given to pairwise criteria.
Hence, their \cite{das2020multi}  final selection problem is:

\small
\begin{align}
\label{eqn:oldsiftloss}
    &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
    &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
\end{align}
\normalsize
Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, a frame $j$ should have the minimum dissimilarity with a new frame $i$ in order to become its representative. Similarly, for pointwise score, a frame $j$ should have a higher loss value to be included as a part of the representative set $R_{t=1}$, so that training it can help generalize better. Using the above intuitions, we further show that for the solution of formulation \ref{eqn:oldsiftloss}, the following conditions must hold.

\begin{theorem}
The score function in Equation \ref{eqn:oldsiftloss} is 
\begin{equation}
\sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p
\end{equation}

A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
\begin{itemize}
% \item $\sum_{i=1}^m Q^n_{ij} < \sum_{i=1}^m Q^n_{ij'}$ where $j \neq j'$
\item For any incoming point i $\in X_{t+1}$ , $Q^n_{ij} < Q^n_{ij'}$ where $j \neq j'$
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
\item $\sum_{i=1}^m Q^n_{ij} < \frac{ \sum_{i=1}^m z_{i,k}^o Q^o_{ik} + \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
\end{itemize}
%where k = $argmin_j \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{i,j}^o Q_{i,j}^o$
where k = $argmin_j \sum_{i=1}^m z_{i,j}^o Q_{i,j}^o$
\end{theorem}

\begin{corollary}
\label{coro1}
For pointwise score ($\rho = 0$), the score function is
\begin{equation}
- \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t)\right]+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p
\end{equation}

A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
\begin{itemize}
% \item $L^n_j$ is the highest among all $j\in X_{t+1}$.
\item $L_j^n > L_{j'}^n$ where $j \neq j'$
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
\item $L^n_j > \frac{ \sum_{i=1}^m z_{i,k}^o L_k^o - \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
\end{itemize}
\end{corollary}
The intuitions are further explained in the Supplementary.

\textbf{Drawbacks of the above formulation}:

However, we notice certain drawbacks in the formulation defined in \cite{das2020multi}. The first drawback of the formulation described in Equation \ref{eqn:oldsiftloss} is that pointwise metric has very limited impact on the set of selected points.
To see this, note that using only pointwise metric yields a maximum of 1 representative for all images belonging to incoming set.
An interesting observation is that when $\rho = 0$, either $0$ or $1$ new representative point is selected from $X_t$. In the context of self-driving, this means that given any incoming frame from a driving scenario, all of them would have the same frame as a representative which would bear the highest loss.
%The following remark notes this when $\rho = 0$.

% Let us illustrate through an example. Suppose $R_t$ and $X_t$ have two frames each.
% $d^o = \begin{bmatrix}
% 1 & 2\\
% 1 & 3
% \end{bmatrix}$ , $d^n = \begin{bmatrix}
% 2 & 1\\
% 1 & 3
% \end{bmatrix}$ , $L^o = \begin{bmatrix}
% 1 & 3
% \end{bmatrix}$ and $L^n = \begin{bmatrix}
% 2 & 1
% \end{bmatrix}$.

When $\rho$ = 0, we have from Equation \ref{eq:joint}, $Q_{ij}^o$ = $- (1-\rho) L_j^o$ and similarly, $Q_{ij}^n$ = $- (1-\rho) L_j^n$. We can see that, $\forall i$ in $R_t$, $Q_{ij}^o$ holds the same values. The same thing holds true $\forall i$ in $X_t$. The representative of any instance $i$ from $X_t$ $(i = 1, ..., m)$ will be the point which either satisfies Corollary \ref{coro1} and belong to $X_{t}$ or has the highest loss among $R_t$. So, all the frames in $X_t$ will be represented by only one frame from $X_t$ or $R_t$. Similarly, with other values of $\rho$ where pointwise metric is given higher weightage, the representatives for some elements $i \in X_t$ are almost similar due to the same reason.

The second drawback is that there is no obvious connection between intended compression ratio, and $\lambda$. Hence, one has to perform grid search over the values of $\lambda$ in order to obtain a particular compression ratio. We thus propose a novel formulation in the next section which can efficiently utilise the pairwise-pointwise criteria for subset selection.

\noteng{SO the entire section is not your contribution, I am not sure why so much space need to be devoted to a work which is not yours - perhaps you may think of recasting}


==> method1.tex <==

In this section, we describe a data-efficient system for training of self-driving vehicle systems from input video data. 
We focus on developing a data efficient system for frame subset selection, which selects the most important video frames for the training of self-driving car models.
% We focus on two main components to such a data efficient system: (1) a system for frame-subset selection, which selects the most important video frames for the training of self-driving car models, and (2) a model for self-driving car which can be trained using a video with irregularly selected frames. 
Our main contribution here is a novel formulation for online selection of subsets of video frames, in the presence of multiple input criteria - both for pairs of input frames and for single input frame. 
% First, we describe an existing state of the art model for self driving cars and propose improvements to the model so that it can perform better with dropped frames (section \ref{sec:CAL-TS}). 
Next, we describe our improved method for online subset selection.
%(section \ref{sec:subset}.

% \subsection{Conditional Affordance Learning with Timestamp}
% \label{sec:CAL-TS}

% % \tr{ Describe the affordances and their connection to self driving like how throttle brake steering angles are calculated. (about 1 paragraph),\\
% % Describe CAL model input, architecture including the framebuffer, and multitask learning aspect (2 - 3 paragraphs),\\}
% %\textbf{Driving Model}: 
% The driving models (or simply models) for self-driving cars take as input a sequence of video frames, and high level driving directions, like \texttt{left, right, straight}; and produce low level driving controls e.g. \textit{steering angle, brake, throttle} as output.
% For this study, we use the CARLA driving simulator \cite{dosovitskiy2017carla} as our testbed, both for collecting training data and for testing out the trained models.
% Also, in this work we built on the popular state of the art driving model - Conditional Affordance Learning model (CAL) \cite{sauer2018conditional}, which is inspired from a chain of works advocating prediction of affordances, starting with \cite{chen2015deepdriving}.

% %which are intermediate level representations of driving intentions  .
% %has divided its framework into two sequential modules: Perception and Controller.


% Affordances are intermediate representations of driving intentions which are easily understood by humans, and the low level representation can be easily computed from them (using non-learned control systems).
% %, which can be obtained from any given frame. These representations are used in the self-driving pipeline to determine the control values for maneuvering the vehicle. 
% Following \cite{sauer2018conditional}, we use six affordances here: (1) 3 discrete - \textit{Red light} , \textit{Speed Sign} and \textit{Hazard Stop} and (2) 3 continuous - \textit{Relative Angle}, \textit{Centerline Distance}, and \textit{Vehicle Distance}. 
% Also, off the above, \textit{relative angle} and \textit{centerline distance} are conditional affordances, as they depend on the high level driving directions: \texttt{left, right, straight}. Finally, all the affordances take a buffer of past frames (input as VGG features) as input, and use a RNN followed by fully-connected layer to predict the affordance values or class probabilities, for continuous and discrete affordances. This module is called the perception module. Figure \ref{fig:timestamp} illustrate this module and also the other components of the testbed: controller and simulator.

% \newcommand{\cD}{\mathcal{D}}
% \newcommand{\bx}{\mathbf{x}}
% \newcommand{\by}{\mathbf{y}}

% Formally, let $\cD = \{ \cD_1,\dots, \cD_M \}$ be a set of $M$ episodes (short videos corresponding to drives of the simulated vehicle, along with captured affordances), and let $\cD_i = \{(\bx_1,\by_1), \dots, (\bx_{N_i},\by_{N_i}) \}$ be the sequence of video frames $\bx_j$, and affordances $\by_j$ for a given episode $\cD_i$. Then the perception module $\mbox{perc}()$ can be described as a prediction model:
% \begin{equation}
% \by_t = \mbox{perc}(\bx_t,\dots,\bx_{t-k+1})
% \end{equation}
% where $k$ is the length of the framebuffer. The implicit assumption here is that the frames $\bx_i$ are sampled at constant intervals. 
% However, in order to make self-driving data efficient, it is necessary to drop some unimportant frames. For example, if the agent vehicle is driving on a straight road, and encountering houses and trees on both its sides at every frame, we may not necessarily store each of the frames. In this scenario, if we intend to drop some frames, the frame buffer will not contain contiguous frames. Hence, the perception module is not receiving consistent inputs in this case.

% Moreover, note that the timestamp information is not even present in the input data, if we drop frames randomly. Hence we provide input for videos with dropped frames as $\cD_i = \{(\bx_1,\by_1,t_1), \dots, (\bx_{N_i},\by_{N_i},t_{N_i}) \}$, where $t_j$ is the timestamp of the corresponding frame. With the modifed input, we define the timestamp features for predicting $\by_j$ as:
% \begin{equation}
% \tilde{\bx}_j(l) = \frac{t_l - t_{j-k+1}}{t_j - t_{j-k+1}} \bx_l,\ \forall l\in\{j-k+1,\dots,j\}
% \end{equation}
% \tr{The key idea here is that entire window of the framebuffer is considered to be of unit time length, and the corresponding features are linearly scaled w.r.t. their temporal distance from the current timestamp (\textit{staleness}), with the oldest image receiving zero weightage.} We note that other ways of capturing the staleness are possible (e.g. passing timestamps as inputs), however we found that this approach yields predictable improvements. This is also similar to how other features, e.g. driving directions are incorporated in the model, instead of passing those features as separate inputs.
% In figure \ref{fig:timestamp}, we have illustrated our proposed Timestamp model. 
% %As we observe, the feature extraction network takes in a sequence of frames and extracts each of its k-dimensional features. 
% The original features $\bx_j$ of the frames are then concatenated with the timestamp weighed features $\tilde{\bx}_j$ and fed into the perception module:
% \begin{equation}
% \by_t = \mbox{perc}((\bx_t,\tilde{\bx}_t)\dots,(\bx_{t-k+1},\tilde{\bx}_{t-k+1}))
% \end{equation}
% %We weigh each component of the features with the difference between the current frame and its previous frame in the frame buffer. In order to normalize the weight, we divide the difference with the range of timestamp value for that corresponding frame buffer. 
% The rest of the model is similar to the CAL driving model.
% % where the predicted affordances are sent to the controller which determine the control values and send it back to the agent vehicle.
% Next we discuss the frame subset selection.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.95\columnwidth]{figures/Timestamp_Model.pdf}
%     %\caption{Red light Affordance Distribution}
%     \caption{Illustration of Timestamp Model}
%     \label{fig:timestamp}
% \end{figure}




%The different task blocks to predict the affordances are designed to take the features of a continuous set of frames. Hence, the deep learning driving model defined in \cite{sauer2018conditional} will be unable to learn the affordances appropriately from the irregularly spaced frame buffer. For e.g., if we drop some frames from the data while the car is at a junction, the CAL driving model might not be able to predict its affordances correctly since it expects consecutive frames in its buffer.

%essential in self-driving task. There are two categories of affordances - discrete and continuous. 
%The discrete affordances comprise of \textit{Red light} , \textit{Speed Sign} and \textit{Hazard Stop}, while the continuous ones are further divided into conditional and unconditional affordances. 

%The conditionality is based on the requirement of the affordance to consider an important factor - \textit{direction} in its computation. \textit{Relative Angle} (angle of the agent vehicle with respect to the road) and \textit{Centerline Distance} are the conditional continuous affordances which consider the direction (straight, left, right) in its prediction, while \textit{Vehicle Distance} is the unconditional continuous affordance. These affordances are used to calculate the control values - \textit{steer} , \textit{throttle} and \textit{brake} which help in deciding the next waypoint of the vehicle. The throttle and brake are dependent on the discrete affordances along with the unconditional continuous affordance. For e.g. , if \textit{Red Light} is True, the throttle is brought down to 0 and brake to a value of 1, or if any vehicle comes in front of the agent vehicle, the throttle value is reduced to a certain extent. Similarly, the steer value is computed using a PID controller considering the conditional continuous affordances.
%It follows a direct perception approach which originates from the psychology of visual perception \cite{gibson1966senses} \cite{gibson2014ecological}. In the context of self driving cars, it refers to mapping a single image to multiple affordance indicators of the situation in road. 
%The perception module takes the frames which arrive from the CARLA \cite{dosovitskiy2017carla} agent as its input. The input images are stacked into a frame buffer of a certain sequence length and are fed into a feature extraction network. The features are provided as input to six different neural networks (task blocks), which are designed to predict the six different affordances (tasks). The loss corresponding to all the six affordances are combined together to form a multi-task training objective function for the perception module.
%The predicted affordances from the perception module are used as input to the controller block. 
%The controllers use the affordances to determine the control values - steer, throttle and brake which is again provided back to the agent vehicle to help it find its next waypoint.

% \tr{Motivate from the above that why CAL is expected to perform poorly when frames are dropped. basically tell that the framebuffer will contain irregularly spaced video frames, and that input is fed to a deep learning model, but the deep learning model does not know the spacing between the frames. Hence it cannot learn the affordances where it is expected to utilize the consecutive frames in order to make a predition. give example.}

%The intuition behind the usage of frame buffer is to simply enhance the memory (of what it has seen in the past few frames) which helps in better prediction of affordances. 



% \tr{Finally describe the timestamp weighted features formally, and then the architecture}
%In order to combat this scenario, we propose a modification in the architecture in Conditional Affordance Learning model \cite{sauer2018conditional}. CARLA \cite{dosovitskiy2017carla} provides us with timestamp information for each frame. We have used this information to form timestamp weighed features to be fed into the different task blocks for prediction of affordances. The reason behind using timestamp information is to make the task blocks learn the gaps in irregularly spaced frames and eventually learn to predict its corresponding affordances.



\subsection{Online Subset Selection}
\label{sec:subset}

%We are interested in training autonomous driving models with using input videos with missing frames. In this paper, we use the conditional affordance learning model \cite{sauer2018conditional}, which is based on direct perception approach, as our driving model. We choose this model due to its simplicity, practicality, and also the available source code and ability to integrate into the popular CARLA simulator \cite{dosovitskiy2017carla}.

%Most models for prediction of intermediate representations, or "affordances" take a buffer of past few frames as input, for prediction of local driving directions, e.g. "centerline distance" or "relative angle" in case of CAL \cite{sauer2018conditional}. This helps in keeping track of the current state of the vehicle, and along with the directional commands, predict the next state of the vehicle.

In this section, we describe our online subset selection formulation. As discussed above, the input to autonomous driving model is a set of episodes, each of which is a sequence of video frames, annotated by corresponding affordances. However, for simplicity, in the context of online frame subset selection, we assume that the episodes have an ordering, and hence the entire data can be thought of as a single dataset $\mathcal{D}$ comprising of video frames $\bx_i$, and labels $\by_i$ corresponding to various learning tasks such as prediction of driving affordances. 
Hence, $\mathcal{D} = \{ (\bx_i,\by_i),\ i=1,\dots,n \}$ where $n$ is the total number of datapoints (annotated video frames) in the dataset. 

Similar to \cite{das2020multi}, we process the data in batches $X_t ,\ t = 1,\dots,T$, where batch size $|X_t| = m$. Hence $mT = n$. We also define the cumulative sets $C_t = \cup_{i=1}^t X_i$. We are interested in constructing representative sets $R_t \subseteq C_t$, such that 
%$R_t$ retains meaningful information from $C_t$ and 
affordance prediction models trained on $R_t$ perform similarly to those trained on $C_t$ and size of $R_t$ is minimized. 
Here, performance is the generalization error, measured as the error on a common test set.


This can be posed as an online subset selection problem \cite{elhamifar2017online}. Given a datapoint $i$ from the set $X_{t+1}$ and another datapoint $j$ from the set $R_t$, $R_{t+1}$ is constructed by solving the problem:
\small
\begin{align}
\label{eqn:eq1}
    &\min_{z^o_{ij},z^n_{ij}} & \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij} + \sum_{i,j=1}^m z_{ij}^n d^n_{ij} + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
    &s.t. & \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    & & z_{i,j}^n, z_{i,j}^o \in [0,1]
    \nonumber
\end{align}
\normalsize
where $d^o_{ij}$ denotes the notion of dissimilarity between new frame $i$ (from $X_{t+1}$) and old frame $j$ (from $R_t$), $d^n_{ij}$ denotes the notion of dissimilarity between new frames $i$ and $j$ (from $X_{t+1}$), and $z_{ij}^o, z_{ij}^n $ are relaxed versions of binary assignment variables. $z_{ij}^o=1 $ denotes that the representative of $i^{th}$ new example (from $X_{t+1}$) is $j^{th}$ old example (from $R_t$), and $z_{ij}^n=1$ denotes that representative of $i^{th}$ new example (from $X_{t+1})$ is the $j^{th}$ new example. Note that here, the indexes $i,j$ are internal to sets $R_t$ and $X_{t+1}$ depending on context $o$ or $n$.

While $d_{ij}$ can be used to encode the perceptual dissimilarity between video frames $i$ and $j$, the above formulation does not incorporate the the pointwise attributes of each data point $x_i,y_i$ w.r.t. to the already trained model $M_t$, where $(x_i,y_i)\in X_{t+1}$. Let $L^n_i$ denote the loss value for datapoint $i$ in $X_{t+1}$ and analogously for $L^o_i$ (denoting loss for datapoint $i$ in $R_t$). \cite{das2020multi} proposes to incorporate it by constructing the $Q$ function as a weighted average of $d$  and $L$ as:

\small
\begin{equation}
Q_{ij} = \rho d_{ij} - (1-\rho) L_j \label{eq:joint}
\label{eq:join}
\end{equation}
\normalsize
where, $0 \leq \rho \leq 1$ is the weightage given to pairwise dissimilarity criteria.
Hence, their \cite{das2020multi}  final selection problem is:
\small
\begin{align}
\label{eqn:oldsiftloss}
    &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
    &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
\end{align}
\normalsize
Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, as explained before, a representative $j$ should have the minimum dissimilarity with a new frame $i$. 


%Since, most of the frames that are input to the driving model and are redundant in terms of information content, and cause a huge overhead in terms of processing power at runtime as well as training time. 
%In this paper, we propose subset selection mechanisms for intelligent selection of images which can be fed to the existing models for autonomous driving and can be trained and tested (operated) on videos with massively and unevenly dropped frames.

%\subsection{Model Description}

%We consider a dataset $\mathcal{D}$ comprising of datapoints (e.g. buffers of video frames) $x_i$, and labels $y_i$ corresponding to various learning tasks on buffers of video frames such as prediction of driving affordances. 
%The data may arrive in either a streaming manner, or in batches. 

%\subsection{Multiple-criteria-based subset selection}

%The above formulation relies on (dis)similarity between the examples in the new set ($X_{t+1}$) and existing representative set ($R_{t}$), for selecting the new representatives. However, this does not take care of the possibility that in many application scenarios, one is interested in selecting points which provide better performance towards a given task. For example, one could be interested in selecting video frames from a self driving car video, which are helpful towards training a driving model. In such scenarios, it is important to also consider other signals, e.g. loss which are dependent on models trained on old representative datapoints (frames). In this section, we develop a novel formulation for using such criteria.

%Let $M_t$ be the model trained on $R_t$.
%%, and $l_t(x_i,y_i)$ be the loss incurred by the datapoint $(x_i,y_i), i\in C_{t+1}$, using the model $M_t$. 
%For our formulation, we further define two types of selection criteria: \textit{pairwise and pointwise criteria}. Pairwise dissimilarity criteria $d_{ij}(t)=d((x_i,y_i), (x_j,y_j) | M_t) $ are evaluated on pairs of examples $( (x_i,y_i), (x_j,y_j) )$ at any point in time. Note that $d_{ij}(t)$ may or may not depend on the current model. For example, in this paper we use SIFT \cite{lowe1999object} as a measure of dissimilarity, which is related to the perceptual dissimilarity between two images and hence independent of the model.
%Pointwise ``dis-quality'' criteria $q_i(t) = q((x_i,y_i)|M_t)$ measure an inverse goodness score for a datapoint $(x_i,y_i)$ given a trained model at time $t$. 
%In this study, we consider the negative log-loss denoted as $L_i(t)=L(x_i,y_i|M_t)$. Here, the loss refers to the multi-task loss which is a combination of the losses from all affordances in the driving model.

%We define the joint pairwise and pointwise dis-quality criteria as:
%\begin{equation}
%Q_{ij}(t) = \rho d_{ij}(t) + (1-\rho) q_j(t) \label{eq:joint}
%\end{equation}
%where, $0 \leq \rho \leq 1$ is the weightage given to pairwise dissimilarity criteria.

%We have setup the joint dis-quality criteria above in a manner such that new datapoints with lower dis-quality score results in better candidates for selection. Hence we pose the  final selection problem as:
%\begin{align}
%\label{eqn:oldsiftloss}
%    &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q_{ij}(t) + \sum_{i,j=1}^m z_{ij}^n Q_{ij}(t) \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
%    &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
%    & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
%\end{align}
%Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, as explained before, a representative $j$ should have the minimum dissimilarity with a new frame $i$. 

\textbf{Drawbacks of the above formulation}:\\
\tr{The first drawback of the formulation described in Equation \ref{eqn:oldsiftloss} is that pointwise metric has very limited impact on the set of points selected. To see this, note that 
 using only pointwise metric yields a maximum of 1 representative for all images belonging to incoming set.} 
For pointwise score ($\rho = 0$), the score function is $ - \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t) \right] $. 
%An interesting observation is that when $\rho = 0$, either $0$ or $1$ new representative points are selected. 
A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
\begin{itemize}
\item $L^n_j$ is the highest among all $j\in X_{t+1}$.
\item $L^n_j > L^o_i,\ \forall i\in R_t$
\item $L^n_j > - \lambda  \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p $
\end{itemize}
\tr{The second drawback is that there is no obvious connection between intended compression ratio, and $\lambda$.} Hence, one has to perform grid search over the values of $\lambda$ in order to obtain a particular compression ratio.
% with lowest value of $q_j(t)$ is selected only when $q_j(t) < \lambda  \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p $. Hence, these hyperparameter values produce trivial results.

%\subsection{Improved Multiple-criteria-based subset selection}
%\label{improved}

%In this formulation, we intend to address the shortcomings in the last formulation. The drawbacks of the method described in Equation \ref{eqn:oldsiftloss} are:
%\begin{enumerate}
%    \item Using only pointwise metric yields only 1 representative for all images belonging to incoming set. This suppresses the impact of the pointwise metrics on the subset selection.
%    \item We have to grid search for the value of $\lambda$ in order to obtain a particular compression ratio.
%\end{enumerate}



\textbf{New formulation}:
Overcoming the drawbacks, we have re-formulated Equation \ref{eqn:oldsiftloss} into the following form:
\small
\begin{align}
\label{eqn:newsiftloss}
    \min_{z^o_{ij},z^n_{ij}} & \rho \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij}(t) + \sum_{i,j=1}^m z_{ij}^n d^n_{ij}(t) \nonumber \\ & -(1-\rho) (\sum_{j=1}^{|R_t|} S_j^o * L_j^o  + \sum_{j=1}^m S_j^n * L_j^n )\\
    &s.t. \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    &z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber \\ 
    &\sum_{j=1}^{m}\| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \leq frac * m
    \nonumber
\end{align}
\normalsize

where, $S^o_j$ = $\frac{1}{\epsilon} \min (\epsilon , \sum_{i=1}^m z_{ij}^o)$ , $S^n_j$ = $\frac{1}{\epsilon} \min (\epsilon , \sum_{i=1}^m z_{ij}^n)$ are the vectors with each element indicating whether j-th indexed image is a representative of any incoming image or not.
$L_i^o$ and $L_i^n$ refer to the pointwise metric (here multi-task loss) corresponding to images belonging to existing and incoming set respectively and, \textit{frac} indicates the fraction of elements we want to retain during selection.
$\epsilon$ is a user input which is designed to be the maximum value taken by the variable $\sum_i z_{ij}$, when none of the $z_{ij}$ denote a representative relation to be true. In an ideal situation (when we achieve a $\{0,1\}$ solution to $z_{ij}$), any positive value for $\epsilon$ is sufficient. In practise, we set $\epsilon$ to a value less than $1$, e.g.$\epsilon = 0.9$.

The key difference between the current formulation and the formulation in equation \ref{eqn:oldsiftloss} is that, in the current formulation, each potential representative can contribute a maximum of its own (negative) loss value, since $S_j$'s can take a maximum value of $1$. Whereas in the formulation in  equation \ref{eqn:oldsiftloss} it is possible for a datapoint to contribute $ - \sum_{i=1}^{m} (L_i^n + L_i^o)$ by becoming a representative for every other point. However, in reality it only adds one data point to the training set. Also, note that $S$ is a concave function, which makes the current formulation a convex optimization problem.

%Unlike the last formulation where pairwise and pointwise metrics were weighed into a single matrix $Q_{ij}$, here we separated the metrics giving each of them their respective indicator variable. This aids in bringing out the impact of pointwise metrics on subset selection. We also resort to pointwise "quality" criteria instead of the inverse goodness score used in Equation \ref{eqn:oldsiftloss}.

The subset cardinality was manually tuned with the help of $\lambda$ in Equation \ref{eqn:oldsiftloss}. In order to have a control over the selection, we brought the cardinality criteria into the constraints by introducing the term \textit{frac} which is manually provided based on the desired compression ratio. For instance, for a compression ratio of 100:20, we provide the value of \textit{frac} as 0.2.

Having addressed the drawbacks, the usage of pointwise metric and the control over cardinality has a positive impact on the subset selection, whose performance is explored in the next section.

\section{Submodular Method}


In this section, we discuss an algorithm based on constrained  submodular optimization for the optimization proposed in equation \ref{eqn:newsiftloss}. We may write the same in the following form:
\small
\begin{equation}
    min_{S \subseteq X} f(S)
\end{equation}
\normalsize
where the function $f(S)$ can be defined as:
\small
\begin{equation}
    f(S) = \sum_{i \in X} min \{ min_{j \in R} (d_{ij}^{o} + \tilde{L_j^o}) , min_{j \in S} (d_{ij}^{n} + \tilde{L_j^n}) \} 
\end{equation}
\normalsize
 with $d_ij$ being the pairwise dissimilalrity and $\tilde{L_j}$ being the inverse loss value.
 
Next, we prove that $-f(S)$ in our definition is submodular. According to definition of submodularity, for $-f(S)$ to be submodular, 
\small
\begin{equation}
    -f(S \cup \{x\}) - (-f(S)) \geq -f(T \cup \{x\}) - (-f(T))
\end{equation}
\normalsize
where $S \subseteq T$ , $x \notin S $ , $x \notin T $. Let us define the notations:\\
\small
\begin{enumerate}
    \item $D_i(S)$ : Function value for finding a representative for an element i $\in$ X with past representative set as $S$. 
    \item $D_i(T)$ : Function value for finding a representative for an element i $\in$ X with past representative set as $T$.
    \item $D_{ix}$ : Function value for finding a representative for an element i $\in$ X with past representative set as $S \cup x$ or $T \cup x$.
\end{enumerate}
\normalsize
Note that there can be 3 possibilities after addition of $x$.
\small
\begin{enumerate}
    \item $x$ does not become a representative of $i \in X$.
    \item $x$ becomes a representative of $i \in X$ only with past representative set as $S$.
    \item $x$ becomes a representative of $i \in X$ with both $S$ and $T$ as past representative sets. 
\end{enumerate}
\normalsize
To prove: 
\small
\begin{equation}
    f(S) - f(S \cup \{x\}) \geq f(T) - f(T \cup \{x\})
\end{equation}
\normalsize
or
\small
\begin{equation}
    D_i(S) - D_{ix} \geq  D_i(T) - D_{ix}
\end{equation}
\normalsize
Under the first possibility, both sides of inequality lead to $0$.

Since $S \subseteq T$, by the form of $f(S)$, $D_i(T) \leq D_i(S)$. Addition of representative for an element $i \in X$ can either decrease the function value or keep it the same.
\small
\begin{equation}
    \therefore{} D_i(T) - D_{ix} \geq 0 , 
    D_i(S) - D_{ix} \geq 0
\end{equation}
\normalsize
Hence, under the second possibility, $D_i(S) - D_{ix} \geq  D_i(T) - D_{ix}$ or $D_i(S) - D_{ix} \geq  0$.

Now, $\because D_i(T) \leq D_i(S), \therefore{} D_i(T) - D_{ix} \leq D_i(S) - D_{ix}$ or $D_i(S) - D_{ix} \geq D_i(T) - D_{ix}$.

Therefore, $-f(S)$ is submodular.

We also discuss an algorithm proposed in  SODA 2014\citep{buchbinder2014submodular} based on constrained submodular optimisation and adopt it in our framework in Algorithm \ref{algo:submodular}.
\small
\begin{algorithm}[tb]
 \caption{: Subset Selection using Submodular approach}
 \label{algo:submodular}
 \begin{algorithmic}[1]
 
 \State \textbf{Input:}
 \State \hspace{2mm}$S_0$: Initial representative set
 \State \hspace{2mm}$X$: Incoming Set of Instances
 \State \hspace{2mm}$k$: Subset cardinality
 \State \hspace{2mm}$f(S)$: Function to be maximised
 \State \hspace{2mm}$S_0 = \phi$
%  \State \hspace{2mm}$T$: Number of incoming batches
 \State \textbf{Process:}
 \hspace{2mm}\For{$i$ = 1,2, $\ldots$, $k$}
 \hspace{2mm}\For{each x $\in$ X \textbackslash $S_{i-1}$} do
 \State  $fv_x \leftarrow f(S_{i-1} \cup {x})$
  \EndFor
%  \State  Select a subset of size $k$ , say $M_i$ such that they yield the maximum value in $fv$
 \State  Select a subset of size $k$ , say $M_i$ such that $\sum_{m \in M_i} fv_m$ is maximised
 \State  Let $u_i$ be a random element from $M_i$ 
 \State $S_i \leftarrow S_{i-1}\cup {u_i}$
 \EndFor
 \State \textbf{Output:}
 \State $S_k$ : Subset of size $k$
 \end{algorithmic}
\end{algorithm}
\normalsize

%%%%% Example with rho = 0
% Let both $R_t$ and $X_t$ have two frames each.\\
% $d^o = \begin{bmatrix}
% 1 & 2\\
% 1 & 3
% \end{bmatrix}$ , $d^n = \begin{bmatrix}
% 2 & 1\\
% 1 & 3
% \end{bmatrix}$ , $L^o = \begin{bmatrix}
% 1 & 3
% \end{bmatrix}$ and $L^n = \begin{bmatrix}
% 2 & 1
% \end{bmatrix}$. When $\rho$ = 0, from Equation \ref{eq:join}, $Q_{ij}^o$ = $- (1-\rho) L_j^o$ and similarly, $Q_{ij}^n$ = $- (1-\rho) L_j^n$. Having used the above values in Equation \ref{eqn:oldsiftloss}, representative of any instance $i$ from $X_t$ $(i = 1, ..., m)$ will be the point which has the highest value of loss which can either belong to $L^o$ or $L^n$. So, all the frames in $X_t$ will be represented by only one frame from $X_t$ or $R_t$ whichever yields the highest loss. In the above mentioned example, the second frame from $R_t$ ($\because L^o[1] = 3$) will be chosen as the representative for all the frames in $X_t$.

==> method3.tex <==

\newtheorem{remark}{Remark}

In this section, we develop a novel formulation for online selection of subsets of video frames, in the presence of multiple input criteria - both for pairs of input frames and for single input frame. 


\subsection{Background}
\label{sec:subset}


In this section, we describe our online subset selection formulation. As discussed above, the input to autonomous driving model is a set of episodes, each of which is a sequence of video frames, annotated by corresponding affordances. However, for simplicity, in the context of online frame subset selection, we assume that the episodes have an ordering, and hence the entire data can be thought of as a single dataset $\mathcal{D}$ comprising of video frames $\bx_i$, and labels $\by_i$ corresponding to various learning tasks such as prediction of driving affordances. 
Hence, $\mathcal{D} = \{ (x_i,y_i),\ i=1,\dots,n \}$ where $n$ is the total number of datapoints (annotated video frames) in the dataset. 

Similar to \cite{das2020multi}, we process the data in batches $X_t ,\ t = 1,\dots,T$, where batch size $|X_t| = m$. Hence $mT = n$. We also define the cumulative sets $C_t = \cup_{i=1}^t X_i$. We are interested in constructing representative sets $R_t \subseteq C_t$, such that 
%$R_t$ retains meaningful information from $C_t$ and 
affordance prediction models trained on $R_t$ perform similarly to those trained on $C_t$ and size of $R_t$ is minimized. 
Here, performance is the generalization error, measured as the error on a common test set.

\subsection{Submodular Method}

In this section, we discuss an algorithm based on constrained  submodular optimization for the optimization proposed in equation \ref{eqn:newsiftloss}. We may write the same in the following form:
\small
\begin{equation}
    min_{S \subseteq X} f(S)
\end{equation}
\normalsize
where the function $f(S)$ can be defined as:
\small
\begin{equation}
    f(S) = \sum_{i \in X} min \{ min_{j \in R} (d_{ij}^{o} + \tilde{L_j^o}) , min_{j \in S} (d_{ij}^{n} + \tilde{L_j^n}) \} 
\label{eq:submod}
\end{equation}
\normalsize
 with $d_ij$ being the pairwise dissimilalrity and $\tilde{L_j}$ being the inverse loss value.

By definition, $-f(S)$ is submodular. For proof, see Supplementary.
% Next, we prove that $-f(S)$ in our definition is submodular. According to definition of submodularity, for $-f(S)$ to be submodular, 
% \small
% \begin{equation}
%     -f(S \cup \{x\}) - (-f(S)) \geq -f(T \cup \{x\}) - (-f(T))
% \end{equation}
% \normalsize
% where $S \subseteq T$ , $x \notin S $ , $x \notin T $. Let us define the notations:\\
% \small
% \begin{enumerate}
%     \item $D_i(S)$ : Function value for finding a representative for an element i $\in$ X with past representative set as $S$. 
%     \item $D_i(T)$ : Function value for finding a representative for an element i $\in$ X with past representative set as $T$.
%     \item $D_{ix}$ : Function value for finding a representative for an element i $\in$ X with past representative set as $S \cup x$ or $T \cup x$.
% \end{enumerate}
% \normalsize
% Note that there can be 3 possibilities after addition of $x$.
% \small
% \begin{enumerate}
%     \item $x$ does not become a representative of $i \in X$.
%     \item $x$ becomes a representative of $i \in X$ only with past representative set as $S$.
%     \item $x$ becomes a representative of $i \in X$ with both $S$ and $T$ as past representative sets. 
% \end{enumerate}
% \normalsize
% To prove: 
% \small
% \begin{equation}
%     f(S) - f(S \cup \{x\}) \geq f(T) - f(T \cup \{x\})
% \end{equation}
% \normalsize
% or
% \small
% \begin{equation}
%     D_i(S) - D_{ix} \geq  D_i(T) - D_{ix}
% \end{equation}
% \normalsize
% Under the first possibility, both sides of inequality lead to $0$.

% Since $S \subseteq T$, by the form of $f(S)$, $D_i(T) \leq D_i(S)$. Addition of representative for an element $i \in X$ can either decrease the function value or keep it the same.
% \small
% \begin{equation}
%     \therefore{} D_i(T) - D_{ix} \geq 0 , 
%     D_i(S) - D_{ix} \geq 0
% \end{equation}
% \normalsize
% Hence, under the second possibility, $D_i(S) - D_{ix} \geq  D_i(T) - D_{ix}$ or $D_i(S) - D_{ix} \geq  0$.

% Now, $\because D_i(T) \leq D_i(S), \therefore{} D_i(T) - D_{ix} \leq D_i(S) - D_{ix}$ or $D_i(S) - D_{ix} \geq D_i(T) - D_{ix}$.

% Therefore, $-f(S)$ is submodular.

Inspired from algorithm proposed in  SODA 2014\cite{buchbinder2014submodular} based on constrained submodular optimisation, we adopt it in our framework in Algorithm \ref{algo:submodular}. The algorithm is a randomised greedy algorithm that examines the dataset $k$ times to select representatives for the incoming elements.
\small
\begin{algorithm}[tb]
 \caption{: Subset Selection using Submodular approach}
 \label{algo:submodular}
 \begin{algorithmic}[1]
 
 \State \textbf{Input:}
 \State \hspace{2mm}$S_0$: Initial representative set
 \State \hspace{2mm}$X$: Incoming Set of Instances
 \State \hspace{2mm}$k$: Subset cardinality
 \State \hspace{2mm}$f(S)$: Function to be maximised
 \State \hspace{2mm}$S_0 = \phi$
%  \State \hspace{2mm}$T$: Number of incoming batches
 \State \textbf{Process:}
 \hspace{2mm}\For{$i$ = 1,2, $\ldots$, $k$}
 \hspace{2mm}\For{each x $\in$ X \textbackslash $S_{i-1}$} do
 \State  $fv_x \leftarrow f(S_{i-1} \cup {x})$
  \EndFor
%  \State  Select a subset of size $k$ , say $M_i$ such that they yield the maximum value in $fv$
 \State  Select a subset of size $k$ , say $M_i$ such that $\sum_{m \in M_i} fv_m$ is maximised
 \State  Let $u_i$ be a random element from $M_i$ 
 \State $S_i \leftarrow S_{i-1}\cup {u_i}$
 \EndFor
 \State \textbf{Output:}
 \State $S_k$ : Subset of size $k$
 \end{algorithmic}
\end{algorithm}
\normalsize

\subsection{Convex formulation}

This can be posed as an online subset selection problem \cite{elhamifar2017online}. Given a datapoint $i$ from the set $X_{t+1}$ and another datapoint $j$ from the set $R_t$, $R_{t+1}$ is constructed by solving the problem:
\small
\begin{align}
\label{eqn:eq1}
    &\min_{z^o_{ij},z^n_{ij}} & \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij} + \sum_{i,j=1}^m z_{ij}^n d^n_{ij} + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
    &s.t. & \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    & & z_{i,j}^n, z_{i,j}^o \in [0,1]
    \nonumber
\end{align}
\normalsize
where $d^o_{ij}$ denotes the notion of dissimilarity between new frame $i$ (from $X_{t+1}$) and old frame $j$ (from $R_t$), $d^n_{ij}$ denotes the notion of dissimilarity between new frames $i$ and $j$ (from $X_{t+1}$), and $z_{ij}^o, z_{ij}^n $ are relaxed versions of binary assignment variables. $z_{ij}^o=1 $ denotes that the representative of $i^{th}$ new example (from $X_{t+1}$) is $j^{th}$ old example (from $R_t$), and $z_{ij}^n=1$ denotes that representative of $i^{th}$ new example (from $X_{t+1})$ is the $j^{th}$ new example. Note that here, the indexes $i,j$ are internal to sets $R_t$ and $X_{t+1}$ depending on context $o$ or $n$.

While $d_{ij}$ can be used to encode the perceptual dissimilarity between video frames $i$ and $j$, the above formulation does not incorporate the the pointwise attributes of each data point $x_i,y_i$ w.r.t. to the already trained model $M_t$, where $(x_i,y_i)\in X_{t+1}$. Let $L^n_i$ denote the loss value for datapoint $i$ in $X_{t+1}$ and analogously for $L^o_i$ (denoting loss for datapoint $i$ in $R_t$). \cite{das2020multi} proposes to incorporate it by constructing the $Q$ function as a weighted average of $d$  and $L$ as:

\small
\begin{equation}
Q_{ij} = \rho d_{ij} - (1-\rho) L_j
\label{eq:joint}
\end{equation}
\normalsize
where, $0 \leq \rho \leq 1$ is the weightage given to pairwise dissimilarity criteria.
Hence, their \cite{das2020multi}  final selection problem is:
\small
\begin{align}
\label{eqn:oldsiftloss}
    &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
    &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
\end{align}
\normalsize
Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, as explained before, a representative $j$ should have the minimum dissimilarity with a new frame $i$. 

\textbf{Drawbacks of the above formulation}:\\

The first drawback of the formulation described in Equation \ref{eqn:oldsiftloss} is that pointwise metric has very limited impact on the set of points selected. The following remark notes this when $\rho = 0$.
\tr{To see this, note that using only pointwise metric yields a maximum of 1 representative for all images belonging to incoming set.
An interesting observation is that when $\rho = 0$, either $0$ or $1$ new representative points are selected. }

\begin{theorem}
The score function in Equation \ref{eqn:oldsiftloss} is $\sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\$

A new point $j$ from the set $X_{t+1}$  for $\rho \leq 0.5$ is selected as a representative by minimizing the above function, only if all of the following hold:
\begin{itemize}
\item $\sum_{i=1}^m Q^n_{ij} < \sum_{i=1}^m Q^n_{ij'}$ where $j \neq j'$
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
\item $\sum_{i=1}^m Q^n_{ij} < \frac{ \sum_{i=1}^m z_{i,k}^o Q^o_{ik} + \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
\end{itemize}
where k = $argmin_j \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{i,j}^o Q_{i,j}^o$
\end{theorem}

\begin{corollary}
For pointwise score ($\rho = 0$), the score function is $- \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t)\right]+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p $

A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
\begin{itemize}
\item $L^n_j$ is the highest among all $j\in X_{t+1}$.
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
\item $L^n_j > \frac{ \sum_{i=1}^m z_{i,k}^o L_k^o - \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
\end{itemize}
\end{corollary}

% \begin{remark}
% For pointwise score ($\rho = 0$), the score function is $- \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t)+ \nonumber \\ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \right]$

% A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
% \begin{itemize}
% \item $L^n_j$ is the highest among all $j\in X_{t+1}$.
% % \item $L^n_j > L^o_i,\ \forall i\in R_t$
% \item $L^n_j > \frac{ \sum_{i=1}^m z_{i,k}^o L_k^o + \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
% \end{itemize}

% The last condition for $p=2$ boils down to $l_j^n \geq \frac{1}{\sqrt{m}}$.

% \end{remark}

% \begin{remark}
% For $\rho = 0.1$ to $0.5$, the score function is $\sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} \nonumber \\ + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\$

% A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
% \begin{itemize}
% \item $Q^n_{ij} < Q^n_{ij'}$ where $j \neq j'$
% % \item $L^n_j > L^o_i,\ \forall i\in R_t$
% \item $Q^n_{ij} < \frac{ \sum_{i=1}^m z_{i,k}^o Q^o_{ik} - \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
% \end{itemize}


% \end{remark}

% \begin{remark}
% For pointwise score ($\rho = 0$), the score function is $ - \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t) \right] $. 
% A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
% \begin{itemize}
% \item $L^n_j$ is the highest among all $j\in X_{t+1}$.
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
% \item $L^n_j > \lambda \frac{\| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
% \end{itemize}
% The last condition for $p=2$ boils down to $l_j^n \geq \frac{1}{\sqrt{m}}$.

% \end{remark}

%%%%% Example with rho = 0
Let both $R_t$ and $X_t$ have two frames each.\\
$d^o = \begin{bmatrix}
1 & 2\\
1 & 3
\end{bmatrix}$ , $d^n = \begin{bmatrix}
2 & 1\\
1 & 3
\end{bmatrix}$ , $L^o = \begin{bmatrix}
1 & 3
\end{bmatrix}$ and $L^n = \begin{bmatrix}
2 & 1
\end{bmatrix}$. When $\rho$ = 0, from Equation \ref{eq:join}, $Q_{ij}^o$ = $- (1-\rho) L_j^o$ and similarly, $Q_{ij}^n$ = $- (1-\rho) L_j^n$. Having used the above values in Equation \ref{eqn:oldsiftloss}, representative of any instance $i$ from $X_t$ $(i = 1, ..., m)$ will be the point which has the highest value of loss which can either belong to $L^o$ or $L^n$. So, all the frames in $X_t$ will be represented by only one frame from $X_t$ or $R_t$ whichever yields the highest loss. In the above mentioned example, the second frame from $R_t$ ($\because L^o[1] = 3$) will be chosen as the representative for all the frames in $X_t$.

\tr{The second drawback is that there is no obvious connection between intended compression ratio, and $\lambda$.} Hence, one has to perform grid search over the values of $\lambda$ in order to obtain a particular compression ratio.


\subsection{New formulation}

Overcoming the drawbacks, we have re-formulated Equation \ref{eqn:oldsiftloss} into the following form:
\small
\begin{align}
\label{eqn:newsiftloss}
    \min_{z^o_{ij},z^n_{ij}} & \rho \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij}(t) + \sum_{i,j=1}^m z_{ij}^n d^n_{ij}(t) \nonumber \\ & -(1-\rho) (\sum_{j=1}^{|R_t|} S_j^o * L_j^o  + \sum_{j=1}^m S_j^n * L_j^n )\\
    &s.t. \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    &z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber \\ 
    &\sum_{j=1}^{m}\| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \leq frac * m
    \nonumber
\end{align}
\normalsize

where, $S^o_j$ = $\frac{1}{\epsilon} \min (\epsilon , \sum_{i=1}^m z_{ij}^o)$ , $S^n_j$ = $\frac{1}{\epsilon} \min (\epsilon , \sum_{i=1}^m z_{ij}^n)$ are the vectors with each element indicating whether j-th indexed image is a representative of any incoming image or not.
$L_i^o$ and $L_i^n$ refer to the pointwise metric (here multi-task loss) corresponding to images belonging to existing and incoming set respectively and, \textit{frac} indicates the fraction of elements we want to retain during selection.
$\epsilon$ is a user input which is designed to be the maximum value taken by the variable $\sum_i z_{ij}$, when none of the $z_{ij}$ denote a representative relation to be true. In an ideal situation (when we achieve a $\{0,1\}$ solution to $z_{ij}$), any positive value for $\epsilon$ is sufficient. In practise, we set $\epsilon$ to a value less than $1$, e.g.$\epsilon = 0.9$.

The key difference between the current formulation and the formulation in equation \ref{eqn:oldsiftloss} is that, in the current formulation, each potential representative can contribute a maximum of its own (negative) loss value, since $S_j$'s can take a maximum value of $1$. Whereas in the formulation in  equation \ref{eqn:oldsiftloss} it is possible for a datapoint to contribute $ - \sum_{i=1}^{m} (L_i^n + L_i^o)$ by becoming a representative for every other point. However, in reality it only adds one data point to the training set. Also, note that $S$ is a concave function, which makes the current formulation a convex optimization problem.



The subset cardinality was manually tuned with the help of $\lambda$ in Equation \ref{eqn:oldsiftloss}. In order to have a control over the selection, we brought the cardinality criteria into the constraints by introducing the term \textit{frac} which is manually provided based on the desired compression ratio. For instance, for a compression ratio of 100:20, we provide the value of \textit{frac} as 0.2.

Having addressed the drawbacks, the usage of pointwise metric and the control over cardinality has a positive impact on the subset selection, whose performance is explored in the next section.


%Since, most of the frames that are input to the driving model and are redundant in terms of information content, and cause a huge overhead in terms of processing power at runtime as well as training time. 
%In this paper, we propose subset selection mechanisms for intelligent selection of images which can be fed to the existing models for autonomous driving and can be trained and tested (operated) on videos with massively and unevenly dropped frames.

%\subsection{Model Description}

%We consider a dataset $\mathcal{D}$ comprising of datapoints (e.g. buffers of video frames) $x_i$, and labels $y_i$ corresponding to various learning tasks on buffers of video frames such as prediction of driving affordances. 
%The data may arrive in either a streaming manner, or in batches. 

%\subsection{Multiple-criteria-based subset selection}

%The above formulation relies on (dis)similarity between the examples in the new set ($X_{t+1}$) and existing representative set ($R_{t}$), for selecting the new representatives. However, this does not take care of the possibility that in many application scenarios, one is interested in selecting points which provide better performance towards a given task. For example, one could be interested in selecting video frames from a self driving car video, which are helpful towards training a driving model. In such scenarios, it is important to also consider other signals, e.g. loss which are dependent on models trained on old representative datapoints (frames). In this section, we develop a novel formulation for using such criteria.

%Let $M_t$ be the model trained on $R_t$.
%%, and $l_t(x_i,y_i)$ be the loss incurred by the datapoint $(x_i,y_i), i\in C_{t+1}$, using the model $M_t$. 
%For our formulation, we further define two types of selection criteria: \textit{pairwise and pointwise criteria}. Pairwise dissimilarity criteria $d_{ij}(t)=d((x_i,y_i), (x_j,y_j) | M_t) $ are evaluated on pairs of examples $( (x_i,y_i), (x_j,y_j) )$ at any point in time. Note that $d_{ij}(t)$ may or may not depend on the current model. For example, in this paper we use SIFT \cite{lowe1999object} as a measure of dissimilarity, which is related to the perceptual dissimilarity between two images and hence independent of the model.
%Pointwise ``dis-quality'' criteria $q_i(t) = q((x_i,y_i)|M_t)$ measure an inverse goodness score for a datapoint $(x_i,y_i)$ given a trained model at time $t$. 
%In this study, we consider the negative log-loss denoted as $L_i(t)=L(x_i,y_i|M_t)$. Here, the loss refers to the multi-task loss which is a combination of the losses from all affordances in the driving model.

%We define the joint pairwise and pointwise dis-quality criteria as:
%\begin{equation}
%Q_{ij}(t) = \rho d_{ij}(t) + (1-\rho) q_j(t) \label{eq:joint}
%\end{equation}
%where, $0 \leq \rho \leq 1$ is the weightage given to pairwise dissimilarity criteria.

%We have setup the joint dis-quality criteria above in a manner such that new datapoints with lower dis-quality score results in better candidates for selection. Hence we pose the  final selection problem as:
%\begin{align}
%\label{eqn:oldsiftloss}
%    &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q_{ij}(t) + \sum_{i,j=1}^m z_{ij}^n Q_{ij}(t) \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
%    &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
%    & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
%\end{align}
%Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, as explained before, a representative $j$ should have the minimum dissimilarity with a new frame $i$. 

%Unlike the last formulation where pairwise and pointwise metrics were weighed into a single matrix $Q_{ij}$, here we separated the metrics giving each of them their respective indicator variable. This aids in bringing out the impact of pointwise metrics on subset selection. We also resort to pointwise "quality" criteria instead of the inverse goodness score used in Equation \ref{eqn:oldsiftloss}.

% with lowest value of $q_j(t)$ is selected only when $q_j(t) < \lambda  \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p $. Hence, these hyperparameter values produce trivial results.

%\subsection{Improved Multiple-criteria-based subset selection}
%\label{improved}

%In this formulation, we intend to address the shortcomings in the last formulation. The drawbacks of the method described in Equation \ref{eqn:oldsiftloss} are:
%\begin{enumerate}
%    \item Using only pointwise metric yields only 1 representative for all images belonging to incoming set. This suppresses the impact of the pointwise metrics on the subset selection.
%    \item We have to grid search for the value of $\lambda$ in order to obtain a particular compression ratio.
%\end{enumerate}


==> newmethod.tex <==
% In this section, we develop a novel formulation for online selection of subsets of video frames, in the presence of multiple input criteria - both for pairs of input frames and for single input frame.

In this section, we develop a novel thresholded formulation for efficient incorporation of pointwise metric along with pairwise metric. Alongside, we also propose a set-function based criteria which is proved to be a submodular function and can be adopted for subset selection using submodular approximation techniques.

\noteng{Where is the threshold part??}

\subsection{Submodular Method}

In this section, we discuss an algorithm based on constrained  submodular optimization for online subset selection problem incorporating both pairwise and pointwise attributes. We may write the following optimisation problem:

\small
\begin{equation}
    min_{S \subseteq X} f(S)
\end{equation}
\normalsize
where the function $f(S)$ can be defined as:
\small
\begin{equation}
    f(S) = \sum_{i \in X} min \{ min_{j \in R} (d_{ij}^{o} + \tilde{L_j^o}) , min_{j \in S} (d_{ij}^{n} + \tilde{L_j^n}) \} 
\label{eq:submod}
\end{equation}
\normalsize
 with $d_{ij}$ being the pairwise dissimilarity and $\tilde{L_j}$ being the inverse loss value.

By definition, $-f(S)$ is submodular. For proof, see Supplementary.

% Next, we prove that $-f(S)$ in our definition is submodular. According to definition of submodularity, for $-f(S)$ to be submodular, 
% \small
% \begin{equation}
%     -f(S \cup \{x\}) - (-f(S)) \geq -f(T \cup \{x\}) - (-f(T))
% \end{equation}
% \normalsize
% where $S \subseteq T$ , $x \notin S $ , $x \notin T $. Let us define the notations:\\
% \small
% \begin{enumerate}
%     \item $D_i(S)$ : Function value for finding a representative for an element i $\in$ X with past representative set as $S$. 
%     \item $D_i(T)$ : Function value for finding a representative for an element i $\in$ X with past representative set as $T$.
%     \item $D_{ix}$ : Function value for finding a representative for an element i $\in$ X with past representative set as $S \cup x$ or $T \cup x$.
% \end{enumerate}
% \normalsize
% Note that there can be 3 possibilities after addition of $x$.
% \small
% \begin{enumerate}
%     \item $x$ does not become a representative of $i \in X$.
%     \item $x$ becomes a representative of $i \in X$ only with past representative set as $S$.
%     \item $x$ becomes a representative of $i \in X$ with both $S$ and $T$ as past representative sets. 
% \end{enumerate}
% \normalsize
% To prove: 
% \small
% \begin{equation}
%     f(S) - f(S \cup \{x\}) \geq f(T) - f(T \cup \{x\})
% \end{equation}
% \normalsize
% or
% \small
% \begin{equation}
%     D_i(S) - D_{ix} \geq  D_i(T) - D_{ix}
% \end{equation}
% \normalsize
% Under the first possibility, both sides of inequality lead to $0$.

% Since $S \subseteq T$, by the form of $f(S)$, $D_i(T) \leq D_i(S)$. Addition of representative for an element $i \in X$ can either decrease the function value or keep it the same.
% \small
% \begin{equation}
%     \therefore{} D_i(T) - D_{ix} \geq 0 , 
%     D_i(S) - D_{ix} \geq 0
% \end{equation}
% \normalsize
% Hence, under the second possibility, $D_i(S) - D_{ix} \geq  D_i(T) - D_{ix}$ or $D_i(S) - D_{ix} \geq  0$.

% Now, $\because D_i(T) \leq D_i(S), \therefore{} D_i(T) - D_{ix} \leq D_i(S) - D_{ix}$ or $D_i(S) - D_{ix} \geq D_i(T) - D_{ix}$.

% Therefore, $-f(S)$ is submodular.

Inspired from algorithm proposed in  SODA 2014\cite{buchbinder2014submodular} based on constrained submodular maximisation, we adopt it in our framework in Algorithm \ref{algo:submodular}. The algorithm is a randomised greedy algorithm that examines the dataset $k$ times to select representatives for the incoming data.
\small
\begin{algorithm}[tb]
 \caption{: Subset Selection using Submodular approach}
 \label{algo:submodular}
 \begin{algorithmic}[1]
 
 \State \textbf{Input:}
 \State \hspace{2mm}$S_0$: Initial representative set
 \State \hspace{2mm}$X$: Incoming Set of Instances
 \State \hspace{2mm}$k$: Subset cardinality
 \State \hspace{2mm}$f(S)$: Function to be maximised
 \State \hspace{2mm}$S_0 = \phi$
%  \State \hspace{2mm}$T$: Number of incoming batches
 \State \textbf{Process:}
 \hspace{2mm}\For{$i$ = 1,2, $\ldots$, $k$}
 \hspace{2mm}\For{each x $\in$ X \textbackslash $S_{i-1}$} do
 \State  $fv_x \leftarrow f(S_{i-1} \cup {x})$
  \EndFor
%  \State  Select a subset of size $k$ , say $M_i$ such that they yield the maximum value in $fv$
 \State  Select a subset of size $k$ , say $M_i$ such that $\sum_{m \in M_i} fv_m$ is maximised
 \State  Let $u_i$ be a random element from $M_i$ 
 \State $S_i \leftarrow S_{i-1}\cup {u_i}$
 \EndFor
 \State \textbf{Output:}
 \State $S_k$ : Subset of size $k$
 \end{algorithmic}
\end{algorithm}
\normalsize

%\subsection{Convex formulation}

% This can be posed as an online subset selection problem \cite{elhamifar2017online}. Given a datapoint $i$ from the set $X_{t+1}$ and another datapoint $j$ from the set $R_t$, $R_{t+1}$ is constructed by solving the problem:
% \small
% \begin{align}
% \label{eqn:eq1}
%     &\min_{z^o_{ij},z^n_{ij}} & \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij} + \sum_{i,j=1}^m z_{ij}^n d^n_{ij} + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
%     &s.t. & \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
%     & & z_{i,j}^n, z_{i,j}^o \in [0,1]
%     \nonumber
% \end{align}
% \normalsize
% where $d^o_{ij}$ denotes the notion of dissimilarity between new frame $i$ (from $X_{t+1}$) and old frame $j$ (from $R_t$), $d^n_{ij}$ denotes the notion of dissimilarity between new frames $i$ and $j$ (from $X_{t+1}$), and $z_{ij}^o, z_{ij}^n $ are relaxed versions of binary assignment variables. $z_{ij}^o=1 $ denotes that the representative of $i^{th}$ new example (from $X_{t+1}$) is $j^{th}$ old example (from $R_t$), and $z_{ij}^n=1$ denotes that representative of $i^{th}$ new example (from $X_{t+1})$ is the $j^{th}$ new example. Note that here, the indexes $i,j$ are internal to sets $R_t$ and $X_{t+1}$ depending on context $o$ or $n$.

% While $d_{ij}$ can be used to encode the perceptual dissimilarity between video frames $i$ and $j$, the above formulation does not incorporate the the pointwise attributes of each data point $x_i,y_i$ w.r.t. to the already trained model $M_t$, where $(x_i,y_i)\in X_{t+1}$. Let $L^n_i$ denote the loss value for datapoint $i$ in $X_{t+1}$ and analogously for $L^o_i$ (denoting loss for datapoint $i$ in $R_t$). \cite{das2020multi} proposes to incorporate it by constructing the $Q$ function as a weighted average of $d$  and $L$ as:

% \small
% \begin{equation}
% Q_{ij} = \rho d_{ij} - (1-\rho) L_j
% \label{eq:joint}
% \end{equation}
% \normalsize
% where, $0 \leq \rho \leq 1$ is the weightage given to pairwise dissimilarity criteria.
% Hence, their \cite{das2020multi}  final selection problem is:
% \small
% \begin{align}
% \label{eqn:oldsiftloss}
%     &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
%     &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
%     & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
% \end{align}
% \normalsize
% Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, as explained before, a representative $j$ should have the minimum dissimilarity with a new frame $i$. 

% \textbf{Drawbacks of the above formulation}:\\

% The first drawback of the formulation described in Equation \ref{eqn:oldsiftloss} is that pointwise metric has very limited impact on the set of points selected. The following remark notes this when $\rho = 0$.
% \tr{To see this, note that using only pointwise metric yields a maximum of 1 representative for all images belonging to incoming set.
% An interesting observation is that when $\rho = 0$, either $0$ or $1$ new representative points are selected. }

% \begin{remark}
% For pointwise score ($\rho = 0$), the score function is $- \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t)+ \nonumber \\ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \right]$

% A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
% \begin{itemize}
% \item $L^n_j$ is the highest among all $j\in X_{t+1}$.
% % \item $L^n_j > L^o_i,\ \forall i\in R_t$
% \item $L^n_j > \frac{ \sum_{i=1}^m z_{i,k}^o L_k^o + \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
% \end{itemize}

% The last condition for $p=2$ boils down to $l_j^n \geq \frac{1}{\sqrt{m}}$.

% \end{remark}

% \begin{remark}
% For $\rho = 0.1$ to $0.5$, the score function is $\sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q^o_{ij} + \sum_{i,j=1}^m z_{ij}^n Q^n_{ij} \nonumber \\ + \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\$

% A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
% \begin{itemize}
% \item $Q^n_{ij} < Q^n_{ij'}$ where $j \neq j'$
% % \item $L^n_j > L^o_i,\ \forall i\in R_t$
% \item $Q^n_{ij} < \frac{ \sum_{i=1}^m z_{i,k}^o Q^o_{ik} - \lambda \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
% \end{itemize}

% The last condition for $p=2$ boils down to $l_j^n \geq \frac{1}{\sqrt{m}}$.

% \end{remark}

% \begin{remark}
% For pointwise score ($\rho = 0$), the score function is $ - \left[ \sum_{j=1}^{|R_t|} z_{i,j}^o  L^o_j + \sum_{j=1}^m z_{i,j}^n  L^n_j(t) \right] $. 
% A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
% \begin{itemize}
% \item $L^n_j$ is the highest among all $j\in X_{t+1}$.
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
% \item $L^n_j > \lambda \frac{\| [z_{1,j}^n \dots z_{m,j}^n ] \|_p }{\sum_{i=1}^m z_{ij}^n} $
% \end{itemize}
% The last condition for $p=2$ boils down to $l_j^n \geq \frac{1}{\sqrt{m}}$.

% \end{remark}

%%%%% Example with rho = 0
% Let both $R_t$ and $X_t$ have two frames each.\\
% $d^o = \begin{bmatrix}
% 1 & 2\\
% 1 & 3
% \end{bmatrix}$ , $d^n = \begin{bmatrix}
% 2 & 1\\
% 1 & 3
% \end{bmatrix}$ , $L^o = \begin{bmatrix}
% 1 & 3
% \end{bmatrix}$ and $L^n = \begin{bmatrix}
% 2 & 1
% \end{bmatrix}$. When $\rho$ = 0, from Equation \ref{eq:join}, $Q_{ij}^o$ = $- (1-\rho) L_j^o$ and similarly, $Q_{ij}^n$ = $- (1-\rho) L_j^n$. Having used the above values in Equation \ref{eqn:oldsiftloss}, representative of any instance $i$ from $X_t$ $(i = 1, ..., m)$ will be the point which has the highest value of loss which can either belong to $L^o$ or $L^n$. So, all the frames in $X_t$ will be represented by only one frame from $X_t$ or $R_t$ whichever yields the highest loss. In the above mentioned example, the second frame from $R_t$ ($\because L^o[1] = 3$) will be chosen as the representative for all the frames in $X_t$.

% \tr{The second drawback is that there is no obvious connection between intended compression ratio, and $\lambda$.} Hence, one has to perform grid search over the values of $\lambda$ in order to obtain a particular compression ratio.


\subsection{Convex formulation}

Overcoming the drawbacks in formulation \ref{eqn:oldsiftloss}, we designed the following convex optimisation problem:
\small
\begin{align}
\label{eqn:newsiftloss}
    \min_{z^o_{ij},z^n_{ij}} & \rho \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij}(t) + \sum_{i,j=1}^m z_{ij}^n d^n_{ij}(t) \nonumber \\ & -(1-\rho) (\sum_{j=1}^{|R_t|} S_j^o * L_j^o  + \sum_{j=1}^m S_j^n * L_j^n )\\
    &s.t. \sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
    &z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber \\ 
    &\sum_{j=1}^{m}\| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \leq frac * m
    \nonumber
\end{align}
\normalsize

where, $S^o_j$ = $\frac{1}{\epsilon} \min (\epsilon , \sum_{i=1}^m z_{ij}^o)$ , $S^n_j$ = $\frac{1}{\epsilon} \min (\epsilon , \sum_{i=1}^m z_{ij}^n)$ are the vectors with each element indicating whether j-th indexed image is a representative of any incoming image or not.
$L_j^o$ and $L_j^n$ refer to the pointwise metric (here multi-task loss) corresponding to images belonging to existing and incoming set respectively and, \textit{frac} indicates the fraction of elements we want to retain during selection.
$\epsilon$ is a user input which is designed to be the maximum value taken by the variable $\sum_i z_{ij}$, when none of the $z_{ij}$ denote a representative relation to be true. In an ideal situation (when we achieve a $\{0,1\}$ solution to $z_{ij}$), any positive value for $\epsilon$ is sufficient. In practise, we set $\epsilon$ to a value less than $1$, e.g. $\epsilon = 0.9$. The following conditions must hold for obtaining the exact solution for our proposed optimization problem.

\begin{theorem}
The score function in Equation \ref{eqn:newsiftloss} is $ \rho (\sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} d^o_{ij} + \sum_{i,j=1}^m z_{ij}^n d^n_{ij}) - (1 - \rho)( \sum_{j=1}^{|R_t|} S_j^o * L_j^o + \sum_{j=1}^m S_j^n * L_j^n)$

A new point $j$ from the set $X_{t+1}$ is selected as a representative by minimizing the above function, only if all of the following hold:
\begin{itemize}
\item $\sum_{i=1}^m z_{ij} \geq \epsilon$
% \item $L^n_j > L^o_i,\ \forall i\in R_t$
\item $\rho \sum_{i=1}^m z_{ij}^{n} d^n_{ij}(t) -(1-\rho) (S_j^n * L_j^n) \leq \sum_{i=1}^m z_{ik}^n d^o_{ik}(t) -(1-\rho)(S_k^o * L_k^o) + max(|d_{ik}^o - d_{ij}^n| , |L_k^o - L_j^n|)$
\end{itemize}
where k = $argmin_j (\rho \sum_{i=1}^m z_{ij}^{o} d^o_{ij} - (1- \rho) S_j^o * L_j^o)$
\end{theorem}

\noteng{Is this your only contribution -- I am confused. }
The key difference between the current formulation and the formulation in equation \ref{eqn:oldsiftloss} is that, in the current formulation, each potential representative can contribute a maximum of its own (negative) loss value, since $S_j$'s can take a maximum value of $1$. Whereas in the formulation in  equation \ref{eqn:oldsiftloss} it is possible for a datapoint to contribute $ - \sum_{i=1}^{m} (L_i^n + L_i^o)$ by becoming a representative for every other point. However, in reality it only adds one data point to the training set. Also, note that $S$ is a concave function, which makes the current formulation a convex optimization problem.

Compression ratio has no direct relation with the parameter $\lambda$. In order to have a control over the selection, we bring the cardinality criteria into the constraints by introducing the term \textit{frac} which is manually provided based on the desired compression ratio. For instance, for a compression ratio of 100:20, we provide the value of \textit{frac} as 0.2. Hence, this provides a more flexible approach to perform subset selection using convex optimisation whose performance is explored in the next section.

% The subset cardinality was manually tuned with the help of $\lambda$ in Equation \ref{eqn:oldsiftloss}.  In order to have a control over the selection, we brought the cardinality criteria into the constraints by introducing the term \textit{frac} which is manually provided based on the desired compression ratio. For instance, for a compression ratio of 100:20, we provide the value of \textit{frac} as 0.2.


%Since, most of the frames that are input to the driving model and are redundant in terms of information content, and cause a huge overhead in terms of processing power at runtime as well as training time. 
%In this paper, we propose subset selection mechanisms for intelligent selection of images which can be fed to the existing models for autonomous driving and can be trained and tested (operated) on videos with massively and unevenly dropped frames.

%\subsection{Model Description}

%We consider a dataset $\mathcal{D}$ comprising of datapoints (e.g. buffers of video frames) $x_i$, and labels $y_i$ corresponding to various learning tasks on buffers of video frames such as prediction of driving affordances. 
%The data may arrive in either a streaming manner, or in batches. 

%\subsection{Multiple-criteria-based subset selection}

%The above formulation relies on (dis)similarity between the examples in the new set ($X_{t+1}$) and existing representative set ($R_{t}$), for selecting the new representatives. However, this does not take care of the possibility that in many application scenarios, one is interested in selecting points which provide better performance towards a given task. For example, one could be interested in selecting video frames from a self driving car video, which are helpful towards training a driving model. In such scenarios, it is important to also consider other signals, e.g. loss which are dependent on models trained on old representative datapoints (frames). In this section, we develop a novel formulation for using such criteria.

%Let $M_t$ be the model trained on $R_t$.
%%, and $l_t(x_i,y_i)$ be the loss incurred by the datapoint $(x_i,y_i), i\in C_{t+1}$, using the model $M_t$. 
%For our formulation, we further define two types of selection criteria: \textit{pairwise and pointwise criteria}. Pairwise dissimilarity criteria $d_{ij}(t)=d((x_i,y_i), (x_j,y_j) | M_t) $ are evaluated on pairs of examples $( (x_i,y_i), (x_j,y_j) )$ at any point in time. Note that $d_{ij}(t)$ may or may not depend on the current model. For example, in this paper we use SIFT \cite{lowe1999object} as a measure of dissimilarity, which is related to the perceptual dissimilarity between two images and hence independent of the model.
%Pointwise ``dis-quality'' criteria $q_i(t) = q((x_i,y_i)|M_t)$ measure an inverse goodness score for a datapoint $(x_i,y_i)$ given a trained model at time $t$. 
%In this study, we consider the negative log-loss denoted as $L_i(t)=L(x_i,y_i|M_t)$. Here, the loss refers to the multi-task loss which is a combination of the losses from all affordances in the driving model.

%We define the joint pairwise and pointwise dis-quality criteria as:
%\begin{equation}
%Q_{ij}(t) = \rho d_{ij}(t) + (1-\rho) q_j(t) \label{eq:joint}
%\end{equation}
%where, $0 \leq \rho \leq 1$ is the weightage given to pairwise dissimilarity criteria.

%We have setup the joint dis-quality criteria above in a manner such that new datapoints with lower dis-quality score results in better candidates for selection. Hence we pose the  final selection problem as:
%\begin{align}
%\label{eqn:oldsiftloss}
%    &\min_{z^o_{ij},z^n_{ij}} \sum_{i=1}^m \sum_{j=1}^{|R_t|} z_{ij}^{o} Q_{ij}(t) + \sum_{i,j=1}^m z_{ij}^n Q_{ij}(t) \nonumber \\ &+ \lambda \sum_{j=1}^m \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p \\
%    &s.t.\sum_{j=1}^{|R_t|} z_{i,j}^o + \sum_{j=1}^m z_{i,j}^n = 1 \nonumber \\
%    & z_{i,j}^n, z_{i,j}^o \in [0,1] \nonumber
%\end{align}
%Here $z_{ij}^o=1$ or $z_{ij}^n=1$ implies that $j^{th}$ old or new frame is the representative of $i^{th}$ new frame. For pairwise score, as explained before, a representative $j$ should have the minimum dissimilarity with a new frame $i$. 

%Unlike the last formulation where pairwise and pointwise metrics were weighed into a single matrix $Q_{ij}$, here we separated the metrics giving each of them their respective indicator variable. This aids in bringing out the impact of pointwise metrics on subset selection. We also resort to pointwise "quality" criteria instead of the inverse goodness score used in Equation \ref{eqn:oldsiftloss}.

% with lowest value of $q_j(t)$ is selected only when $q_j(t) < \lambda  \| [z_{1,j}^n \dots z_{m,j}^n ] \|_p $. Hence, these hyperparameter values produce trivial results.

%\subsection{Improved Multiple-criteria-based subset selection}
%\label{improved}

%In this formulation, we intend to address the shortcomings in the last formulation. The drawbacks of the method described in Equation \ref{eqn:oldsiftloss} are:
%\begin{enumerate}
%    \item Using only pointwise metric yields only 1 representative for all images belonging to incoming set. This suppresses the impact of the pointwise metrics on the subset selection.
%    \item We have to grid search for the value of $\lambda$ in order to obtain a particular compression ratio.
%\end{enumerate}

==> related_short.tex <==
% \tr{driving model}

% \tr{subset selection}
% In this section, we set the stage for our work by surveying two following strands of research: (i) Learning model for self-driving cars (ii) Subset selection.
In this section, we describe few relevant prior works in the area of subset selection.
There are mainly two classes of works surrounding subset selection - one where deep learning models are used for the purpose of selection and the other, where selection is performed using different criteria provided by the user. The first class of techniques \cite{lan2018ffnet}, \cite{Wu_2019_ICCV} \cite{Wu_2019_CVPR} do not come with any optimal algorithmic guarantees with respect to the selection criteria. These are typically selection networks added to the pipeline of existing tasks and are trained jointly. While \cite{Wu_2019_ICCV} and \cite{Wu_2019_CVPR} learn a policy for the task of video recognition , \cite{lan2018ffnet} approaches subset selection as a fast-forwarding problem. All of these methods, coupled with the training algorithms, are typically too expensive to be deployed on edge devices. The second class of techniques essentially selects the data points based on different defined criteria. These criteria may include reconstruction error \cite{chen2012surveillance}, linear dependency \cite{joneidi2020select}, perceptual similarity \cite{elhamifar2017online} or criteria based on end tasks such as distinctiveness and uncertainty \cite{huang2018cost} \cite{das2020multi}. However, neither of \cite{chen2012surveillance} , \cite{joneidi2020select}, \cite{elhamifar2017online} used any task-specific metric in their optimisation algorithms. On the other hand, \cite{huang2018cost} proposed an approach for subset selection in image classification, where pointwise metrics like distinctiveness and uncertainty from the classification model were used in an active learning setting. This helped in selecting and querying limited number of significant samples thus making it cost-efficient, yet maintaining appropriate model performance.

In this work, we specifically focus on the criteria based techniques to develop our subset selection method. Following the two line of works \cite{elhamifar2017online}, \cite{huang2018cost}, the authors of \cite{das2020multi} used a combination of pairwise and pointwise metrics for selecting subset of frames from videos with the end-task of semantic segmentation. We build on the work of \cite{das2020multi}, focusing on their limitations and adapting our proposed formulation in a more difficult task of autonomous driving which as we know, depends on several tasks in hand. We develop techniques to prioritize the important tasks essential for the task of autonomous driving and incorporate it in our subset selection method.
